Capuchin: Causal Database Repair for Algorithmic Fairness

Fairness is increasingly recognized as a critical component of machine learning systems. However, it is the underlying data on which these systems are trained that often reflect discrimination, suggesting a database repair problem. Existing treatments of fairness rely on statistical correlations that can be fooled by statistical anomalies, such as Simpson's paradox. Proposals for causality-based definitions of fairness can correctly model some of these situations, but they require specification of the underlying causal models. In this paper, we formalize the situation as a database repair problem, proving sufficient conditions for fair classifiers in terms of admissible variables as opposed to a complete causal model. We show that these conditions correctly capture subtle fairness violations. We then use these conditions as the basis for database repair algorithms that provide provable fairness guarantees about classifiers trained on their training labels. We evaluate our algorithms on real data, demonstrating improvement over the state of the art on multiple fairness metrics proposed in the literature while retaining high utility.

==> Capuchin(Pre-print) (1)/appx.tex <==

\vspace*{-0.3cm}
\section{Appendix}

\subsection{Additional Background}
\label{app:addback}





\paragraph{\bf New Proof of Impossibility Result in ~\cite{chouldechova2017fair}}
Chouldechova~\cite{chouldechova2017fair} proves the following {\em
impossibility result}: the Equalized Odds and Predictive Parity are
impossible to achieve simultaneously when prevalence of the two
populations differs, meaning $\pr(Y=1|S=0) \neq \pr(Y=1|S=1)$.  The
proof follows immediately from her observation that, for each
population group $S=i$, the following holds\footnote{EO implies
$FP/(1-FN)$ is the same for both groups,
$\frac{\pr(O=1|S=0,Y=0)}{\pr(O=1|S=0,Y=1)}=\frac{\pr(O=1|S=1,Y=0)}{\pr(O=1|S=1,Y=1)}$,
while PP implies that $(1-PPV)/PPV$ is the same for both groups,
$\frac{\pr(Y=0|O=1,S=0)}{\pr(Y=1|O=1,S=0)}=\frac{\pr(Y=0|O=1,S=1)}{\pr(Y=1|O=1,S=1)}$.
When the prevalence differs, EO and PP cannot hold simultaneously.}:
 %
\begin{align*}
 \frac{\pr(O=1|S=i,Y=0)}{\pr(O=1|S=i,Y=1)} =
%
 &  \frac{\pr(Y=1|S=i)}{\pr(Y=0|S=i)}  \frac{\pr(Y=0|O=1,S=i)}{\pr(Y=1|O=1,S=i)}
\end{align*}

The following provides a simple alternative proof of the impossibility result using conditional independence.
%
\begin{prop} \label{prop:imp}  For any probability distribution $\pr$, if $S \indep O| Y$ and $S \indep Y| O$ then $S \indep Y$.
\end{prop}
%
\begin{myproof}{Proposition}{\ref{prop:imp}}  \em
From  $S \indep O| Y$ and  $S \indep Y| O$  it follows that $\pr(S|Y)=P(S|O)$ (1), which in turns implies $\pr(Y|S)\pr(O)=\pr(O|S)\pr(Y)$ (apply Bayes rule to the both sides of (1)). By summarization over $O$ we get $\pr(Y|S)=\pr(Y)$, which completes the proof.
\end{myproof} 
%
\paragraph*{\bf Implication Problem for CIs} The implication problem for CI is the problem of deciding whether  a CI $\varphi$ is logically follows from  a set of CIs $\Sigma$, meaning that in every distribution in which $\Sigma$ holds, $\varphi$ also holds. The following set of sound but incomplete axioms, known as {\em Graphoid}, are given in \cite{pearl1985graphoids} for this implication problem.


	Suppose $\att$ consists of a set of protected attributes $\mb P$ such as race and gender;  a set of  attributes $\mb X$ that might be used for decision making, e.g., credit score; a binary outcome attribute $Y$, e.g., good or bad credit score.
	Assume a classifier is trained on $S \subseteq \mb P \cup \mb X$ to predict $Y$.  Suppose $O$ consists of the classifier decisions. Throughout this paper we assume the classifier provides a good appropriation of the conditional distribution of $Y$, i.e.,  $\pr(Y|S) \approx \pr(O|S)$. 

\begin{itemize}

	\item (\bf Symmetry)
	\begin{align}
	(\mb X \indep \mb Y| \mb Z) \rightarrow (\mb Y \indep \mb X| \mb Z)  \label{ax:sy}
	\end{align}
	\item (\bf Decomposition)
	\begin{align}
	(\mb X \indep \mb W \mb Y|  \mb Z)  \rightarrow (\mb X \indep \mb W|  \mb Z)  \label{ax:dec}
	\end{align}
	\item (\bf	Weak Union)
	\begin{align}
	(\mb X \indep \mb W \mb Y|  \mb Z)  \rightarrow 	(\mb X \indep  \mb Y|  \mb Z \mb W)  \label{ax:wu}
	\end{align}

	\item (Contraction)
	\begin{align}
	(	\mb X \indep \mb Y|  \mb W \mb Z) \land  (\mb X \indep \mb W|  \mb Z) \rightarrow (\mb X\indep \mb Y \mb W | \mb Z)	 \label{ax:con}
	\end{align}
\end{itemize}


For strictly positive distribution in addition to the above the following axiom also holds:

{
\begin{itemize}
	\item ({\bf Intersection})
	\begin{align}
	(	\mb X \indep \mb Y|  \mb W \mb Z) \land  (\mb X \indep \mb W| \mb Y \mb Z) \rightarrow (\mb X\indep \mb Y \mb W | \mb Z)	 \label{ax:int}
	\end{align}
\end{itemize}
}


\paragraph*{\bf  Causal Models}  A probabilistic causal model (PCM) is a tuple
$\cm = \langle \mb U, \mb V , \mb F, \pr_{\mb U} \rangle$, where
$\mb U$ is a set of background or exogenous variables that cannot be
observed but which can influence the rest of the model; $\mb V$ is a
set of observable or endogenous variables;
$\mb F = (F_X)_{X \in \mb V}$ is a set of \emph{structural functions}
$F_X : Dom(\mb{Pa}_{\mb U}(X)) \times Dom(\mb{Pa}_{\mb V}(X))
\rightarrow Dom(X)$,
where $\mb{Pa}_{\mb U}(X) \subseteq \mb{U}$ and
$\mb{Pa}_{\mb V}(X) \subseteq \mb V-\set{X}$ are called the exogenous
parents and endogenous parents of $X$ respectively; and $\pr_{\mb U}$
is a joint probability distribution on the exogenous variables
$\mb U$.  Intuitively, the exogenous variables $\mb U$ are not known,
but we know their probability distribution, while the endogenous
variables are completely determined by their parents (exogenous and/or endogenous).

\paragraph*{\bf Causal DAG}  To each PCM $\cm$ we associate a causal graph $\cg$ with nodes
consisting of the endogenous variables $\mb V$, and edges consisting
of all pairs $(Z,X)$ such that $Z \in \mb{Pa}_{\mb V}(X)$; we write
$Z \rightarrow X$ for an edge.  $\cg$ is always assumed to be acyclic,
and called Causal DAG.  One can show that the probability distribution
on the exogenous variables uniquely determined a distribution
$\pr_{\mb V}$ on the endogenous variables and, under the {\em causal
	sufficiency} assumption\footnote{The assumption requires that, for
	any two variables $X, Y \in \mb{V}$, their exogenous parents are
	disjoint and independent
	$\mb{Pa}_{\mb U}(X) \indep \mb{Pa}_{\mb U}(Y)$.  When this
	assumption fails, one adds more endogenous variables to the model to
	expose their dependencies.}, $\pr_{\mb V}$ forms a Bayesian network,
whose graph is exactly $\cg$:

\begin{align}
\pr(\mb V) = & \prod_{X \in \mb V} \pr(X | \mb{Pa}(X)) \label{eq:bayesian}
\end{align}

Thus justifies omitting the exogenous variables from the causal DAG,
and capturing their effect through the probability distribution
Eq.(\ref{eq:bayesian}).  We will only refer to endogenous variables,
and drop the subscript $\mb{V}$ from $\mb{Pa}_{\mb{V}}$ and
$\pr_{\mb{V}}$.  A path in $\cg$ means an undirected path, i.e. we may
traverse edges either forwards or backwards; a directed path is one
where we traverse edges only forwards.

\paragraph*{\bf d-Separation} We review the notion of d-separation,
which is the graph-theoretic characterization of conditional
independence.  A {\em path} $\mb{P}$ from $X$ to $Y$ is a sequence of
nodes $X = V_1, \ldots, V_\ell = Y$ such that
$V_i \rightarrow V_{i+1}$ or $V_i \leftarrow V_{i+1}$ forall $i$.
$\mb P$ is {\em directed} if $V_i \rightarrow V_{i+1}$ forall $i$, and
in that case we write $X \stackrel{*}{\rightarrow} Y$, and say that
$X$ is an {\em ancestor}, or a {\em cause} of $Y$, and $Y$ is a {\em
  descendant} or an {\em effect} of $X$.  If the path contains a
subsequence $V_{k-1} \rightarrow V_k \leftarrow V_{k+1}$ then $V_k$ is
called a {\em collider}.  A path with a collider is {\em closed};
otherwise it is {\em open}; an open path has the form
$X \stackrel{*}{\leftarrow} \stackrel{*}{\rightarrow} Y$, i.e.  $X$
causes $Y$ or $Y$ causes $X$ or they have a common cause.  Given two
sets of nodes $\mb{X},\mb{Y}$ we say that a set $\mb{Z}$ {\em
  d-separates}\footnote{d stands for ``directional''.}  $\mb X$ and
$\mb Y$, denoted by $(\mb{X} \indep \mb{Y} |_d \ \mb{Z})$, if for any
all paths $P$ from $\mb{X}$ to $\mb{Y}$ one of the followings hold:
(1) $\mb P$ is closed at a collider node $V$ such that neither $V$ nor
any of its descendants are in $\mb Z$; (2) $\mb P$ contains a
non-collider node $V'$ such that $V' \in \mb P$. We say that a set
$\mb{Z}$. d-Separation is a sufficient condition for conditional
independence, see Prop.~\ref{prop:d:separation}

%for any open path $P$ from $\mb{X}$ to $\mb{Y}$, $\mb{Z} \cap \mb{P} \neq \emptyset$ (``$\mb{Z}$ closes all open paths''), and (2) for any path from $\mb X$ to $\mb Y$ and any collider $V$ on this path, $\mb Z$ does not contain either $V$ or any of its descendants (``$\mb{Z}$ does not open any closed path'' \dan{I don't think this statement is correct}).  \babak{My Suggestion: We say $\mb Z$ closes a path $\mb P$ between $\mb X$ and $\mb Y$ if one of the following holds: (1) $\mb P$ contains a collider node $V$ such that neither $V$ nor any of its descendants are  in $\mb Z$; (2) $\mb P$ contains a non-collider node $V'$ such that $V' \in \mb P$. We say that a set $\mb{Z}$ {\em d-separates}\footnote{d stands for ``directional''.}  $\mb X$ and $\mb Y$, denoted by $(\mb{X} \indep \mb{Y} |_d \ \mb{Z})$ iff $\mb Z$ closes all pathes between $\mb X$ and $\mb Y$.}


\paragraph*{\bf General Identification Criterion} In the presence of unrecorded variables in the causal DAG, the effect of interventions can not be identified using Eq.~\ref{eq:af}. A set of sound and complete axioms known as {\em $do$-calculus} can be used to decide whether the effect of intervention can be identified from the observed distribution \cite{pearl2009causality}. If the effect is identifiable  then by repeatedly applying the rules of do-calculus, one can obtain an statement {\em equivalent} to Eq.~\ref{eq:af}, but free from unobserved variables. Since identification is not the focus of this paper,  we assume all variables are observed hence Theorem \ref{theo:af} is sufficient for identification.



\paragraph*{\bf Markov Blanket}   We briefly review the notion of Markov
blanket, which used in Sec~\ref{sec:jfc}.
\vspace*{-0.1cm}
\begin{defn} \cite{pearl2014probabilistic} Fix a joint probability
	distribution $\pr(\mb v)$ and a variable $X \in \mb V$.  A set of
	variables $\mb  B(X) \subseteq \mb V - \set{X}$ is called a {\em Markov
		Blanket} of $X$ if $(X \indep \mb V - \mb  B(X) - \set{X} | \mb  B(X))$;
	it is called a {\em Markov Boundary} if it is minimal w.r.t. set
	inclusion,  denoted
	$\mmb(X)$.
\end{defn}

In the admission process in Fig~\ref{ex:cmexm}	$\mmb(X)=\{D,H\}$, simply because $O \indep G| H, D$ (since $\set{H,D}$ d-separate $O$ and $G$).
%The following relates Markov boundary with causal DAGs.
%\babak{moved from body. To be revised}
It is known that if $\pr$ is a strictly positive distribution (i.e., forall $\mb v \in Dom(\mb V), P(\mb v)>0$), then $\mmb(V)$ is unique for all $V \in \mb V$  and can be learned from data in polynomial time \cite{margaritis2003learning}. Strictly positive distributions do not allows for logical functional dependencies between their variables. The requirement can be satisfied in data by removing logical dependencies \cite{salimi2018bias}. Note that under the faithfulness assumption, the Markov boundary of a node $X$ in the causal graph consists of the parents of $X$, the children of $X$, and the parents of the children of $X$ \cite{neapolitan2004learning}. %Note that Markov boundary can learned from data in polynomial time \cite{margaritis2003learning}.


Note that if $\mb X$ is the set of all inputs of the algorithm included in data, then $\mmb(O)=\mb X$, i.e., parents of $X$ form a boundary for $O$. This is because $(O \indep  \mb V-\mb X|\mb X)$ is implied from the functional dependency (FD) $\mb X \fd O$, which can be discovered from data by a linear search through the attributes. Hence, ROD essentially requires that conditioned on admissible inputs of $\mb X \cap \mb A$, the outcome of algorithm becomes independent of the protected attribute, meaning the algorithm treats similarly individuals that are similar on $\mb X \cap \mb A$ characteristics but  different in $S$. Any imbalance indicated by ROD is worrisome and requires scrutiny.  Also note that in general Markov boundary can be learned from data by the linear number of iterations through the variables \cite{margaritis2003learning}.


\begin{prop}  \label{prop:umb}  Fix a strictly positive probability distribution $\pr_{\mb V}$.   It holds that for any variable $V \in \mb V$, the unique Markov boundary of $V$, $\mmb(V)$ is unique.
\end{prop}

\begin{myproof}{Proposition}{\ref{prop:umb}}{  The uniqueness of the Markov Boundary is implied from the intersection axiom (cf.  Eq~\ref{ax:int}) as follows:
Without loss of generality suppose $\mb V= V\mb X \mb W \mb Z \mb Y$, where $\mb X$ and $\mb Y$ are disjoint. We show that   if two sets $\mb X \mb Z$  and $\mb Y \mb Z$ form a Markov boundary for $V$ then their intersection, i.e, $Z$ is  a Markov blanket for $V$. This contradicts the subset minimality of a Markov boundary.  We show this in the following steps using Graphoid axioms.

			\begin{align}
	  V &\indep \mb W, \mb Y|	\mb X \mb Z  \label{mb1} \\
		  V &\indep \mb W, \mb X|	\mb Y \mb Z   \label{mb2} \\
		  V &\indep \mb Y, \mb X|	\mb Z   \hspace*{0.5cm}  \label{inter}  \text{By  (\ref{mb1}) ,  (\ref{mb2})  Dec. and Inter. axioms} \\
	  V &\indep \mb W|	\mb X \mb Z \mb Y \hspace*{0.3cm} \label{wu}  \text{By  (\ref{mb1}) and Weak Union} \\
	  	  V &\indep \mb W\mb X\mb Y |	\mb Z  \hspace*{0.3cm}    \text{By  (\ref{inter}) ,  (\ref{wu}) and Contraction}  \nonumber
	\end{align}

Therefore, Markov Boundary of $V$ is unique.
}
\end{myproof}
%\subsection{\bf Extra Propositions}
%\label{app:prop}


%\begin{prop} \label{prop:imposib} Given three variables $S,Y$ and $O$, if  $S \indep Y|O$ and  $S \indep Y|O$ then  $S \indep Y$
%\end{prop}


%\subsection{\bf Extra Examples}

%\begin{example}  \label{ex:eo_exm}
%Let us simplify the admission process example and suppose $G \rightarrow H \leftarrow  Q \rightarrow O$,  $Q$ represent applicant qualifications. The causal DAG models a admission process in which admission decisions are only based on applicants qualifications. However, applicants gender and their qualifications influence their hobbies. It is known DAG for any distribution that is faithful to this DAG, G \indep O How

% The causal DAG models  a discriminative collage that only admits qualified males. It also asserts that applicant qualifications is independent of their gender, i.e.,  $G \indep Q$. Suppose a classifier only uses $Q$ to predict $A$, i.e., $O=Q$. Clearly, the classifier is not discriminative and satisfies DP, i.e., $P(O=1|\text{male})=P(O=1|\text{female})=\frac{1}{2}$. However, $\pr(O=0|\text{male}, A=0)=1$
%but $\pr(O=1|\text{female}, A= 0)=\frac{1}{2}$. (This is simply because conditioning on $Y$ opens the path between $O$ and $S$, hence renders spurious correlation between them; this phenomenon known as Berkson's paradox, see \cite{pearl2009causality}).
%\end{example}


\ignore{
\babak{needs to be revised}
\begin{example}  \label{ex:dod_more}First we compute degree of discrimination in the proceed represented by the causal DAG shown in Fig.~\ref{fig:cgex}(b), we have


	\begin{align}
	\qii(A,G| D) &=& \E \big[ \big| \sum_{h} \Pr(A=1|\text{male},h,d) \pr(h|\text{male}) -  \nonumber \\ &&
	\Pr(A=1|\text{female}|h))    \pr(h|\text{female})  \big] \big| \label{eq:adexmp1}
	\end{align}

\end{example}

Now, notice that in the modified causal DAG after performing interventions $A$ is independent of $G$ condition on $H$ and $D$, thus, $\Pr(A=1|\text{female},h,d)=\Pr(A=1|\text{female},h,d)=\Pr(A=1|h,d)$ which further simplify

\begin{align}
\qii(A,G| D) &=& \E \big[  \big|  \sum_{h}\Pr(A=1|,h,d) (\pr(h|\text{male}) -   \pr(h|\text{female})  \big| \big] \label{eq:adexmp2}
\end{align}

Intuitively,  Eq.~\ref{eq:adexmp2} computes the effect of chancing gender on admission rate through changing applicant's height.
It is clear that $\qii(A,G| D)=0$, i.e., the admission process does not discriminate, iff $\pr(h|\text{male})= \pr(h|\text{female})=0$ or equivalently $H \indep G$. Thus, since  $H \not  \indep G$ in Fig.~\ref{fig:cgex}(b) the admission process is discriminative.

Now, let us compute $\qii(A,G| D)$ for the admission process modeled shown in Fig.~\ref{fig:cgex2}. In this case in the modified model $A$ is independent of both $G$ and $Y$ thus, \ref{eq:adexmp1} reads as:

\begin{align}
\qii(A,G| D) &=& \E \big[ \big| \Pr(A=1|d)  \big( \sum_{h}\pr(h|\text{male}) -   \pr(h|\text{female})  \big)\big| \big] \nonumber \\
&=& \E \big[ \big| \Pr(A=1|d)  (1 -  1)  \big| \big]
=0 \label{eq:adexmp2}
\end{align}

That is the te admission process is not discriminative. Indeed it is justifiably fair.
}



%	\subsection{Supplementary Propositions}

	%This section contains extra graphs for the experiments in Sec~\ref{sec:extendtoend}. Note that for AdultData, positive values of ROD indicate discrimination against protected groups. Whereas for COMPAS data,  ROD below 1 indicates discrimination against protected groups.

	\ignore{
		\begin{figure*}[htp]
			\centering


			\includegraphics[width=.3\textwidth]{fig/bias_adult_sex_orgLR.pdf} \hfill
			\hspace*{-1.5cm} 	\includegraphics[width=.3\textwidth]{fig/bias_adult_sex_orgMLP.pdf}\hfill
			\hspace*{-1.5cm} \includegraphics[width=.3\textwidth]{fig/bias_adult_sex_orgMLP.pdf}\hfill

			%\includegraphics[width=.3\textwidth]{fig/bias_compas_gender_orgLR.pdf} \hfill
			%\hspace*{-1.5cm} 	\includegraphics[width=.3\textwidth]{fig/bias_compas_gender_orgMLP.pdf}\hfill
			%\hspace*{-1.5cm} \includegraphics[width=.3\textwidth]{fig/bias_compas_gender_orgRF.pdf}\hfill

			\vspace*{0.3cm}
			\includegraphics[width=.35\textwidth]{fig/bias_compas_race_org_LR.pdf} \hfill
			\hspace*{-1.5cm} 	\includegraphics[width=.35\textwidth]{fig/bias_compas_race_org_MLP.pdf}\hfill
			\hspace*{-1.5cm} \includegraphics[width=.35\textwidth]{fig/bias_compas_race_org_RF.pdf}\hfill
			\caption{Extra graphs for experiments in Sec~\ref{sec:extendtoend}.}
			\label{fig:extendtoendextra}
		\end{figure*}
	}


	\ignore{
		\begin{figure*}[htp]
			\centering

			\includegraphics[width=.3\textwidth]{fig/bias_adult_nips_orgLR.pdf} \hfill
			\hspace*{-1.5cm} 	\includegraphics[width=.3\textwidth]{fig/bias_adult_nips_orgMLP.pdf}\hfill
			\hspace*{-1.5cm} \includegraphics[width=.3\textwidth]{fig/bias_adult_nips_orgRF.pdf}\hfill

			\vspace*{0.3cm}
			\includegraphics[width=.3\textwidth]{fig/bias_compas_nips_orgLR.pdf} \hfill
			\hspace*{-1.5cm} 	\includegraphics[width=.3\textwidth]{fig/bias_compas_nips_orgMLP.pdf}\hfill
			\hspace*{-1.5cm} \includegraphics[width=.3\textwidth]{fig/bias_compas_nips_orgRF.pdf}\hfill


			\caption{Extra graphs for experiments in Sec~\ref{sec:comp}.}
		\end{figure*}
	}


	 \paragraph*{\bf Counterfactual Fairness}   Given a set of features $\mb X$, a protected attribute $S$, an outcome variable $Y$, and a set of unobserved  background  variables $\mb U$, Kusner et
	al.~\cite{kusner2017counterfactual} defined a predictor $\tilde Y$
	to be {\em counterfactually fair} if for any $\mb x \in Dom(\mb X)$:
	%
	{ 
		%
		\begin{align}
		P( \tilde{Y}_{S\leftarrow 0}(\mb U) = 1| \mb X = \mb x,S = 1) = P( \tilde{Y}_{S\leftarrow 1}(\mb U)= 1| \mb X = \mb x;S = 1) \label{eq:cfair}
		\end{align}
		%
	}
	%
	\noindent  where, $\tilde{Y}_{S\leftarrow s}(\mb U)$ means intervening on
	the protected attribute in an unspecified configuration of the exogenous factors.
	The definition meant to capture the requirement that the protected attribute $S$ should not be a cause of $\tilde{Y}$ at individual level.  However, it fails on the simple example in Ex~\ref{ex:intsprox}. This is because, 
	$P({O}_{G\leftarrow g}(U_O) = 1)=  P(U_O=1) P({Y}_{G\leftarrow g}(U_O) = 1 | U_O=1)=\frac{1}{2}$ for $g=\set{0,1}$. We note that the stricter version of counterfactual fairness in \cite{DBLP:journals/corr/KusnerLRS17} also fails to capture the individual-level unfairness in this example. We report that this observation has been confirmed by the authors of \cite{DBLP:journals/corr/KusnerLRS17}.  We defer the full comparison for future work.

%

\begin{myproof}{Lemma}{\ref{prop:gen}} 
	Because the classifier is a deterministic function trained on $\pr_{B'}$, it follows that $\pr_{T}(o,s,i,a)=\pr_{B'}(o,s,i,a) = \pr_{B'}(o|a) \pr_{B'}(i,s,a)$.
  Hence it is sufficient to show that  $\kld{\pr_T(o|s,i,a)}{\pr_T(o|a)} = 0$ or $\pr_T(o|s,i,a)=\pr_T(o|a)$.
  We show this in the following steps:
%
%Since we mention that the classifier is trained on B', I don't think we need to repeat it inline -Luke
{ 
	\begin{align}  
	\pr_T(o|s,i,a)=& \frac{\pr_T(o,s,i,a)}{\pr_T(s,i,a)} \\
	=& \frac{\pr_{B'}(o,s,i,a)}{\pr_T(s,i,a)} \\
	=& \frac{\pr_{B'}(o|a) \pr_{B'}(s,i,a) }{\pr_T(s,i,a)} \label{rhs}
	\end{align}
}
{  
	\begin{align}
	\pr_T(o|a)=& \frac{\pr_T(o,a)}{\pr_T(a)} \\
	=& \frac{ \sum_{s,i} \pr_{B'}(o,i,s,a)}{\pr_T(a)} \\
	=& \frac{ \sum_{s,i} \pr_{B'}(o|a) \pr_{B'}(s,i, a) }{\pr_T(a)}   \\
	=& \frac{\pr_{B'}(o|a) \pr_{B'}(a) }{\pr_T(a)} \label{leh}
	\end{align}
}
	Hence,
%
{  
	\begin{align}   
	\kld{pr_T(o|s,i,a)}{pr_T(o|a)}& \\
	& \hspace*{-3cm} =  - \sum   \pr_T(o|i,s,a) \log  \frac{\pr_T(o|a)}{\pr_T(o|s,i,a)} \\
	& \hspace*{-3cm} =  - \sum  \pr_T(o|i,s,a)  \log \frac{ \frac{\pr_{B'}(o|a) \pr_{B'}(a) }{pr_T(a)}} {\frac{\pr_{B'}(o|a) \pr_{B'}(i,s,a) }{\pr_T(s,i,a)}} \\
	& \hspace*{-3cm} =  - \sum  \pr_T(o|i,s,a) \log \frac{\pr_{B'}(s,i|a)}{\pr_T(s,i|a)}  \label{ratio}
	\end{align}
}
	Thus,  $\kld{\pr_T(o|s,i,a)}{\pr_T(o|a)} = 0$ if $\pr_T(s,i|a)  \pr_{B'}(s,i|a)$,
  which implies $\pr_T(o|s,i,a)=\pr_T(o|a)$
	or equivalently that $(Y \indep S,\mb I|_{\Pr_T} \mb A)$. This completes the proof.

\end{myproof}

\subsection{\bf Proofs and Supplementary Propositions and graphs}
\label{app:proof}

\begin{myproof}{Theorem}{\ref{theo:af}}  Recall that a causal $\cg$ admits the following factorization of the observed distribution:
%
{ 	\begin{eqnarray}
	\Pr(\mb v)= \prod_{V \in \mb V} \Pr(v| \mb{pa}(V)) \label{eq:fac}
	\end{eqnarray}}
%
	Now, each atomic intervention $do(X=x)$ modifies the causal DAG  $\cg$ by removing parents of $X$ from $\cg$.  Therefore, the probability distribution $P(\mb v| do(\mb X= \mb x))$ can be obtained from the observed  distribution $P(\mb v)$  by removing all factors
	$\Pr(x|\mb{pa}(X))$, for $X \in \mb X$, from $P(\mb v)$, i.e.,
{ 		\begin{align}
	\Pr(\mb v| do(\mb X= \mb x)) & = &\frac{\Pr(\mb v)}{ \prod_{i=0}^{m} \pr(x_i|\mb{pa}(X_i))}
	\label{ps:inter}
	\end{align}}
	The following holds according to the chain rule of probability:
	{  
	\begin{align}
	\Pr(\mb v) & = & \prod_{i=0}^{m}  \bigg(\Pr\big(\mb{pa}(X_i)|  \bigcup_{j=0}^{i-1} \mb{pa}(X_j ), \bigcup_{j=0}^{i-1}x_j  \big) \bigg) \bigg(  \Pr(x_i|  \bigcup_{j=0}^{i} \mb{pa}(X_j), \bigcup_{j=0}^{i-1}x_j) \bigg) \nonumber \\
	& & \pr(\mb w| \mb x, \mb z)
	\label{ps:chain}
	\end{align}
}
	\noindent where, $\mb Z= \bigcup_{X \in \mb X} \mb{Pa}(X)$, $\mb W=\mb V-(\mb X \cup \mb Z)$ and $j \geq0$. \ignore{For example for $\mb X=\{X_0,X_1\}$ we have:
	\begin{align}
	\Pr(\mb v) & = & \Pr(\mb{pa}(X_0))   \Pr(x_0|\mb{pa}(X_0)) \nonumber  \\ & & \Pr(\mb{pa}(X_1)|\mb{pa}(X_0),x_0)   \Pr(x_1| \mb{pa}(X_0),\mb{pa}(X_1),x_0)   \nonumber  \\
	& &\pr(\mb w| \mb x, \mb z)\nonumber
	\end{align}}
	It holds that in a causal DAG $\cg$, any node $ X \in \mb V $ is independent of its non-descendant condition on it parents $\mb{Pa}(X)$ (known as Markov property \cite{pearl2014probabilistic}). This is simply because  $\mb{Pa}(X)$ d-separates $X$ from its non-descendants.  Therefore, the following is implied from
	the assumption that $X_i$ is an non-descendant of $X_{i+1}$:
		{ 
	\begin{align}
	\Pr(x_i|  \bigcup_{j=0}^{i} \mb{pa}(X_j), \bigcup_{j=0}^{i-1}x_j) = \Pr(x_i|   \mb{pa}(X_i) )
	\ \text{for} \ i=0,m
	\label{ps:indep}
	\end{align}}
	Hence,
	{ 
	\begin{align}
	\Pr(\mb v) & = &   \bigg( \prod_{i=0}^{m} \Pr\big(\mb{pa}(X_i)|  \bigcup_{j=0}^{i-1} \mb{pa}(X_j ), \bigcup_{j=0}^{i-1}x_j  \big) \bigg) \bigg( \prod_{i=0}^{m} \Pr(x_i|  \mb Pa(X_i)) \bigg) \nonumber \\
	& & \pr(\mb w| \mb x, \mb z)
	\label{ps:schain}
	\end{align}}

	The following implied from Eq.~\ref{ps:schain} and \ref{ps:inter}.
		{ 
	\begin{align}
	\Pr(\mb v| do(\mb X= \mb x)) =& \frac{\Pr(\mb v)}{ \prod_{i=0}^{m} \pr(x_i|\mb{pa}(X_i))}  \nonumber \\
	 &= \bigg( \prod_{i=0}^{m} \Pr\big(\mb{pa}(X_i)|  \bigcup_{j=0}^{i-1} \mb{pa}(X_j ), \bigcup_{j=0}^{i-1}x_j  \big) \bigg) \pr(\mb w| \mb x, \mb z)
	\label{ps:simp}
	\end{align}}
	Now,  by summation over all variables except for $Y$ and $\mb X$  in Eq.~\ref{ps:simp} we obtain the following, which proves the theorem.
	{ 	\begin{align}
	P(y|do(\mb X= \mb x ))= \sum_{ \mb z \in \mb Z } \Pr( y | \mb x, \mb z ) \bigg( \prod_{i=0}^{m} \Pr\big(\mb{pa}(X_i)|  \bigcup_{j=0}^{i-1} \mb{pa}(X_j ), \bigcup_{j=0}^{i-1}x_j  \big) \bigg)
	\end{align}}
\end{myproof}



%	\proof[   Theorem \ref{theo:fair_learn}]{ First we show  $O \indep \mb  W| \mb D$, i.e., $\pr(o|\mb d)=\pr(o|\mb w,\mb d)$ implies from (1)  $Y \indep \mb W| \mb D$ and (2) $\Pr(y| \mb d, \mb x) \approx \Pr(o| \mb d, \mb x)$.v	\begin{alignv	\Pr(o|\mb d)&=\sum_{\mb w}\Pr(o,\mb w|\mb d)&  \nonumber\\ v	&=\sum_{\mb w} \frac{\Pr(o,\mb w, \mb d)}{\pr(\mb d)}    \nonumber\\ v	&=\sum_{\mb w} \frac{\Pr(y|\mb w,\mb d)\Pr(\mb w,\mb d)}{\pr(\mb d)} \hspace*{1cm}\text{(By (2))}&\nonumber \\ v	&=\sum_{\mb w} \frac{\Pr(y|\mb d)\Pr(\mb w,\mb d)}{\pr(\mb d)}  \hspace*{0.3cm}\text{(By~(1))}\nonumber \\	&=  \Pr(y|\mb d) \sum_{\mb w}\Pr(\mb w|\mb d)&\nonumber \\ v	&=  \Pr(y|\mb d) &\nonumber \\ v	&=  \Pr(y|\mb d,\mb w)   \hspace*{1cm}\text{(By (1))}&\nonumber \\ v	&=  \Pr(o|\mb d,\mb w)  \hspace*{1cm}\text{(By (2))} &\nonumber 	\end{align}	Therefore,  (4) ($O \indep \mb  W| \mb D$) holds. Now since the classifier is trained on $\mb W \cup \mb X$ it holds that (5) $(O \indep \mb V-(\mb D \cup \mb W \cup \set{O})| \mb D,\mb W)$.  This is because $\mb D \cup \mb W$ functionally determine $O$.  Now by applying the Contraction axiom (cf.~Eq~ \ref{ax:con}) to (4) and (5) we obtain ($O \indep \mb V-(\mb D \cup \set{O})| \mb D$), which in turn implies  ($O \indep \mb \mb V'| \mb D$) for any ($\mb \mb V' \subseteq \mb V-(\mb D \cup \set{O})$) by Decomposition axiom (cf. Eq~\ref{ax:dec}). This completes the proof.
%

	\begin{myproof}{Proposition} {\ref{th:jfcd}} \em In one direction, we note that, for any choice of
		$\mb K$, the causal graph corresponding to an intervention
		$do(\mb K = \mb k)$ disconnects $S$ and $O$, and therefore
		intervening on $S$ does not affect $O$.  In the other direction, let
		$\mb P$ be a path from $S$ to $O$ s.t.
		$\mb P \cap \mb A = \emptyset$, and let $\mb K$ be the set of all
		variables not in $\mb P$; in particular, $\mb A \subseteq \mb K$.
		The causal graph corresponding to an intervention on $\mb K$
		consists of a single path $S \rightarrow^* O$ because all other
		edges are removed by the intervention.  Since $S$ has no parents,
		intervening on $S$ is the same as conditioning on $S$, and, since
		$\pr$ is faithful, we have $\pr(O=o|S=0) \neq \pr(O=0|S=1)$ for some
		outcome $O=o$, contradicting the assumption of
		$\mb K$-fairness.
	\end{myproof}
%
%
%
\begin{myproof}{Theorem}{\ref{theo:suff_jf}}  We show that an algorithm $\mc A$ is $\mb A$-fair if  $\mmb(O) \subseteq \mb A$. From Theorem~\ref{theo:af}, we obtain:
	{ 	\begin{eqnarray}
	\pr(O=o| do(S=i),do(\mb A = \mb a))= \sum_{ \mb z \in Dom(\mb Z)}  \pr( y | S=i, \mb A=\mb a, \mb z )  \nonumber \\  \bigg( \prod_{i=0}^{m} \pr\big(\mb{pa}(X_i)\bigg|  \bigcup_{j=0}^{i-1} \mb{pa}(X_j ), \bigcup_{j=0}^{i-1}x_j  \big) \bigg)
	\end{eqnarray}}
\noindent	where,  $\mb Z= \bigcup_{A \in \mb A} \mb{Pa}(A)$. Without loss of generality assume
	$\mb Z \cap \mb A' = \emptyset$. Let $\mb A=\mmb(O) \cup  \mb A'$ and $ \mb V'=\mb V-\{ \mb A' \cup \mb Z \cup \set{S} \}$. From the definition of Markov boundary we have $(O \indep \mb V', \mb A', S, \mb Z |  \mmb(O))$. It follows from Decomposition and Weak  Union axioms in Graphoid that $(O \indep  S, \mb Z |  \mmb(O), \mb A')$, hence
	$(O \indep  S, \mb Z |  \mb A)$. We obtain the following for $i=\{0,1\}$:
%
	{ 	\begin{eqnarray}
	\pr(O=o| do(S=i),do(\mb A = \mb a)) &=&  \pr( y | A=\mb a ) \nonumber \\ &&  \hspace*{-2cm}\sum_{ \mb z \in Dom(\mb Z)}     \bigg( \prod_{i=0}^{m} \pr\big(\mb{pa}(X_i)\bigg|   \bigcup_{j=0}^{i-1} \mb{pa}(X_j ), \bigcup_{j=0}^{i-1}x_j  \big) \bigg)  \nonumber \\
	&=&  \pr( y | A=\mb a)  \label{eq:sum}  \noindent
	\end{eqnarray}}
%
	Note that (\ref{eq:sum}) obtained by the fact that each product inside the summation becomes 1 (simply because $\sum_X \pr(X|Y)=1$) This proves the $\mb A$-fairness of $\mc A$. $\mb K$-fairness for each $\mb K \supseteq \mb A$ can be proved in a similar way.
\end{myproof}
% 


	\begin{myproof}  {Corollary}{\ref{col:fair_learn}}{Without loss of generality, suppose $\mb V=Y\mb D\mb Z \mb W\mb U $ with $\mb X= \mb A \cup \mb Z$ and $\mb A= \mb W \cup \mb Z$. Since the classifier is trained on $\mb X$, there is a functional dependency $\mb X \fd O$, which implies $(O \indep \mb  Y, \mb W, \mb U |  \mb A,\mb Z)$(1), i.e.,  $\mb X$ forms a Markov blanket for $O$. It is also implied from the assumptions $\pr(Y=1| \mb X=\mb x) \approx \pr(O=1| \mb X=\mb x)$ and  $ (Y \indep \mb X-\mb A  | \mb{A}\cap X )$ that $ (O \indep \mb A | \mb Z)$ approximately holds (2). By applying the Contraction axiom in Graphoid to (1) and (2), we obtain  $ (O \indep Y \mb A, \mb  W, \mb U  | \mb Z)$ i.e., $\mmb(O) \subseteq \mb A$. Therefore, $\mc A$ is justifiably fair according to Theorem~\ref{theo:suff_jf}. This completes the proof of part (a). Part (b) is implied from  part(1), definition of Markov boundary and Decomposition axiom in Graphoid.}
\end{myproof}
%\proof[ Proof of Corollary \ref{cor:mb_fair}]{ From the definition of Markov Boundary and the Decomposition axiom it is implied that for any $\mb W \subseteq \mb{V}-\mb{D}-\{Y\} $, 	 $Y \indep \mb W |\mb{D}$.  Thus both requirements inTheorem	\ref{theo:fair_learn} are satisfied.}


%\proof[Proof of Lemma~\ref{lema:bag_set}]{ Construct $D'$ from $D$ as follow: for each tuples $t \in D$ with multiplicity $m$, we insert a set of tuples $(i,t)$ for $i=0,m$ in $D'$. Now, if $D' \models \mb X \indep \mb Y \cup \set{K}| \mb Z)$ then according to the Decomposition axiom (cf.Eq~\ref{ax:dec}) $ D' \models \mb X \indep \mb Y| \mb Z$, thus $ D \models \mb X \indep \mb Y| \mb Z$. The other direction is trivial.
%}




%\proof{ To show the first part, i.e., if $\mb A$ is justifiably fair then $(S \indep O | \mb A, \mb{Des}(\mb A),\mb W)$. It is sufficient to show that there exists  $\mb W \subseteq \mmb(O)$ such that $\mb A \cup \mb{Des}(\mb A) \cup \mb W$ d-separates $S$ and $O$. Note that If $\mc A$ is justifiably fair then it follows from Corollary~\ref{cor:jfcd} that 	all directed paths from $S$ to $O$ are intermediated by $\mb A$.  Also note that under faithfulness assumption Markov Boundary of $O$ consists of its children, parent and parents of its children, hence,   $\mb{Pa}(O) \subseteq \mmb(O)$. It is clear that conditioning on $\mb A$ closes all directed paths from $S$ to $O$.   However, $\mb A \cup \mb{Des}(\mb A)$ may also be a collider node in some path between $S$ and $O$, hence conditioning on $\mb{Pa}(O) \subseteq \mmb(O)$ may open those paths.  It is clear that those path can be closed by further conditioning on an appropriate  subset of the Markov boundary of $O$. In addition, confounding paths between $S$ and $O$ can be clothes by conditioning on a subset of the parents of $O$. Thus clearly, $\mb{Pa}(O) \cup \mb A$ d-separates $S$ and $O$. Now suppose a variable $ V \in \mb{Pa}(O)$ is in $\mb{Des}(\mb N)$ but not in $\mb{A}$, then one of the following holds: either all path between $\mb N$ to $O$  are  intermediated by $\mb A$, or all paths from $S$ to $N$ are intermediated by $\mb A$, because otherwise the algorithm is not justifiably fair., Hence $V \in  \mb{Des}(\mb A)$.  This complements the proof of the first part. The second part implied  from the first part and the correspondence between d-septation and conditional independence in faithful distributions.}

\begin{prop}  \em \label{prop:deg}Given a \fairapp $(\mc A, S, \mb A, \mb I)$, suppose the probability distribution of $\mc A$ is faithful to the causal DAG.  Then, the application is justifiably fair iff $\delta(S;O| \linebreak \mb  \mmb(O) \cap \mb A)=1$.
\end{prop}


\begin{myproof}{Proposition}{\ref{prop:deg}} 
It is easy to see $\delta(S;O|  \mb \mmb(O)$ $\cap \mb A)=1$ iff  $S \indep O|  \mb   \mmb(O) \cap \mb A$. Under the faithfulness assumption, we obtain  $\mmb(O) \cap \mb A$ and d-separates $S$ and $O$. Hence, all directed paths from $S$ to $O$ go thorough $\mb  \mmb(O) \cap \mb A$. Therefore, the algorithm is justifiably fair according to Theorem \ref{th:jfcd}. The converse is immediate from the  natural assumption that $O$ does not have any descendants in the causal DAG; hence, its Markov boundary consists of the algorithm's inputs.
\end{myproof}

\begin{myproof}{Proposition}{\ref{prop:min_rep_lin}} 
	The proposition follows from three facts, all easily verified. (1)
	$D \subseteq \hb$, (2) $\hb$ satisfies the MVD $\mb Z \mvd \mb X$,
	and (3) If two databases $D_1, D_2$ satisfy the MVD then so does
	$D_1 \cap D_2$.  Indeed, the three facts imply that, for any repair
	$D'$, the database $\hb \cap D'$ is also a repair and
	$|\Delta(D, \hb \cap D')| \leq \Delta(D, D')|$, hence, if $D'$ is a
	minimal repair, then $D' \subseteq \hb$.
\end{myproof}


==> Capuchin(Pre-print) (1)/conc.tex <==
\vspace*{-0.1cm}
\section{Conclusions and Future Work}

\ignore{We considered a causal approach for fair ML, reducing it 
to a database repair problem.  We showed that conventional  associational and causal fairness metrics can over- and under-report discrimination.  We defined a new notion of fairness, called  as  {\em justifiable fairness},
that addresses shortcoming of the previous definitions and arguably the strongest notion of fairness that is testable from data. We then proved sufficient properties
for justifiable fairness and use these results to 
translate the properties into saturated conditional independences
that we can be seen as multivalued dependencies  with which to repair the data. We then propose multiple algorithms for implementing these repairs.  Our experimental results show that our algorithms not only outperform state-of-the-art
pre-processing approaches for fairness on our own metrics, but that they are also competitive with existing approaches on conventional metrics. We empirically show that our methods are robust to unseen test data.}


We considered a causal approach for fair ML, reducing it 
to a database repair problem.  We showed that conventional fairness metrics,
including some causal approaches, 
%Sandy:  Replace "end up" with "become" in following clause?
end up as variants of statistical parity
due to the assumptions they make, and that all associational metrics can over-
and under-report discrimination due to statistical anomalies such as Simpson's Paradox.

Instead, we make explicit the assumptions for admissible
variables --- variables through which it is
permissible for the protected attribute to influence the outcome. We use these assumptions to define a new notion of fairness
and to reason about previous definitions.  We then prove sufficient properties
for fairness and use these results to 
translate the properties into saturated conditional independences
 that we can interpret as multivalued dependencies  with which to repair the data. We then propose multiple algorithms for implementing these repairs by casting the problem in 
terms of Matrix Factorization and MaxSAT. 

Our experimental results show that our algorithms not only outperform state-of-the-art
 pre-processing approaches for fairness on our own metrics, but that they are also competitive with existing approaches on conventional metrics. We empirically show that our methods are robust to unseen test data.
   Our results represent an initial attempt to link the language of causality with  database dependencies. 
 
   In future work, we aim to study the effect of training databases that are non-representative of the underling population on our results.
Currently, our proofs assume that the classifier approximates the true distribution, which 
is a common assumption in the machine learning literature.  However, another important source of discrimination  is selection bias or non-representativeness, which we must also correct.  Our
methods do correct for these forms of bias empirically, but we aim to prove bounds on the fairness
metrics based on divergence between training data and test data.


==> Capuchin(Pre-print) (1)/discussion.tex <==
\vspace*{-0.25cm}
\section{Discussion}
\label{sec:diss} 
%\vspace*{-0.65cm}
\reva{
  \paragraph*{\bf Generalizability to Unseen Test Data} In the
  following we briefly discuss the generalizability of the proposed
  repair algorithm to unseen test data.  Recall that the bag $B$
  represents the training data, $B'$ its repair, and let $T$ be the
  unseen test data.  We prove the following in Appendix~\ref{app:proof}:


  \begin{lemma} \label{prop:gen}  If the repaired data satisfies
    $(Y \indep S,\mb I|_{\pr_{B'}} \mb A)$ and the unseen test data
    satisfies $\pr_T(s,\mb i|\mb a) = \pr_{B'}(s,\mb i|\mb a)$, then
    the unseen test data also satisfies
    $(Y \indep S,\mb I|_{\Pr_T} \mb A)$
  \end{lemma}

  % \begin{lemma} \label{prop:gen} Given empirical distributions
  %   $\Pr_B$ and $\Pr_T$ obtained from i.i.d samples of a population
  %   $\Pr_P$ and a fairness application $(\mc A,$ $S, \mb A, \mb I)$,
  %   suppose $\mc A$ is a sensible classifier trained on $B'$, a
  %   repair of $B$ w.r.t. the CI $(Y \indep S,\mb I| \mb A)$, and
  %   tested on $\Pr_T$, then it holds that
  %   $(Y \indep S,\mb I|_{\Pr_T} \mb A)$ if
  %   $\pr_T(s,i|a) = \pr_{B'}(s,i|a) $.
  % \end{lemma}

  The goal of  repair is precisely to satisfy
  $(Y \indep S,\mb I|_{\pr_{B'}} \mb A)$, hence the classifier trained
  on the repaired data $B'$ will be justifiable fair on the test data
  $T$ provided that $\pr_T(s,\mb i|\mb a) = \pr_{B'}(s,\mb i|\mb a)$.
  It is generally assumed that the test and training data are drawn
  from the same distribution $\pr$.  By the law of large numbers, the
  empirical distribution of i.i.d samples of size
  $N\rightarrow \infty$ converges to $\pr$, hence $\pr_T=\pr_B$ in the
  limit.  Therefore, the algorithm will be justifiable fair on the
  test data, provided that the repair is done such that
  $\pr_B(s,\mb i| \mb a) = \pr_{B'}(s,\mb i |\mb a)$. This condition
  is satisfied by the IC repair method which simply repair data by coupling marginal distributions, because it holds by
  construction that
  $\pr_{B'}(y,s,\mb i,\mb a) = \pr_{B}(y,\mb a)\pr_{B}(s,\mb i,\mb
  a)/\pr_{B}(\mb a)$.   In contrast, the condition is only
  approximately satisfied by the MaxSAT and MF approaches, translating
  to slightly weaker fairness guarantees on unseen test data.  Nevertheless, we
  empirically show in Sec~\ref{sec:exp} that MaxSAT and MF approaches
  maintain a significantly better balance between accuracy and fairness. We note that our repair methods can be naturally extended to repair both training and test data for stricter fairness grantees, we consider this extension as future work.
%I think we can let the experiments section state this, now that we've planted the seed that they're different -Luke
\ignore{Specifically, IC radically changes the empirical distribution for sparse data, which negatively impacts the accuracy of the ML algorithms and usability of data.}
%I think that these are good notions for future work, but since we are hurting for space they don't feel
%important to me to bring up here -Luke
\ignore{We note that the condition established in Lemma\ref{prop:gen} can be fed into the MaxSAT
and MF approaches as a constraint, which we defer to future work.
We also note that our repair methods can be naturally extended to repair both training and test data, we consider this extension as future work.}
\vspace*{-.2cm}	\ }

\revb{
  \paragraph*{\bf  Scalability}  As shown in Sec~\ref{sec:repdata}, repairing data w.r.t. a single CI  is an NP-complete problem.
	Therefore, the scalability of our proposed repair methods is equal to that of MaxSAT solvers and approximation algorithms for matrix factorization.
	However, our repair problem is embarrassingly parallel and can be scaled to large datasets by partitioning data into small chunks formed by the conditioning set (see Sec~\ref{sec:experi}).
	In this paper we focused on a single CI, which suffices for many real world fairness applications. We leave the natural extension to future work.
  %Specifically, to maintain the accuracy the repair method should ensure that the joint distribution of  $\pr_B'(y, s,i,a)$ is close to $\pr_{B'}(y,s,i,a)$.
}

%\subsection{Scaling up by partitioning and parallelizing}


%\paragraph{\bf Weighting schemes}


==> Capuchin(Pre-print) (1)/experiment.tex <==







%\subsection{Related Work}
%label{sec:rw}




%Moreover, it is unclear how to enforce such notion of fairness in the context of classification algorithms  through preprocessing data, which is the focus of this paper. \cite{feldman2015certifying,calmon2017optimized}, in-processing \cite{kamishima2012fairness,pmlr-v54-zafar17a,calders2010three,nabi2018fair,kilbertus2017avoiding} and post-processing approaches \cite{hardt2016equality,pmlr-v65-woodworth17a}.

%In contrast in  Sec.~\ref{sec:fair_enforce} we show that our definition of fairness leads to a natural procedure for preventing observational discrimination in classification algorithms. We empirically show that our method has practical fairness guaranties even if the underling causal DAG is not known.  In addition, in Sec~\ref{sec:cvs}, we show that our definition of fairness encompass and generalizes the exiting statistical definition of fairness.
%\paragraph*{\bf Connection to common statistical notions of fairness}


%\ignore{Specifically, \cite{kilbertus2017avoiding} partitions the set of variables that are descendant of a protected attribute into {\em resolving} and {\em non-resolving} variables, where resolving variables are those  that are influenced by $S$ in a manner that we accept as nondiscriminatory. They further define that a variable $V$ exhibits {\em unresolved discrimination} if there exists a directed path from $S$ to $V$ that is not intermediated by a resolving variable and $V$ itself is non-resolving. The require }

\begin{table}[] \centering
	\begin{small} 
		\begin{tabular}{@{}lrrrrrrrrr@{}}\toprule
			{Dataset} & {Att. [$\#$]} & {Rows[$\#$]} &  IC & MF &  MS(H.) &  MS(S.)   \\ \midrule
			\textbf{Adult}~\cite{adult} & 10 & 48k & 12  & 20& 40 & 30 \\ \hdashline
			\textbf{\nipsadult}~\cite{NIPS2017_6988} & 4 & 48k & 2  & 3& 20  & NA \\ \hdashline
			\textbf{COMPAS}~\cite{larson2016we}& 7  & 7k & 2 &3 &7 & 8\\ \hdashline
			\textbf{\nipscompas}~\cite{NIPS2017_6988}& 5  & 7k & 2 &3 &9 & NA\\ \hdashline
		\end{tabular}
	\end{small}
	\caption{      \textmd{ Runtime in seconds for  experiments in Sec.~\ref{sec:extendtoend}.}}
	\label{tbl:data}
\end{table}


%https://tex.stackexchange.com/questions/112343/beautiful-table-samples
\vspace{-0.2cm}
\section{Experimental Results}
\label{sec:exp}
%note: repair for particular contexts


\label{sec:experi}
%We implemented \sys\, in Python to use it
%as a standalone library.
This section presents experiments that evaluate the feasibility and
efficacy of \sys.  We aim to address the following questions.
{\bf Q1}: What is the end-to-end performance of \sys\ in terms of utility and fairness, with respect to our different algorithms?
{\bf Q2}: To what extent are the repaired datasets modified by the repair process of \sys?
{\bf Q3}: How does \sys\ compare to state-of-the-art pre-processing methods for enforcing fairness in predictive classification algorithms? \revd{Table~\ref{tbl:data} reports the running time of the repair algorithms.}

%{\bf Q4:} What is the efficacy of the proposed optimization techniques?



\subsection{Degree of Discrimination}
\label{sec:rod}

%\dan{I moved it here from sec. 3.  Please check it's in the right	place.  Also, shorten the text.}

To assess the effectiveness of the proposed approaches, we next propose a metric that quantifies the degree of discrimination of a classification algorithm.

If we have access to the causal DAG, we could directly compute the {\em degree of interventional discrimination}
of an algorithm: given admissible variables $\mb A$,
for each $\mb K \supseteq \mb A$, compute the ratio of the LHS and RHS of Eq.~\ref{eq:cfair}
using Theorem~\ref{theo:af}, and average the
results.
However,  in many practical
settings we must make judgments about the fairness of an algorithm whose inputs are unknown and
	that may access information that is not even available in the dataset.  We cannot assume access
to an underlying causal DAG in these situations.
For example, in
the case of COMPAS, the recidivism prediction tool, it has been
hypothesized that the algorithm is truly racially discriminatory
\cite{larson2016we}; \sys\ confirms this in Sec~\ref{sec:extendtoend}. %since the bias persists even after applying various transformations designed to eliminate discrimination. \babak{I am not sure what transformations means here}
However, the algorithm itself
is not available to determine which inputs were used and how they might relate.
%Another choice might be to infer the causal DAG from the data itself, but it is known that  discovery of the full structure of a causal DAG is not possible from observational data  \cite{spirtes2000causation,pearl2009causality}.
Instead, we propose a new metric for discovering evidence of potential
discrimination from data that uses the causal framework we described but is
still applicable in situations where all we know is which attributes in the Markov boundary of $O$  are admissible.

\begin{definition} \em Given a\fairapp
	$(\mc A,$ $S, \mb A, \mb I)$, let $\mb A_b=\mmb(O)- \mb I$. We quantify the {\em  ratio of observational discrimination (ROD)} of  $\mc A$ against $S$  in a context $\mb A_b=\mb a_b$ as $\delta(S;O| \mb a_b) \defeq  \frac{\pr(O=1|S=0, \mb a_b) \pr(O=0|S=1 , \mb a_b)}{\pr(O=0|S=0, \mb a_b) \pr(O=1|S=1,  \mb  a_b)}$.
\end{definition}
%
%Note that ROD can be naturally extended to non-binary protected attributes by comparing all pairs of groups. Also note that $\delta(S,O|\mb D)$ can be estimated from data by applying common conditional probability estimation methods such as matching and subclassifications or incorporating modeling assumptions (see ~\cite{loux2017comparison} for a review).
%
Intuitively, ROD calculates the effect of membership in a protected group on the odds of the positive outcome of $\mc A$ for subjects that are similar on $\mb A_b=\mb a_b$ ($\mb A_b$ consists of admissible attributes in the Markov boundary of the outcome).
If $\delta(S;O| \mb a_b)=1$ , then there is no observational evidence that $\mc A$ is discriminatory toward subjects with similar characteristics $\mb a_b$. If  $\delta(S;O| \mb a_b)>1$, then the algorithm potentially discriminates against the protected group, and vice versa if $\delta(S;O| \mb a_b)<1$. ROD is sensitive to the choice of a context $\mb A_b=\mb a_b$ by design. The overall ROD denoted by $\delta(S,O|\mb A_b)$ can be computed by averaging $\delta(S,O|\mb a_b)$  for all $\mb a_b \in \mb A_b$. For categorical data, standard methods in {\em meta analysis} for computing {\em pooled odds ratio} and assessing statistical significance can be applied (see~\cite{chang2017meta,loux2017comparison}). It is easy to see for faithful distributions that ROD=1 coincides with justifiable fairness (see Prop~\ref{prop:deg} in the Appendix~\ref{app:proof}).
%Sandy:  mention appendix number above?

%We immediately obtain the following relation between ROD and justifiable fairness.
\vspace*{-0.3cm}
\subsection{Setup}
\label{sec:setup}
The datasets used for experiments are listed in Table~\ref{tbl:data}.
We implemented our MaxSAT encoding algorithm in Python. For every instance of the input
data, our algorithm constructed the appropriate data files in WCNF format. We used the
Open-WBO~\cite{martins2014open} solver to solve the weighted MaxSAT instances.
%
%\paragraph*{Datasets}

%\bill{Add a table with four entries: Adult, COMPAS, binned Adult, binned COMPAS.  The table can have four columns: name, rows, variables, references where it is used.  Need to make it clear that Fig 7 and 8 are DIFFERENT datasets than Fig 12 and 13.}

%\paragraph*{Classifiers}
We report the empirical utility of each classifier using Accuracy (ACC) = $\frac{TP+TN}{TP+FP+FN+TN}$ via 5-fold cross-validation.  We evaluate using three classifiers: Linear Regression (LR), Multi-layer Perceptron (MLP), and Random Forest (RF).  We selected LR and RF for comparison with Calmon et al.~\cite{NIPS2017_6988}.  We added MLP because it was the highest accuracy method out of ten alternative methods tested on the original (unrepaired) data.  We do not report on these other methods for clarity.

%The only other classifier that offered competitive accuracy was AdaBoost, but it was found to be prohibitively slow.

%the utility and fairness of \sys's repair methods on the following classifiers: the Logistic Regression (LR),  Multilayer Perceptron (MLP) neural network and Random  Forest (RF). The empirical accuracy of the classifiers was then measured by Accuracy (ACC) = $\frac{TP+TN}{TP+FP+FN+TN}$  using 5-fold cross-validation.

%\paragraph*{Fairness Metrics}
We evaluated using the fairness metrics in Table~\ref{tab:expmetrics}. For computing these metrics, conditional expectations were estimated as prescribed in  \cite{salimi2018bias}. We used standard techniques in meta-analysis to compute the pooled odds ratio \cite{chang2017meta}, and its statistical significance, needed to compute ROD. Specifically, we reported the p-value of the ROD, where the null hypothesis was ROD=1; (low p-values suggest the observed ROD is not due to random variation). We combined the p-values from cross-validation test datasets using Hartung's method \cite{hartung1999note}; p-values were dependent due to the overlap in cross-validation tests.  We normalized ROD between 0 and 1, where 0 shows no observational discrimination. We reported the absolute value of the averages of all metrics computed from each test dataset, where the smaller the value, the less the discrimination exhibited by the classifier.

\begin{table*} \centering
\begin{tabular}{ll}
\toprule
\textbf{Metric}    & \textbf{Description} and \textbf{Definition}\\
\midrule
ROD      & \begin{tabular}[c]{@{}l@{}}Ratio of Observation Discrimination:\\ (See Sec.\ref{sec:rod})\end{tabular} \\
\hdashline
DP       & \begin{tabular}[c]{@{}l@{}}Demographic Parity: \\ $Pr(O=1 | S=1) - Pr(O=1 | S=0)$\end{tabular}                                          \\
\hdashline
TPB     & \begin{tabular}[c]{@{}l@{}}True Positive Rate Balance: \\ $Pr(O=1 | S=1,Y=1) - Pr(O=1 | S=0, Y=1)$\end{tabular}                         \\
\hdashline
TNB     & \begin{tabular}[c]{@{}l@{}}True Negative Rate Balance:\\ $Pr(O=0 | S=1, Y=0)-Pr(O=0 | S=0, Y=0)$\end{tabular}                           \\
\hdashline
CDP      & \begin{tabular}[c]{@{}l@{}}Conditional Statistical Parity:\\ $\E_{\mb a}[Pr(O = 1|S = 1, \mb a) - Pr(O = 1|S = 0, \mb a)]$\end{tabular}                \\
\hdashline
CTPB    & \begin{tabular}[c]{@{}l@{}}Conditional TPRB:\\ $\E_{\mb a}[Pr(O = 1|S = 1,Y = 1, \mb a) - Pr(O = 1|S =0, Y=1, \mb a)]$\end{tabular}                      \\
\hdashline
CTNB    & \begin{tabular}[c]{@{}l@{}}Conditional TNRB: \\ $\E_{\mb a} [\Pr(O=0|S=1,Y=0,\mb a)-\Pr(O=0|S=0, Y=0,\mb a)]$\end{tabular}              \\
\hdashline
\end{tabular}
\caption{\textmd{Fairness metrics used in our experiments.}}
\label{tab:expmetrics}
\end{table*}

%\vspace*{-0.1cm}
%\end{minipage}
%\begin{minipage}{0.3\textwidth}
% \begin{tabular}{ll}
%Feldman  & Feldman et al.~\cite{feldman2015certifying} \\
%\hline
%Calmon   & Calmon et al.~\cite{NIPS2017_6988}  \\
%%\hline
%MD       & Capuchin via Matrix Decomposition  \\
%\hline
%IC       & Capuchin via Independent Coupling \\
%\hline
%MS(Hard) & Capuchin via MaxSAT, strong enforcement \\
%\hline
%MS(Soft) & Capuchin via MaxSAT, strong enforcement
% \end{tabular}
%\end{minipage}


%Given a binary sensitive attribute $S$, outcome of classifier $O$, true labels $Y$ and a set of admissible variables $\mb A$, we reported the following fairness metrics: Ratio of Observation Discrimination (ROD) defined in this paper (cf. Sec.~\ref{sec:counter_fair});
%Demographic Parity (DP): $\Pr(O=1|S=1)-\Pr(O=1|S=0)$; true positive rate balance (TPRB): $\Pr(O=1|S=1,Y=1)-\Pr(O=1|S=0, Y=1)$; TN rate balance (TNRB): $\Pr(O=0|S=1,Y=0)-\Pr(O=0|S=0, Y=0)$;  In addition, we reported the expected DP, TPRB and TNRB within subpopulations that are homogeneous on the admissible variables $\mb A$.  Specifically, we measured: Conditional DP (CDP): $\E_{\mb a} [\Pr(O=1|S=1, \mb a)-\Pr(O=1|S=0,\mb a)]$; Conditional TPRB (CTPRB): $\E_{\mb a} [\Pr(O=1|S=1,Y=1,\mb a)-\Pr(O=1|S=0, Y=1,\mb a)]$; Conditional TNRB (CTNRB): $\E_{\mb a} [\Pr(O=0|S=1,Y=0,\mb a)-\Pr(O=0|S=0, Y=0,\mb a)]$. % In addition to ROD, we measure the  conditional mutual information $I(O; \mb V-\mb A|  \mb A)$.  It is clear that $I(O; \mb V-\mb A|  \mb A)=0$ iff $\mmb(O)=\mb A$. %Therefore, the classifier is justifiably fair if $I(O; \mb V-\mb A|  \mb A)=0$. If $\mmb(O) \subseteq \mb A$ then it is also implied that $\delta(S;O| \mb A)=1$. \babak{to be revised}



%\paragraph*{MaxSAT}


%\paragraph*{System} The experiments were performed locally on a 64-bit OS X machine with an Intel Corei7 processor (16 GB RAM, 2.8 GHz). \babak{Add Dragon specifications}




%\begin{figure*}[t!]
%	\includegraphics[scale=0.3]{fig/bias.pdf}
%	\caption{Results of the experiments.}
%	\label{fig:graphs2}
%\end{figure*}

\begin{figure}
	\begin{subfigure}[t]{1\textwidth} \centering
		\hspace*{-1cm}		\includegraphics[scale=0.15]{bias_adult_sex_MLP.pdf}
		\includegraphics[scale=0.15]{bias_compas_race_MLP.pdf}
		\includegraphics[scale=0.15]{bias_compas_nips_MLP.pdf}
		\includegraphics[scale=0.15]{bias_adult_nips_MLP.pdf}
\caption{ \textmd{Fairness Comparison of \sys\ for MLP classifier.}}
	\end{subfigure}
		\begin{subfigure}[t]{1\textwidth} \centering
		\hspace*{-1cm}		\includegraphics[scale=0.15]{bias_adult_sex_RF.pdf}
		\includegraphics[scale=0.15]{bias_compas_race_RF.pdf}
		\includegraphics[scale=0.15]{bias_compas_nips_RF.pdf}
		\includegraphics[scale=0.15]{bias_adult_nips_RF.pdf}
		\caption{ \textmd{Fairness Comparison of \sys\ for RF classifier.}}
	\end{subfigure}

	\begin{subfigure}[t]{1\textwidth} \centering
		\hspace*{-1cm}		\includegraphics[scale=0.15]{bias_adult_sex_LR.pdf}
		\includegraphics[scale=0.15]{bias_compas_race_LR.pdf}
		\includegraphics[scale=0.15]{bias_compas_nips_LR.pdf}
		\includegraphics[scale=0.15]{bias_adult_nips_LR.pdf}
		\caption{ \textmd{Fairness Comparison of \sys\ for LR classifier.}}
	\end{subfigure}
	\caption{ \textmd{Bias reduction performance  of \sys\ for MLP classifier.}}
		\label{fig:MLPbias}
\end{figure}

\subsection{End-To-End Results}

\label{sec:extendtoend}

In the following experiments, a fairness constraint was enforced on training data using \sys\ repair algorithms (cf. Sec~\ref{sec:repdata}).  Specifically, each dataset was split into five training and test datasets.  All training data were repaired separately using Matrix Factorization (MF), Independent Coupling (IC) and two versions of the MaxSAT approach: MS(Hard), which feeds all clauses of the lineage of a CI into MaxSAT, and MS(Soft), which only feeds small fraction of the clauses.  We tuned  MaxSAT to enforce CIs approximately. We then measured the utility and discrimination metrics for each repair method as explained in Sec~\ref{sec:setup}. For all datasets, the chosen training variables included the Markov boundary of the outcome variables, which were learned from data using the Grow-Shrink algorithm \cite{margaritis2003learning} and permutation  \cite{salimi2018bias}. 
%
%
%
%
%
%
%

%
%





{\bf Adult data.} Using this dataset, several prior efforts in algorithmic fairness have reported  gender discrimination based on a strong statistical dependency between income and gender in favor of males \cite{luong2011k,vzliobaite2011handling,tramer2017fairtest}. However, it has been shown that Adult data is inconsistent \cite{salimi2018bias} because its income attribute reports household income for married individuals, and there are more married males in data. Furthermore, data reflects the historical income inequality that can be reinforced by ML algorithms. %Specifically, its income attribute reports the adjusted gross income as indicated in the individual's tax forms, which depends on filing status (jointly and separately), could be household income.  In fact,  the number of married males in Adult data is almost 8 times greater than married females, and  marriage has a strong positive association with high income (more that 80\% of individuals with high income are married).  Now, suppose a bank builds a ML model using Adult data to predict income of the mortgage applicants, which it uses to make decisions about an applicant's future income. The mentioned inconsistency would lead to a significant gender bias toward female applicants. Furthermore, data reflects the historical income inequality that can be reinforced by ML algorithms in other contexts.
We used \sys\ to remove the mentioned sources of discrimination from Adult data.  Specifically, we categorized the attributes in Adult data as follows: $(\mb S)$ sensitive attributes: gender (male, female); $(\mb A)$ admissible attributes: hours per week, occupation, age, education, etc.; $(\mb N)$ inadmissible attributes: marital status; $(Y)$ binary outcome: high income.  As is common in the literature, we assumed that the potential influence of gender on income through some or all of the admissible variables was fair; {for example, gender influences education and occupation, which in turn influence income, but, for this experiment, these effects were not considered discriminatory.} However, the direct influence of gender on income, as well as its indirect influence on income through marital status, were assumed to be  discriminatory. To remove the bias, we enforced the CI  $(Y \indep \mb S, \mb N| \mb D)$ on training datasets using the \sys\ repair algorithms. Then, we trained the classifiers on both original and repaired training datasets using the set of variables $ \mb A \cup \mb N \cup \mb S$. We also trained the classifiers on original data using only $\mb A$, i.e., we dropped the sensitive and inadmissible variables.


\begin{figure}[htbp]  \centering
	\begin{subfigure}{0.7\textwidth} 
	\hspace*{-.9cm}		\includegraphics[scale=0.5]{adult.pdf}
	\end{subfigure}
	\caption{\textmd{Performance of \sys\ on Adult data.}}
				\label{fig:adult}
\end{figure}


Fig.~\ref{fig:adult} compares the  utility and bias of \sys\ repair methods on Adult data.  As shown, all repair methods successfully reduced
the ROD for all classifiers. As shown in Fig.~\ref{fig:MLPbias}, the repaired data also improved associational fairness measures: the \sys\ repair methods had an effect similar to dropping the sensitive and inadmissible variables completely, but they delivered much higher accuracy (because the CI was enforced approximately).   {The residual bias after repair was expected since: (1) the classifier was only an approximation, and (2) we did not repair the test data.   However, as shown in most cases, the residual bias indicated by ROD was not statistically significant. This shows that our methods are robust (by design) to the mismatch between the distribution of repaired data and test data.}  These repair methods delivered surprisingly good results: when partially repairing data using the MaxSAT approach, i.e, using MS(Soft), almost 50\% of the bias was removed while accuracy decreased by only 1\%. We also note that the residual bias generally favored the protected group (as opposed to the bias in the original data). % in this paper we do not distinguish the two cases, though we acknowledge that practical applications typically will. \bill{Seems like if we have better results distinguishing protected vs. privileged, we could report them.}  Recall that fairness metrics shown in Fig.~\ref{fig:endtoend1} were absolute values. See Fig\ref{fig:extendtoendextra} for the original values of the fairness metrics.

\begin{figure}[htbp] \centering
	\begin{subfigure}{0.7\textwidth}
		\hspace*{-.9cm}	\includegraphics[scale=0.5]{compas.pdf}
	\end{subfigure}	\caption{\textmd{Performance of \sys\ on COMPAS data.}}
\label{fig:compas}
\end{figure}


{\bf COMPAS.}  For the second experiment, we used the ProPublica COMPAS dataset \cite{larson2016we}. This dataset contains records for all offenders in Broward County, Florida in 2013 and 2014. We categorized the attributes in COMPAS data as follows: $(\mb S)$ protected attributes: race (African American, Caucasian); $(\mb A)$ admissible attributes:  number of prior convictions, severity of charge degree, age; \textbf{(Y)} binary outcome: a binary indicator of whether the individual is a recidivist. As is common in the literature, we assumed that it was fair to use the admissible attributes to predict recidivism even though they can potentially be influenced by race, and our only goal in this experiment was to address the direct influence of race. We pursued the same steps as explained in the first experiment. \ignore{we used \sys\ to enforce the CI  $(Y \indep \mb S| \mb A)$. Then, we trained the classifiers on both original and repaired training datasets on $ \mb A \cup \mb S$. We also trained the classifiers on the original data but only on $\mb A$, i.e., we dropped the sensitive variable. }
%The bias is shown for the sensitive attribute race and for MLP classifiers. (We report bias for other classifiers and sensitive attributes in Fig.~\ref{fig:extendtoendextra} in the Appendix.)
Fig.~\ref{fig:compas} compares the bias and utility of \sys\ repair methods to original data.  As shown, all repair methods successfully reduced the ROD. However, we observed that MF and IC performed better than MS on COMPAS data (as opposed to Adult data); see~\ref{sec:rep_metho_com} for an explanation. \ignore{An interesting observation is that the significant DP, TPRB and TNRB values could be explained by the admissible variables. \bill{I didn't get the point of the last sentence} Also} {We observed that in some cases, repair improved the accuracy of the classifiers
on test data by preventing overfitting.}

%



In addition, we used \sys\ to compute the ROD  for the COMPAS score and compared it to the same quantity computed for the ground truth. While we obtained a 95\% confidence interval of $(0.7, 0.9)$ for ROD for ground truth, we obtained a 95\% confidence interval of (0.3,  0.5) for ROD for the COMPAS score (high, low). That is, for individuals with the same number of prior convictions and severity of charges, COMPAS overestimated the odds of recidivism by a factor close to 2. The fact that the admissible variables explain the majority of the association between race and recidivism --- but not the association between COMPAS scores and recidivism --- suggests COMPAS scores are highly racially biased.
%
%





%
%

\subsection{Comparing \sys\ Repair Methods}
\label{sec:rep_metho_com}
To compare  \sys\ repair methods beyond the utility experiments in Sec~\ref{sec:extendtoend}, we compared the number of tuples added and deleted for each method, as well as the bias reduction on training data. Fig~\ref{fig:com_rep} reports these measures for the experiments in Sec~\ref{sec:extendtoend}. Note that all numbers were normalized between 0 and 1, where ROD=1 shows no discrimination.  For Adult data, we tuned the MS approach to repair data only by tuple deletion and compared it to a naive approach that repaired data using lineage expression but without using the MaxSat solver. As shown in Fig~\ref{fig:com_rep}, the MaxSat approach removed up to 80\% fewer tuples than the naive approach. %Note that residual bias after repairing data in IC and MD is due to rounding errors in Algorithm \ref{algo:smi}.




In general, the MaxSAT approach was the most flexible repair method (since it can be configured for partial repairs).  Further, it achieved better classification accuracy, and it balanced tuple insertion and deletion.  {Further, it could be extended naturally to multiple CIs, though we defer this extension for future work.}  In terms of the utility of classification, the MS approach performed better on sparse data in which the conditioning groups consisted of several attributes. Figure \ref{fig:bias-accur} shows that repairing a very small fraction of inconsistencies (i.e., clauses in the lineage expression of the associated CI) in the experiment conducted on Adult data  (Sec~\ref{sec:extendtoend})  led to a significant discrimination reduction. This optimization makes the MS approach more appealing in terms of balancing bias and utility.  However, for dense data, IC and MD performed better. This difference was because the size of the lineage expression grew very large when the conditioning sets of CIs consisted of only a few attributes.


\begin{figure}[ht]  \centering
  \includegraphics[width=.33\linewidth]{bias_adult.pdf}
\hspace*{0.8cm}    \includegraphics[width=.3\linewidth]{rep_adult.pdf}
    \\
      \includegraphics[width=.33\linewidth]{bias_compas.pdf}
  \hspace*{0.8cm}         \includegraphics[width=.3\linewidth]{rep_compas.pdf}
        	\caption{\textmd{Comparison of different repair methods. All methods successfully enforced fairness constraint, but with different ratio of tuple insertion and deletion. On Adult data  MaxSAT outperformed the other methods due to sparsity.}}
	\label{fig:com_rep}
\end{figure}


\begin{figure}[htbp] \centering

	\begin{subfigure}{0.8\textwidth} 
\hspace{1.9cm}	\includegraphics[scale=0.4]{bias-disc.pdf}
	\end{subfigure}
	\caption{\textmd{Bias-utility trade off in MaxSAT approach.Repairing only small fraction of conflicts with the fairness constraint in Adult data significantly reduced discrimination.}}
	\label{fig:bias-accur}
\end{figure}
\begin{figure} \centering
	\begin{subfigure}{0.3\textwidth} \centering
\hspace{-3.3cm}	\includegraphics[scale=0.5]{mul_core.pdf}
		\caption*{(a)}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth} \centering
		\includegraphics[scale=0.5]{sing_core.pdf}
		\caption*{(b)}
	\end{subfigure}
	\caption{\textmd{Speed up achieved (a) by partitioning  and parallel processing  on 128 cores; (b)  by partitioning  on a single core.}}
	\label{fig:opti}
\end{figure}

%Each repair method is associated with different distance functions.

To evaluate the effect of partitioning and parallelizing on different methods, we replicated the experiment in sec~\ref{sec:extendtoend} and partitioned Adult data into several chunks of approximately equal sizes; we then repaired the chunks in parallel on a cluster of 128 cores.  Fig~\ref{fig:opti} shows the achieved speed up; all approaches were parallelizable.
Parallel processing was most appealing for MaxSAT since MaxSAT solvers were much more efficient on smaller input sizes. While partitioning had no effect on MF and IC on  a single-core machine, as shown in  Fig~\ref{fig:opti}(b), it sped up MaxSAT approach on even a single core. \revd{Note that partitioning data into several small chunks does not necessarily speed up the MaxSAT approach, since MaxSAT solver must be called for several small inputs. Hence, performance does not increase linearly by increasing the number of chunks. In general partitioning data into several instance of medium size delivers the best performance.}


%\revd{W3: The experiments do not measure runtime and it is not clear why the approach shows poor scalability above 16 threads.}








\subsection{Comparing \sys\ to Other Methods}
\label{sec:comp}
We compared \sys\  with two reference pre-processing algorithms, Feldman et al.~\cite{feldman2015certifying} and  Calmon et al.~\cite{NIPS2017_6988}. Feldman's  algorithm modifies each attribute so that the marginal distributions based on the subsets of the attribute with a given sensitive value are all equal. \ignore{, but it does not modify training labels.} Calmon's algorithm randomly
transforms all variables except for the sensitive attribute to reduce the dependence between training labels and the sensitive attribute subject to the following constraints: (1) the joint distribution of the transformed data is close to the original distribution, and (2) individual attributes are not substantially distorted. {An example of a distorted attribute in the COMPAS dataset would be changing a felon with no prior conviction to 10 prior convictions.} Individual distortion is controlled for using a distortion constraint, which is domain dependent and has to be specified for each dataset. and every single attribute. Note that both approaches are designed to transform training and test data. 

We used these algorithm only to repair training datasets and compare their bias and utility to \sys. In addition, since the distortion function required in Calmon's algorithm is completely arbitrary,  we replicated the same experiments conducted in \cite{feldman2015certifying} using binned Adult data and binned COMPAS data. We note that the analysis in \cite{feldman2015certifying} was restricted to only a few attributes, and the data was excessively binned to few categories (to facilitate the definition of distortion function). As a result, the bias and utility obtained in this experiment was mismatched with Sec~\ref{sec:extendtoend}. For binned Adult data, the analysis was restricted to age, education and gender. COMPAS data used the same attributes as we used in Sec~\ref{sec:extendtoend}. For both datasets, we assumed all attributes  were admissible; hence, the direct effect of direct effect of the protected attribute to outcome was removed.


\begin{figure}[htbp] \centering
	\begin{subfigure}{0.8\textwidth} 
	\hspace*{-.9cm}\includegraphics[scale=0.5]{adult_fled_nips.pdf}
	\end{subfigure}
	\caption{\textmd{Comparing \sys\ and other methods on Binned Adult data.}}
\label{fig:binnedadult}
\end{figure}

Figs.~\ref{fig:binnedadult} and \ref{fig:binnedcompas}  compares the utility and bias of \sys\ to the reference algorithms. The insights obtained from this experiment follow. For binned Adult data, all methods significantly reduced ROD, even though the goal of Calmon's and Fledman's algorithm is essentially to reduce DP. Similarly, \sys\ reduced DP and other associational metrics as a side effect. However, \sys\ outperformed both methods in terms of utility. Because COMPAS data was excessively binned, the ROD in training labels became insignificant for COMPAS, and accuracy dropped by 2\%. We observe that both reference algorithms enforced DP at the cost of increasing ROD; however, in some cases the introduced bias was not statistically significant. In terms of  utility, all methods of \sys\ (except for MaxSAT) performed better than Feldman's algorithm, and all \sys\ methods outperformed Calmon's algorithm quite significantly. This experiment shows that enforcing DP, while unnecessary, can severely affect the accuracy of a classifier and, even more importantly, introduce bias in sub-populations.




This experiment shows that enforcing DP, while unnecessary, can severely affect the accuracy of a classifier and, even more importantly, introduce bias in sub-populations. In this case, while the overall average of recidivism for protected and privileged groups became more balanced using these approaches, the classifier became unfair toward people with the same number of convictions and charge degrees. We note that the observed bias was toward the majority group. Note that \sys\'s MS approach did not perform well on either of these datasets (as opposed to the original data) because of data density. {Also note that for COMPAS data, \sys\ delivered better overall utility than the original data because, for Calmon's dataset (as opposed to the original data), we observed that dropping race indeed increased the accuracy of both RF and MLP classifiers.}



\begin{figure}[htbp] \centering
	\begin{subfigure}{0.8\textwidth} 
	\hspace*{-.9cm}	\includegraphics[scale=0.5]{compas_fled_nips.pdf}
	\end{subfigure}
	\caption{\textmd{Comparing \sys\ and other methods on Binned COMPAS data.}}
\label{fig:binnedcompas}
\end{figure}


%We also note that unlike the other two methods which distort a huge fractions of record in data, \sys\ only remove and insert few number of attributes. Specifically, our MaxSAT approach






%\subsection{Effectiveness of the Optimization Techniques}


==> Capuchin(Pre-print) (1)/intro.tex <==
\vspace*{-0.1cm}
\section{Introduction}
\label{sec:intro}


In 2014, a team of machine learning experts from Amazon Inc. began
work on an automated system to review job applicants' resumes.
According to a recent Reuters article~\cite{amazonhire2018}, the experimental system
gave job candidates scores ranging from one to five and was trained
on 10 years of recruiting data from Amazon.  However, by 2015
the team realized that the system showed a significant gender bias
towards male over female candidates because of
historical discrimination in the training data.  Amazon edited the system to
make it  gender agnostic, but there was no guarantee that discrimination did not occur through other means, and the project was
totally abandoned in 2017.

Fairness is increasingly recognized as a critical component of machine
learning (ML) systems, which make daily decisions that affect people's lives~\cite{courtland2018bias}.
The data on which these systems are trained reflect institutionalized
discrimination that can be reinforced and legitimized through automation.  A naive (and ineffective) approach sometimes used in practice is to
simply omit the protected attribute (say, race or gender) when
training the classifier. However, since the protected attribute is
frequently represented implicitly by some combination of proxy variables, the
classifier still learns the discrimination reflected in training data.
For example, zip code tends to predict race
due to a history of segregation~\cite{amazonrace2016,selbst2017disparate}; answers to personality
tests identify people with disabilities~\cite{bodie2017law,personalitywsj2017}; and keywords can reveal gender on a resume~\cite{amazonhire2018}.
As a result, a classifier trained
without regard to the protected attribute not only fails to remove discrimination, but it can complicate the detection and mitigation of
discrimination downstream via in-processing or post-processing
techniques~\cite{russell2017worlds,galhotra2017fairness,corbett2017algorithmic,chouldechova2017fair,kusner2017counterfactual,kilbertus2017avoiding,nabi2018fair,Veale:2018:FAD:3173574.3174014}, which we next describe.

% Approaches to reduce or eliminate these sources of bias can be
% categorized as pre-processing (where the data is repaired prior to
% training)\cite{}, in-processing (where the machine learning algorithm
% itself is modified to balance accuracy with fairness)\cite{}, or
% post-processing (where the result of the classifier is adjusted to
% improve fairness)\cite{}. Of these, pre-processing has been considered
% a preferable approach, as a suitably repaired dataset can be used in
% data sharing situations when the classifier is not available or when
% the data provider cannot control which classifiers will be used.
%


%%%%%%%%%%%%%%%%%
%\babak{I suggest using discrimination instead of bias.}
%%%%%%%%%%%%%%%%%


The two main approaches to reduce or eliminate sources of discrimination are summarized in Fig.~\ref{tbl:famla}.
%Sandy: insert figure number above.
The most popular is the in-processing, where the ML algorithm itself is
modified; this approach must be reimplemented for every ML application.
% specific to the ML algorithm sgenerally does not offer a guarantee that underlying discrimination is not reflected in other uses cases. %and generally does not offer a guarantee that discrimination does not happen through other means \bill{what other means are we referring to?}.
The alternative is to process either the training data (pre-processing) or the output of the classifier itself (post-processing).
%Sandy:  Is this called "post-processing"? If so, say so.
%Indeed, some systems
%make adjustments to both training and test data~\cite{NIPS2017_6988}. \bill{Test data is not the output of the classifier. Post=processing is fine.  Modifying tyhe test data to adjust one's evaluation is potentially suspect.}
We advocate for the pre-processing strategy, which is agnostic to the choice of ML algorithm and instead interprets the problem as a database repair task.


% Since they are agnostic to the choice of ML algorithm they are more general yet more challenging.

%
%the two main categories of which define the columns in Fig
One needs a quantitative measure of discrimination  in order to remove  it.
%In order to reduce or remove the bias, one needs a quantitative metric
%of the bias or discrimination.
A large number of fairness definitions have been proposed (see Verma and Rubin for a recent discussion \cite{Verma:2018:FDE:3194770.3194776}),
which we broadly categorize in Fig.~\ref{tbl:famla}. The best-known measures are based on \emph{associative} relationships between the protected attribute
and the outcome.
% e.g., the ratio of accuracy rates or false positive rates between protected and priveleged groups, and variants~\cite{zliobaite2015survey}.
% A common class of sophisticated approaches to  interrogate fairness and quantify discrimination is to
% use an associative relationship between the protected attribute, other
% variables, and an outcome (reviewed in Sec.~\ref{sec:?????}).
For example, Equalized Odds requires that both protected and privileged groups have the same true positive (TP) and false positive (FP) rates.  However, it has been shown that associative definitions of fairness can be mutually exclusive~\cite{chouldechova2017fair} and fail to distinguish between discriminatory, non-discriminatory and spurious correlations between a protected attribute and the outcome of an algorithm~\cite{kilbertus2017avoiding,nabi2018fair,dwork2012fairness}.

%But these metrics often do not distinguish
%between discrimination and spurious correlations between the outcome and
%the protected attribute.

%\bill{Briefly describe NIPS, QII, and/or Scheddeiger paper} \dan{it suffices if we name the best known ones, e.g. false positive rate, etc}.


\begin{example} \em \label{ex:berkeley} In a well-studied case, UC
	Berkeley was sued in 1973 for discrimination against females in
	graduate school admissions when it was found that 34.6\% of females
	were admitted in 1973 as opposed to 44.3\% of males.  It turned out
	that females tended to apply to departments with lower overall
	acceptance rates ~\cite{salimi2018bias}.  When broken down by department,  a slight bias toward female applicant
	was observed, \ignore{the admission
	rates for men and women were approximately
	equal} a result that did not constitute evidence for gender-based discrimination.
	%\bill{This interpretation is a bit dangerous by today's standards. The legal definition is disparate impact, which says that we don't care about how it happened, the school can be liable if one can show that women were accepted at different rates.  This case is of course a bit exceptional, because each department made decisions independently.}
\end{example}

Such situations have recently motivated a search for a more principled measure
of fairness and discrimination based on \emph{causality}
\cite{kilbertus2017avoiding,nabi2018fair,kusner2017counterfactual,galhotra2017fairness,russell2017worlds}. These approaches measure the discriminatory causal influence of the protected attribute on the outcome of an algorithm.
However, they typically assume access to background information regarding the underlying causal model, which is unrealistic in practice.
For example, Kilbertus et al. assume the underlying casual model is provided as a structural equation model~\cite{kilbertus2017avoiding}.
Moreover, no existing proposals describe comprehensive systems for pre-processing data to mitigate causal discrimination.

%So far no algorithms or systems based on these ideas have been described, and no comprehensive framework for reasoning about fairness has been proposed. \dan{the last sentence is too weak.}

This paper describes a new approach to removing discrimination by {\em
	repairing the training data} in order to remove the effect of any inappropriate and discriminatory
causal relationship between the protected attribute and classifier predictions, without assuming adherence to an underlying causal models.
%\bill{the reader won't know what inadmissible means here, or even after the example in the next sentence.  It's totally opaque. The intuition is "variables that define subgroups in which fairness must be enforced" or something.  But that seems contrived.  I think we need a paragraph that uses no jargon whatsoever but attempts to explain the overall idea.  You can't just look at global measures, because sometimes it's just a statistical coincidence.  You have to reason about the counterfactual: what would happen if an individual candidate was male instead of female?  If their outcome changes, there is evidence of bias. But we need to do this carefully: there are some situations in which fairness must be enforced, and others where it need not.  The language of causality gives us an appropriate context in which to reason about thses cases. }
% In this paper, we use counterfactual reasoning as the basis for a new
% system \sys to afford algorithmic transparency and fairness.

\begin{figure*} \centering
	\begin{tabular}{ r|c|c| }
		\multicolumn{1}{r}{}
		&  \multicolumn{1}{c}{Associational}
		& \multicolumn{1}{c}{Causal} \\
		\cline{2-3}
		In-processing& \cite{kamishima2012fairness,pmlr-v54-zafar17a,calders2010three,kilbertus2017avoiding} & \cite{nabi2018fair,kilbertus2017avoiding,russell2017worlds} \\
		(Modify the ML Algorithm) & & \\ \cline{2-3}
		Pre/post-processing  &  \cite{feldman2015certifying,NIPS2017_6988,hardt2016equality,pmlr-v65-woodworth17a} & \sys \\
		(Modify the input/output Data) & & (this paper)\\ 	\cline{2-3}
	\end{tabular}
\caption{       \textmd{ Different categories of fairness aware machine-learning methods, based on whether they work with associations/causal definition and  whether they modifying algorithm/data to enforce fairness.}}
	%	\caption{Different categories of fairness aware machine-learning methods, based on whether they work with associations/causal definition and  whether they modifying algorithm/data to enforce fairness.}
	\label{tbl:famla}
\end{figure*}


Our system, \sys, accepts a dataset consisting of a protected
attribute (e.g., gender, race, etc.), an outcome attribute (e.g.,
college admissions, loan application, or hiring decisions), and a set
of \emph{admissible variables}  through which it is
permissible for the protected attribute to influence the outcome.
For example, the applicant's choice of department in
Example~\ref{ex:berkeley} is considered admissible despite being correlated
with gender.  The system repairs the input data by inserting or removing tuples,
changing the empirical probability distribution to remove the
influence of the protected attribute on the outcome through any
causal pathway that includes inadmissible attributes.
That is, the repaired training data can be seen as a \emph{sample
	from a hypothetical fair world}. We make this notion more
precise in Section \ref{sec:fairdef}.

% \luke{(To address a:D1 below, and since I don't think we mention this story anywhere:) Taken as a whole, this means that classifiers trained on the repaired data learn to make classifications with a measurable increase in fairness, \emph{even when applied to biased test data}}.

%\reva{(D1) The authors constantly move between constraints on a database and properties of a probability distribution. And, they equate frequencies in the database to probabilities. It is not super clear how this affects the results, but definitely this is not right. Just because proportions in a database match, it does not mean one can prove conditional independence in the distribution from which the data were drawn. And, if data were drawn from a distribution with some independence properties, they may not hold strictly (except in asymptotic) in the sample. I am not sure if the authors can rewrite the paper and the definitions while avoiding this problem.}

Unlike previous measures of fairness based on causality~\cite{nabi2018fair,kilbertus2017avoiding,russell2017worlds}, which require the
presence of the underlying causal model, our definition is based solely on
the notion of \emph{intervention}~\cite{pearl2009causality} and can be guaranteed even in the absence of causal models.
The user need only distinguish admissible and inadmissible attributes; we prove that this information is sufficient
to support the causal inferences needed to mitigate discrimination.

We use this \emph{interventional} approach to derive in
Sec.~\ref{sec:fairdef} a new fairness definition, called {\em
	justifiable fairness}. Justifiable fairness subsumes and improves on several
previous definitions and can correctly distinguish fairness violations
and non-violations that would otherwise be hidden by statistical
coincidences, such as Simpson's paradox.  We prove next, in
Sec.~\ref{sec:jfc}, that, if the training data satisfies a simple
saturated conditional independence, then any reasonable algorithm
trained on it will be fair.

Our core technical contribution, then, consists of a new approach to repair
training data in order to enforce the saturated conditional independence that guarantees fairness.
The database repair problem has been extensively studied in the
literature~\cite{DBLP:series/synthesis/2011Bertossi}, but in terms of database
constraints, not conditional independence. In Sec.~\ref{sec:repdata} we first define
the problem formally and then present a new technique to reduce it to a
multivalued functional dependency MVD~\cite{AbiteboulHVBook}.
Finally, we introduce new techniques to repair a dataset for an MVD
by reduction to the MaxSAT and Matrix Factorization problems.

%%% We then design multiple database repair algorithms to correct
%%% these dependencies, proving that any classifier trained on the
%%% repaired data will satisfy our fairness definition, up to typical
%%% representativeness and accuracy assumptions.

%We call our approach \emph{interventional fairness}, and it has two advantages
%over previous causality-based definitions: it is easier to justify
%to end users because it can be translated to fairness among individuals that have the same admissible characteristics
%and allows us to develop a data repair algorithm that
%removes the discrimination from the training data, as oppose to the other causality-based approach which enforce fairness using in-processing  techniques. %\bill{all previous proposals would claim that.}.
% The system also optionally accepts a causal model capturing the
% background knowledge of the causal relationships between the
% attributes, when these relationships are known.  \sys then generates
% a new dataset that removes the influence between the protected
% attribute and the outcome \emph{regardless of the causal pathway
% that this influence takes.}

%We show that interventional fairness subsumes a number of previous
%definitions for fairness as special cases, and describe several
%situations that represent clear fairness violations yet are not
%captured by any of the previous definitions.  Next, we show that
%interventional fairness is related to a collection of multi-valued
%dependencies on the input data, which have been extensively studied in
%the database literature~\cite{AbiteboulHVBook}.  Using this
%connection, we design a data repair algorithm that modifies the
%training data by deleting tuples and/or inserting synthetic tuples,
%and guarantees that the repaired data satisfies interventional
%fairness.
%
% dataset, with the effect of deleting tuples and inserting synthetic
% tuples such that problematic relationships are removed and other
% relationships are preserved.  The new dataset represents a new joint
% probability distribution that exhibits the desired conditional
% independence properties implied by a causal analysis.  This framework
% also allows us to define a new metric for fairness, called
% \emph{\metric}, that captures situations that other approaches ignore,
% and a new family of algorithms called \emph{\fairalgorithm} that can
% produce the desired dataset.   adult valentino2012websites
We evaluate our approach in Sec~\ref{sec:exp} on two real datasets commonly studied
in the fairness literature, the adult dataset \cite{adult} and the COMPAS
recidivism dataset~\cite{valentino2012websites}. We find that our algorithms
not only capture fairness situations other approaches
cannot, but that they outperform the existing state-of-the-art
pre-processing approaches \emph{even on other fairness metrics for
	which they were not necessarily designed}. % \dan{we need list more
%  specifics facts from the experiments and brag about them}
Surprisingly, our results show that our repair algorithms can mitigate
discrimination as well as prohibitively aggressive approaches, such as
dropping all inadmissible variables from the training set, while maintaining
high accuracy.  For example, our most flexible algorithm, which involves
a reduction to MaxSAT, can remove almost 50\% of the discrimination while
decreasing accuracy by only 1\% on adult data.
%Our approach was also able to replicate the previous findings
%that even though the admissible variables explain the majority
%of the association between race and recidivism, the
% COMPAS still overestimated the odds of recidivism by a factor close to 2,
% revealing an extreme racial bias.






% In addition, most previous proposals for measuring and improving fairness evaluate their approach by making adjustments to both the training set and the test set, which is not a realistic situation: the test set is not available during training time in production deployments, and it only used in experimental situations. \bill{need an example here}.

%Fairness research has been shown to relate to questions of algorithmic transparency \cite{qii}: mechanisms to expose and adjust sources of bias that affect fairness can be generalized to show how the relationships in the training data influence outcome decisions\cite{}.
%\dan{to flesh out this paragraph or remove}

% \bill{Need a super simple example}
%such that the relationship using Our framework uses counterfactual reasoning in the following way: (a) It allows reasoning about variables that are not explicitly used by an algorithm yet affect its outcome indirectly via covariatess.  (b) it allows derivation of causal relatinships from observational data, making it applicable in settings where the algorithm is not available or testing is not feasible. (c) It enables our system to distinguish between causal versus spurious correlations between variables and outcome of an algorithm.\bill{These arguments seem a bit vague.}


%But releasing data publicly via open data portals is untenable in many situations: corporate data is encumbered with contractual obligations to protect competitive advantage, datasets may exhibit biases that can reinforce discrimination~\cite{NBERw22776} or damage the accuracy of models trained using them~\cite{mcfarland2015big}, and all transportation data is inherently sensitive with respect to privacy~\cite{demontjoye2013unique}. To enable data sharing in these sensitive situations, we advocate releasing ``algorithmically adjusted'' datasets that \textit{destroy causal relationships between certain sensitive variables} while \textit{preserving relationships in all other cases}.

%In contrast, we prove that the \algorithm algorithm can guarantee \metric on the result for any classifier that satisfies intuitive correctness properties.

%Example of fairness not captured by previous methods:

%Something about sparsity, categorical variables?

%Causal approaches. State of the art is NIPS paper.

%Experiments: State of the art


We make the following contributions:
\begin{itemize}
	\item We develop a new framework for causal fairness that does not require a complete causal model.
	\item We prove sufficient conditions for a fair classifier based on this framework.
	\item We reduce fairness to a database repair problem by linking causal inference to multivalued dependencies (MVDs).
	\item We develop a set of algorithms for the repair problem for MVDs.
	\item We evaluate our algorithms on real data and show that they meet our goals and outperform competitive methods on multiple metrics.
\end{itemize}


%Sandy:  Following can be removed or condensed/inserted into contributions list above.

Section \ref{sec:peri} presents background on fairness and causality, while Section \ref{sec:counter_fair} describes sufficient conditions for
a fair classifier and derives the database repair problem.
In Section \ref{sec:repdata}, we present algorithms for solving the database repair problem and show, in Section \ref{sec:exp}, experimental evidence that our algorithms outperform the
state-of-the-art on multiple fairness metrics while preserving high utility.
%Our system falls into the first category of Fig.~\ref{tbl:famla} and,
%thus, affects only the training data: it is independent of the
%machine learning algorithm used.  Once the data is repaired, learning
%and inference can proceed with no changes.
%Furthermore, the repaired data is guaranteed to satisfy a
%simple fairness definition, namely interventional fairness, which is
%easy to understand and easy to justify to end users.  Finally, unlike
%previous fairness definitions based on causality, we do not require a
%full causal model, instead base our definition on the notion of
%intervention.
%\item Experimental evidence that the \fairalgorithm\ outperforms state-of-the-art fairness pre-processing schemes on most conventional metrics as well as \metric.


%The {\em degree of interventional discrimination} of an algorithm can be computed taking average of either the difference or ratio of RHS and LHS of Eq~\ref{eq:cfair} computed for each context formed by $\mb x$ and $\mb k$. Computing degree discrimination requires the causal DAG to be available to analyst. However, in many practical settings only partial information regarding the underlying  causal DAG might be available. Next, we propose a metric for discovering  potential evidences for discrimination from data, which is applicable to domains in which only information regarding admissible variables is available.

%\babak{we should keep the intro under 2 pages}


==> Capuchin(Pre-print) (1)/macros.tex <==
%\usepackage{anysize}
%\usepackage{geometry}
%\geometry{top=1in, left=1in, right=1in, bottom=1in,footskip=.25in}
%\marginsize{1in}{0.8in}{1in}{1in}%tblr
%\usepackage[showframe,bottom=0.2in,footskip=.25in]{geometry}
%\usepackage[left=1in, right=1in, top=1in]{geometry}
%\newcommand{\cmt}[2]{\textcolor{dkmag}{[#1: #2]}}
%\newcommand{\personname}[1]{\cmt{Personname}{#1}}
%\newcommand{\standout}[1]{\textit{\textcolor{dkmag}{#1}}}
\usepackage{amsfonts}
\usepackage{booktabs}
\usepackage{dsfont}
\usepackage{siunitx}
\usepackage{multirow}
\pagenumbering{arabic}
\usepackage{graphicx}
\usepackage{listings}
\usepackage{commath}
%\usepackage[draft]{hyperref}
\usepackage{epstopdf}
\usepackage{hyperref}
\usepackage{color}
\usepackage{url}
\usepackage{mathtools}
\usepackage{caption}
\usepackage{alltt}
\usepackage{mathrsfs}
%\usepackage{multicol}
%\usepackage{lineno}
\usepackage{float}
\usepackage{subcaption}
%\usepackage{subfloat}
%\usepackage{float}
\captionsetup[subfigure]{labelformat=brace}
%\usepackage[linesnumbered,ruled]{algorithm2e}
%\usepackage{classicthesis}
%\usepackage[a4paper,bindingoffset=0.2in,left=1in,right=1in,top=1in,bottom=1in,footskip=.25in]{geometry}
%\usepackage[left=1in,right=1in,top=1in,bottom=0.5in,footskip=.25in]{geometry}
\usepackage{graphicx,fancyvrb}
\usepackage[colorinlistoftodos]{todonotes}
%\usepackage{algorithm}
\usepackage[linesnumbered,ruled,vlined]{algorithm2e}
\usepackage{algpseudocode}
%\usepackage[bottom=0.8in]{geometry}
%\usepackage{lipsum}
\usepackage{amsmath,amssymb}
%\usepackage{color, MnSymbol} %, hyperref} %wrapfig,
%\usepackage{array,multirow,graphicx,tabularx}
%\usepackage{aliascnt}
%\usepackage{relsize}
%\usepackage{titling}
%\usepackage{fullpage} %,enumitem}
%\usepackage[T1]{fontenc}
%\usepackage{enumitem}
%\usepackage[shortlabels]{enumitem}
%\setlist{nolistsep}
%\setlist[enumerate]{nosep}
\usepackage{booktabs}
\usepackage{caption}
\usepackage{float}
%\usepackage{titlesec}
\usepackage{capt-of}
%\usepackage{footnote}
\usepackage{booktabs}
\usepackage{colortbl}
\usepackage{xcolor}
\usepackage{xfrac}
\usepackage{footnote}
%dashed line
\usepackage{array}
\usepackage{arydshln}
\setlength\dashlinedash{0.2pt}
\setlength\dashlinegap{1.5pt}
\setlength\arrayrulewidth{0.3pt}
%usepackage[T1]{fontenc}
%\usepackage{fontspec}
%\setmainfont[Scale=0.85, Ligatures={Required,Common,Contextual,TeX}]{TeX Gyre Schola} % Incredible font inside latex

%
%\usepackage{fancyhdr}
%\usepackage{fullpage} %, hyperref}
%\usepackage{amssymb, amsmath, enumitem, titling, hyperref}
%\usepackage[standard]{ntheorem}
%%\usepackage[sort&compress]{natbib}
%\usepackage[top=0.65in, bottom=1.2in, left=0.95in, right=0.95in]{geometry}
% %\ifthenelse{\value{page}=1}
%          %{\setlength\headheight{40pt}}
%          %{\setlength\headheight{0pt}}
%
%\usepackage[backend=bibtex,sorting=anyt, maxnames=7, firstinits=true]{biblatex} %hyperref=true,
%\renewcommand*{\bibfont}{\footnotesize}
%\bibliography{bib_rs}
%%\renewcommand{\baselinestretch}{0.9}
\def\sharedaffiliation{%
\end{tabular}
\begin{tabular}{c}}
\usepackage{amsmath,amsfonts,amssymb}
%Spencer
\usepackage{todonotes}
\newcommand{\vset}[1]{\mathbf{#1}}
%\usepackage{amsthm}
%
%\theoremstyle{definition}
%\newtheorem{definition}{Definition}[section]
% end Spencer

\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
	#1\;\delimsize|\delimsize|\;#2%
}
\newcommand{\kld}[2]{\ensuremath{D_{KL}\infdivx{#1}{#2}}\xspace}



\newcommand{\reva}[1]{{ { { #1}}}}
\newcommand{\revb}[1]{{{ { #1}}}}
\newcommand{\revc}[1]{{{{ #1}}}}
\newcommand{\revd}[1]{{{{ #1}}}}
\newcommand{\reve}[1]{{{ { #1}}}}
%\newcommand{\revf}[1]{{{\color{red} {#1}}}}


\definecolor{mygreen}{rgb}{0,0.6,0}
\definecolor{mygray}{rgb}{0.5,0.5,0.5}
\definecolor{mymauve}{rgb}{0.58,0,0.82}
\DeclareMathOperator{\dis}{d}

\lstset{
	breaklines=true,                                     % line wrapping on
	language=SQL,
	frame=ltrb,
	framesep=5pt,
	basicstyle=\normalsize,
	keywordstyle=\color{blue},
	identifierstyle=\ttfamily\color{mygreen}\bfseries,
	commentstyle=\color{Brown},
	stringstyle=\ttfamily,
	emph={count,sum,avg,/},
	emphstyle={\color{red}},
	showstringspaces=ture,
	classoffset=1, % starting new class
	otherkeywords={WITH, VIWE},
	keywordstyle=\color{weborange},
	classoffset=0,
}


\usepackage{listings}
\lstnewenvironment{VerbatimText}[1][]{
    \renewcommand*{\lstlistingname}{Code}
    \lstset{fancyvrb=true,basicstyle=\footnotesize,captionpos=b,xleftmargin=2em,#1}
}{}

\newcommand{\mypm}{\mathbin{\tikz [x=1.4ex,y=1.4ex,line width=.1ex] \draw (0.0,0) -- (1.0,0) (0.5,0.08) -- (0.5,0.92) (0.0,0.5) -- (1.0,0.5);}}%


\newcommand{\qii}{\delta}

\usepackage{booktabs}
\usepackage{pgfplots}
\usepackage{pgfplotstable}

\newcommand{\createcontingencytable}[4]{ %
	% #1=table name
	% #2=first column name
	% #3=new row sum name
	% #4=new column sum name
	\pgfplotstablecreatecol[
	create col/assign/.code={% In each row ...
		\def\rowsum{0}
		\pgfmathtruncatemacro\maxcolindex{\pgfplotstablecols-1}
		% ... loop over all columns, summing up the elements
		\pgfplotsforeachungrouped \col in {1,...,\maxcolindex}{
			\pgfmathsetmacro\rowsum{\rowsum+\thisrowno{\col}}
		}
		\pgfkeyslet{/pgfplots/table/create col/next content}\rowsum
	}
	]{#3}{#1}%
	%
	% Transpose the table, so we can repeat the summation step for the columns
	\pgfplotstabletranspose[colnames from={#2},input colnames to={#2}]{\intermediatetable}{#1}
	%
	% Sums for each column
	\pgfplotstablecreatecol[
	create col/assign/.code={%
		\def\colsum{0}
		\pgfmathtruncatemacro\maxcolindex{\pgfplotstablecols-1}
		\pgfplotsforeachungrouped \col in {1,...,\maxcolindex}{
			\pgfmathsetmacro\colsum{\colsum+\thisrowno{\col}}
		}
		\pgfkeyslet{/pgfplots/table/create col/next content}\colsum
	}
	]{#4}\intermediatetable
	%
	% Transpose back to the original form
	\pgfplotstabletranspose[colnames from=#2, input colnames to=#2]{\contingencytable}{\intermediatetable}
}
%

\PassOptionsToPackage{hyphens}{url}\usepackage{hyperref}
\newcommand{\inp}{{{\mb X }}}
\newcommand{\cm}{{{\mb M }}}
\newcommand{\acm}{{{\mb M_{\mc A} }}}
\newcommand{\cg}{ G}
\newcommand{\acg}{ G_{\mb M_{\mc A}} }

\newcommand{\nipsadult}{{{Binned Adult}}}
\newcommand{\nipscompas}{{{Binned COMPAS}}}

\usepackage{amsmath}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\fge}{{\bf {FGE}}}
\newcommand{\scmit}{{\bf {SNMIT}}}
\newcommand{\cmit}{{\bf {MIT}}}
\newcommand{\icmit}{{\bf {FNMIT}}}
\newcommand{\iscmit}{{\bf {FMIT}}}
\newcommand{\hcmit}{{\bf {HyMIT}}}
\newcommand{\ogsal}{{\bf {OGS}}}
\newcommand{\gsal}{{\bf {GS}}}
\newcommand{\pdal}{{\bf {CD}}}
\newcommand{\delay}{{\tt \textsc{Flight Delay}}}
\newcommand{\ate}{{\tt \textsc{ATE}}}
\newcommand{\nde}{{\tt \textsc{NDE}}}
\newcommand{\nie}{{\tt \textsc{NIE}}}
\newcommand{\E}{{\tt \mathbb{E}}}
\newcommand{\pr}{{\tt \mathrm{Pr}}}
\newcommand{\sys}{{\textsc{Capuchin}}}
\newcommand{\dal}{{{SGS}}}
\newcommand{\bigCI}{\mathrel{\text{\scalebox{1.07}{$\perp\mkern-10mu\perp$}}}}
\newcommand{\nbigCI}{\cancel{\mathrel{\text{\scalebox{1.07}{$\perp\mkern-10mu\perp$}}}}}
\newcommand{\rred}[1]{\textcolor{red}{#1}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\ind}[0]{\textrm{Indep}}
\newcommand{\ignore}[1]{}
\newcommand{\comlb}[1]{{\vspace{2mm}\noindent \rred{\bf COMM(Dan):}}~ #1 \hfill {\bf    END.}\\}
\newcommand{\combabak}[1]{{\vspace{4mm}\noindent \bf  COMM(Babak):}~ {\em \rred{#1}}\hfill {\bf END.}\\}



\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}

\newcommand{\dan}[1]{{{\color{magenta} Dan: [{#1}]}}}
\newcommand{\babak}[1]{{\texttt{\color{red} Babak: [{#1}]}}}
\newcommand{\bill}[1]{{\texttt{\color{olive} Bill: [{#1}]}}}
\newcommand{\luke}[1]{{\texttt{\color{blue} Luke: [{#1}]}}}
\newcommand{\johannes}[1]{{\texttt{\color{blue} Johannes: [{#1}]}}}
\newcommand{\red}[1]{{\textbf {{\color{red} [{#1}]}}}}
\newcommand{\scream}[1]{{\texttt{\color{red}{\textbf{[{#1}]}}}}}

\newcommand{\LOGSPACE}{{\scriptsize $  \mathrm{LOGSPACE}$}}
\newcommand{\NLOGSPACE}{{\scriptsize $  \mathrm{NLOGSPACE}$}}
\newcommand{\PTIME}{{\scriptsize $  \mathrm{PTIME}$ }}
\newcommand{\nindep}{\mbox{$\not\!\perp\!\!\!\perp$}}
\newcommand{\indep}{\mbox{$\perp\!\!\!\perp$}}





\newcommand{\tr}{1} %{\mathtt{t}}
\newcommand{\cn}{0} %{\mathtt{c}}

%infotheo
\newcommand{\rep}{D'}
\newcommand{\icq}{Q_\varphi}
\newcommand{\hb}{D^*}


\newcommand{\satt}{\mathbf{a}}
\newcommand{\att}{\mathbf{A}}
\newcommand{\sx}{\mathbf{x}}
\newcommand{\bx}{\mathbf{X}}
\newcommand{\pn}{\textmd{N}}
\newcommand{\ent}{{\mathcal{H}}}
\newcommand{\minf}{{{I}}}
\newcommand\mvd{\twoheadrightarrow}
\newcommand{\amvd}{\twoheadrightarrow_\alpha}
\newcommand{\fd}{\rightarrow}
\newcommand{\afd}{\rightarrow_\alpha}
\newcommand{\bfd}{\rightarrow_\beta}
\newcommand{\abfd}{\rightarrow_{\alpha+\beta}}
\newcommand{\A}{\texttt{A}}
\newcommand{\K}{\texttt{K}}
\newcommand{\deletelater}[1]{{\textbf {{\color{green} [{#1}]}}}}
\newcommand{\intervrel}{\texttt{intervened-relation}}

\newcommand{\annot}{\texttt{annot}}
\newcommand{\supp}{\texttt{supp}}
\newcommand{\sch}{{\mathcal{S}}}
\newcommand{\rel}{{\mathcal{R}}}
%\newcommand{\interv}{{\Gamma}}
\newcommand{\real}{{\mathbb{R}}}
\newcommand{\nat}{{\mathbb{N}}}
\newcommand{\explattr}{{\{E\}}}
%\newcommand{\change}{{\Delta}}
\newcommand{\bool}{{\textit{b}}}


\newcommand{\AP}{\texttt{AP}}
\newcommand{\highval}{\texttt{high}}
\newcommand{\midval}{\texttt{mid}}
\newcommand{\lowval}{\texttt{low}}
\newcommand{\aplow}{\texttt{poor}}
\newcommand{\aphigh}{\texttt{good}}
\newcommand{\dbnull}{\texttt{null}}
\newcommand{\relset}{\mathcal{R}}
\newcommand{\reltop}{{\mathcal{R}}_{top}}
\newcommand{\relbot}{{\mathcal{R}}_{bot}}
\newcommand{\attrset}{\mathcal{A}}
\newcommand{\attrtop}[1]{{\mathcal{A}}_{{top}, {#1}}}
\newcommand{\attrbot}{{\mathcal{A}}_{bot}}
%\newcommand{\featureset}{\mathcal{B}}
\newcommand{\wcl}{\mathscr{C}(\mb{C})}
\newcommand{\rwq}{{ {\mc{Q}_{rw}}}}
\newcommand{\db}{{D}}
\newcommand{\dbdom}{\mathbf{DB}}
\newcommand{\intervadditive}{{intervention-additive}}
\newcommand{\val}{{v}}
\newcommand{\valorig}{{u}}
%\newcommand{\dbdom}{\mathcal{D}}
\newcommand{\inputclass}{\mathcal{C}}
%\newcommand{\intervene}{\mathcal{I}}
%\newcommand{\tbaff}{{\tt{T_{Aff}}}}
%\newcommand{\attaff}{{\tt{A_{Aff}}}}
\newcommand{\univ}{{{U}}}
\newcommand{\pk}{{\mathtt{pk}}}
\newcommand{\fk}{{\mathtt{fk}}}
\newcommand{\expl}{{\phi}}
%\newcommand{\pk}{{\tt \mathtt{\pk}}}
\newcommand{\sign}{{\tt \mathtt{sign}}}
%\newcommand{\expldom}{{\Phi}}

\newcommand{\select}{\tt {\textsc{Select}}}
\newcommand{\where}{{\tt \textsc{Where}}}
\newcommand{\with}{{\tt \textsc{With}}}
\newcommand{\distinct}{{\tt \textsc{distinct}}}
\newcommand{\groupby}{{\tt \textsc{Group By}}}
\newcommand{\from}{{\tt \textsc{From}}}
\newcommand{\ct}{{\tt \textsc{Count}}}
\newcommand{\create}{{\tt \textsc{Create}}}
\newcommand{\explanation}{{\tt \textsc{Explanation}}}
%\newcommand{\Pr}{{\tt {Pr}}}
\newcommand{\on}{{\tt \textsc{On}}}
\newcommand{\sqlwith}{{\tt \textsc{With}}}
\newcommand{\as}{{\tt \textsc{as}}}
\newcommand{\cascade}{{\tt \textsc{Cascade}}}
\newcommand{\sqland}{{\tt \textsc{And}}}
\newcommand{\sqlin}{{\tt \textsc{In}}}
\newcommand{\true}{{\tt true}}
\newcommand{\false}{{\tt false}}
\newcommand{\inmath}[1]{{\mathtt {#1}}}

\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}
\newcommand{\ie}{{\em i.e.}} %\xspace}
\newcommand{\eg}{{\em e.g.}} %\xspace}
\newcommand{\etal}{{et al.}} %\xspace}
\newcommand{\aka}{{\em a.k.a.}\xspace}
\newcommand{\algorithmicbreak}{\textbf{Break}}
\newcommand{\backwd}{\mathcal{B}}
\newcommand{\mbl}{{\bf B}}
\newcommand{\mmb}{{\bf MB}}
\newcommand{\emb}{{ \bf MB}_\epsilon}
\newcommand{\embl}{{\bf B}_\epsilon}
\newcommand{\emmb}{{\bf IB}_{(\epsilon,\beta)}}
\newcounter{enumQues}
\newcommand{\mf}[1]{\mathrm{\mathfrak{#1}}}
\newcommand{\mb}[1]{{\mathbf{#1}}}
\newtheorem{defn}{Definition}[section]
\newtheorem{rem}[defn]{Remark}
\newtheorem{conj}[defn]{Conjecture}
\newtheorem{example}[defn]{Example}
\newenvironment{myproof}[2] {\paragraph{Proof of {#1} {#2} :}}{\hfill$\square$}
\newtheorem{corollary}[defn]{Corollary}
\newtheorem{lemma}[defn]{Lemma}
\newtheorem{theorem}[defn]{Theorem}
\newtheorem{definition}[defn]{Definition}
\newtheorem{prop}[defn]{Proposition}
\newtheorem{obs}[defn]{Observation}
\newtheorem{assumption}[defn]{Assumption}
\newcommand{\proj}[1]{{\Pi}}
\newcommand{\sel}[1]{{\sigma}}

\newcommand{\un}[1]{{\underline{#1}}}
\newcommand{\ov}[1]{{\overline{#1}}}
\newcommand{\cut}[1]{}
\newcommand{\eat}[1]{}

\newcommand{\causalframework}{interventional fairness}
\newcommand{\metric}{interventional discrimination}
\newcommand{\fairalgorithm}{interventional fairness}

\newcommand{\defeq}{\stackrel{\text{def}}{=}}

\newcommand{\fairapp}{fairness application~}


==> Capuchin(Pre-print) (1)/preli.tex <==

\begin{table} \centering
	\centering
	\begin{tabular}{|l|l|} \hline
		\textbf{    Symbol} & \textbf{Meaning} \\ \hline
		$X, Y, Z$ & attributes (variables)\\
		$\mb{X}, \mb{Y}, \mb{Z}$ & sets of attributes \\
		$Dom(X), Dom(\mb{X})$ & their domains \\
		$x \in Dom(X), \mb{x} \in Dom(\mb{X})$ & a single value, a tuple of values \\
		$D$ & the database instance \\
		$\mb{V}$ & the attributes of the database $D$ \\
$\cm = \langle \mb U, \mb V , \mb F, \pr \rangle$ & Probabilistic Causal Model (PGM) \\
		$\cg$ & causal DAG \\
		$X \rightarrow Y$ & an edge in $\cg$ \\
		$\mb{Pa}(X)$ & the parents of $X$ in $\cg$ \\
		$\mb P$ & a path in $\cg$ \\
		$X \stackrel{*}{\rightarrow} Y$ & a directed path in $\cg$ \\
		$\mb Z \mvd \mb X$ & multivalued dependency (MVD) \\
		$\mb X \indep_{\pr} \mb Y | \mb Z$ or $\mb X \indep \mb Y | \mb Z$ & conditional independence \\
		$(\mb{X} \indep \mb{Y} |_d \ \mb{Z})$ & d-Separation in $\cg$. \\
		$\mmb(X)$ & The Markov boundary of $X$ \\
				$I$ & Inadmissible attributes \\
								$A$ & Admissible attributes \\
		\hline
	\end{tabular}
	\caption{      \textmd{ Notation used in the paper.}}
	\label{tab:notations}
\end{table}
%\frvc{
{
	\section{Preliminaries}
	%}
	\label{sec:peri}
}

%\revc{ W3: Related to W2: I do not like the fact that authors equate empirical frequencies in the data to joint probabilities that the data were drawn from.}

We review in this section the basic background on database repair, algorithmic
fairness and models of causality,  the
building blocks of our paper.

The notation used is summarized in Table~\ref{tab:notations}.  We
denote variables (i.e., dataset attributes) by uppercase letters,
$X, Y, Z, $ $V$; their values with lower case letters, $x,y,z, v$; and
denote sets of variables or values using boldface ($\mb X$ or
$\mb x$).  The domain of a variable $X$ is $Dom(X)$, and the domain of
a set of variables is $Dom(\mb X) = \prod_{Y\in \mb X} Dom(Y)$. In
this paper, all domains are discrete and finite; continuous domains
are assumed to be binned, as is typical.  A {\em database instance} $D$
is a relation whose attributes we denote as $\mb V$.  We assume set
semantics (\ie,\ no duplicates) unless otherwise stated, and we denote
the cardinality of $D$ as $n = |D|$.  Given a partition
$\mb X \cup \mb Y \cup \mb Z= \mb V$, we say that $D$ satisfies the
{\em multivalued dependency} (MVD) $\mb Z \mvd \mb X $ if
$D= \Pi_{\mb X \mb Z}(D) \Join \Pi_{\mb Z \mb Y}(D)$.





Typically, training data for ML is a bag $B$.  We convert it into a
set $D$ (by eliminating duplicates) and a probability distribution
$\pr$, which accounts for
multiplicies;\footnote{$\pr(\mb v) \defeq \frac{1}{|B|}\sum_{t \in
    B}1_{t=\mb v}$.} We call $D$ the support of $\pr$.  We say that
$\pr$ is {\em uniform} if all tuples have the same probability.  We
say $\mb X$ and $\mb Y$ are {\em conditionally independent (CI)} given
$\mb Z$, written $(\mb X \indep_\pr \mb Y | \mb Z)$, or just
$(\mb X \indep \mb Y | \mb Z)$
if $\pr(\mb x| \mb y, \mb z) =\pr(\mb x| \mb z)$ whenever
$\pr(\mb y, \mb z) > 0 $.  Conditional independences satisfy the
Graphoid axioms~\cite{pearl1985graphoids}, which are reviewed in
Appendix~\ref{app:addback} and are used in proofs.  When
$\mb V = \mb X \mb Y \mb Z$, then the CI is said to be {\em saturated}.
A uniform $\pr$ satisfies a saturated CI iff its support
$D$ satisfies the MVD $\mb Z \mvd \mb X$.  Training data usually does
not have a uniform $\pr$, and in that case the equivalence between the
CI and MVD fails~\cite{wong2000implication}; we address this issue in
Sec.~\ref{sec:repdata}.

The {\em database repair problem} is the following: we are given a set
of constraints $\Gamma$ and a database instance $D$, and we need to
perform a minimal set of updates on $D$ such that the new database
$\rep$ satisfies $\Gamma$~\cite{DBLP:series/synthesis/2011Bertossi}.
The problem has been studied extensively in database theory for
various classes of constraints $\Gamma$.  It is NP-hard even
when $D$ consists of a single relation (as it does in our paper)
and $\Gamma$ consists of functional
dependencies~\cite{DBLP:conf/pods/LivshitsKR18}.  In our setting,
$\Gamma$ consists of conditional independence statements, and it
remains NP-hard, as we show in Sec.~\ref{sec:repdata}.




\vspace*{0.1cm}
\subsection{Background on  Algorithmic Fairness}
\label{sec:cvs}




\begin{figure*}  \centering
	\begin{tabular}{|l|l|} \hline
		\textbf{     Fairness Metric}  & \textbf{Description}  \\ \hline
		% \rowcolor{black!20}
		Demographic Parity (DP) \cite{calders2009building}  & $S \indep O$  \\
		a.k.a. Statistical Parity \cite{dwork2012fairness} & \\
		or Benchmarking \cite{simoiu2017problem} & \\ \hline
		%
		Conditional Statistical parity \cite{corbett2017algorithmic} & $S \indep O |\mb A$ \\ \hline
		%
		% \rowcolor{black!20}
		Equalized Odds (EO) \cite{hardt2016equality} \footnotemark[2] & $S \indep O| Y $  \\
		a.k.a.  Disparate Mistreatment  \cite{zafar2017fairness} & \\ \hline
		%
		Predictive Parity (PP)\cite{chouldechova2017fair} \footnotemark[3]  & $S \indep Y| O $  \\
		a.k.a. Outcome Test  \cite{simoiu2017problem} & \\
		or Test-fairness  \cite{chouldechova2017fair} & \\
		or Calibration \cite{chouldechova2017fair}, & \\
		or Matching Conditional Frequencies \cite{hardt2016equality} & \\ \hline
	\end{tabular}  
	\caption{      \textmd{ Common associational definitions of fairness and their conditional independence statement counterparts.}} \label{tbl:asdef}
\end{figure*}




Algorithmic fairness considers a {\em protected attribute} $S$, the
{\em response variable} $Y$, and a prediction algorithm
$A : Dom(\mb X) \rightarrow Dom(O)$, where $\mb X \subseteq \mb V$,
whose prediction is denoted $O$ (some references denote it $\tilde Y$)
and called\ignore{ {\em output} or} {\em outcome}.  For simplicity, we
assume $S$ classifies the population into protected $S=1$ and
privileged $S=0$, for example, female and male.  Fairness definitions
can be classified as associational or causal.

%The goal is to ensure that the algorithm does not discriminate against the protected group.  Many definitions for discrimination (or fairness) have been proposed in the literature~\cite{zliobaitesurvey,arvind} and can be broadly classified into associational and causal definitions; see Fig.~\ref{tbl:famla}.

\paragraph{\bf Associational fairness} is based on statistical measures on the
variables of interest; a summary is shown in Fig.~\ref{tbl:asdef}.
\textit{Demographic Parity} (DP)
\cite{calders2010three,kamiran2009classifying,zemel2013learning,simoiu2017problem,dwork2012fairness}, requires an algorithm to classify both
the protected and the privileged group with the same probability,
$\pr(O=1|S=1)=\pr(O=1|S=0)$. As we saw
in Example~\ref{ex:berkeley}, the lack of statistical parity cannot be
considered as evidence for gender-based discrimination; this
has motivated the introduction of \textit{Conditional Statistical Parity} (CSP)
\cite{corbett2017algorithmic}, which controls for a set of
admissible factors  $\mb A$, i.e.,
$\pr(O=1|S=1,\mb A= \mb a)=\pr(O=1|S=0,\mb A=\mb a)$.  % or equivalently
%$(O \indep S|\mb D)$. 
% \dan{Is a risk factor the same as an admissible  variable?  If so then we should mention this here, it makes it easier to justify admissible variables later.} \babak{yes, the motivation is similar. However, in our language anything that is inadmissible is admissible (it might has nothing to do with S)}In Example~\ref{ex:berkeley}, the risk factor is
%{\em department}. 
 Another popular measure used for predictive
classification algorithms is  \textit{Equalized Odds} (EO), which
requires that both protected and privileged groups to have the same false
positive (FP) rate, $\pr(O=1|S=1,Y=0)=\pr(O=1|S=0,Y=0)$ , and the same
false negative (FN) rate, $\pr(O=0|S=1,Y=1)=\pr(O=0|S=0,Y=1)$ \ignore{, or,
equivalently, $(O \indep S|Y)$.} Finally, \textit{Predictive Parity} (PP)
requires that both protected and unprotected groups have the same
predicted positive value (PPV),
$\pr(Y=1|O=i,S=0)=\pr(Y=1|O=i,S=1) \ \text{for} \ i,=\{1,0\} $. It has been shown that these measures can be mutually exclusive \cite{chouldechova2017fair} (see Appendix \ref{app:addback}).




\paragraph{\bf  Causal fairness \cite{kusner2017counterfactual,kilbertus2017avoiding,nabi2018fair,russell2017worlds,galhotra2017fairness}}
was motivated by the need to address difficulties generated by
associational fairness and assumes an underlying causal model.  We
first discuss causal DAGs before reviewing causal fairness.
%%% The paragraph below was present in the submitted paper:
% {\em Counterfactual
% fairness}~\cite{kusner2017counterfactual,russell2017worlds} requires
% that the distribution of possible predictions for an individual
% remains unchanged when an individual's protected attributes are
% changed; as we explain below, counterfactual fairness, as defined
% in~\cite{kusner2017counterfactual}, is equivalent to conditional
% statistical parity in most cases.  {\em Path-specific causal
% effects} \cite{nabi2018fair,kilbertus2017avoiding} defines fairness
% in terms of the existence of specific causal paths from $S$ to $O$
% that are deemed to be discriminatory.  It is known that path
% specific causality is notoriously difficult to estimate in practice.
% {\em Individual fairness}~\cite{dwork2012fairness} is an appeal of
% causal fairness qthat requires fairness to hold for similar
% individuals.

\subsection{Background on Causal DAGs }

\label{sec:causal:dag}

%For space, I think this is safe to omit. Plus the citation shows up shortly
%hereafter. -Luke
We now review causal directed acyclic graphs (DAGs) and refer the reader
to Appendix \ref{app:addback} and \cite{pearl2009causality} for more details.


\paragraph*{\bf Causal DAG}
A \textit{causal DAG} $\cg$ over set of variables $\mb V$ is a directed acyclic graph that
models the functional interaction between variables in $\mb V$.  Each node $X$ represents
a variable in $\mb V$ that is functionally determined by: (a) its parents $\mb{Pa}(X)$
in the DAG, and (b) some set of \emph{exogenous} factors that need not appear in the DAG,
as long as they are mutually independent.
This functional interpretation leads to the same decomposition of the  joint probability distribution of $\mb V$ that characterizes Bayesian networks \cite{pearl2009causality}:
\begin{align}
\pr(\mb V) = & \prod_{X \in \mb V} \pr(X | \mb{Pa}(X)) \label{eq:bayesian1}
\end{align}



\paragraph*{\bf $d$-Separation and Faithfulness}
A common inference question in a causal DAG is how to determine whether a
CI $(\mb X \indep \mb Y | \mb Z)$ holds.  A sufficient criterion is
given by the notion of d-separation,  a syntactic condition
$(\mb X \indep \mb Y |_d \mb Z)$ that can be checked directly on the
graph.  $\pr$ and $\cg$ are
called {\em Markov compatible} if $(\mb X \indep \mb Y |_d \mb Z)$
implies $(\mb X \indep_\pr \mb Y | \mb Z)$; if the converse
implication holds, then we say that $\pr$ is {\em faithful} to $\cg$.
The following is known:


\begin{prop} \label{prop:d:separation}  If $\cg$ is a causal DAG and
  $\Pr$ is given by Eq.(\ref{eq:bayesian1}), then they are Markov
  compatible.
\end{prop}
%\babak{i reword faithfulness assumption. It is unusual to say graph is faithful to the distribution. Since it is the generative model.}



\begin{figure*} 
	\hspace*{.8cm}	\begin{subfigure}{0.4\textwidth} 
	\hspace*{.8cm}	\includegraphics[scale=0.15]{Fig2_a.pdf}
	\caption{}
	\end{subfigure}
	\begin{subfigure}{0.4\textwidth} 
	\hspace*{.8cm}	\includegraphics[scale=0.15]{Fig2_b.pdf}
		\caption{ }
	\end{subfigure}
	\caption{(a) Represents a causal DAG with $A=$ admission outcome, $G=$ applicant's gender,
		$H=$ applicant's hobbies and $D=$ applicant's choice of department (cf. Ex.~\ref{ex:cmexm}).
		(b) Represents  the causal DAG obtained after external interventions (cf. Ex.~\ref{ex:cmexm}).}
	\label{fig:cgex}
\end{figure*}



\paragraph*{\bf Counterfactuals and \texttt{do} Operator}
A \textit{counterfactual} is an intervention where we actively modify
the state of a set of variables $\mb X$ in the real world to some
value $\mb X= \mb x$ and observe the effect on some output $Y$.
Pearl~\cite{pearl2009causality} described the $do$ operator that
allows this effect to be computed on a causal DAG, denoted
$\pr(Y|do(X=x))$.  To compute this value, we assume that $X$ is
determined by a constant function $X=x$ instead of a function provided
by the causal DAG.  This assumption corresponds to a modified graph
with all edges into $\mb X$ removed, and values of these variables are
set to $\mb x$.  The Bayesian rule Eq.(\ref{eq:bayesian1}) for the
modified graph defines $\pr(Y|do(\mb X=\mb x))$; the exact expression
is in \cite[Theorem 3.2.2]{pearl2009causality}. We give an
alternative and, to our best knowledge, new formula expressed by
introducing some compensating factors; the proof is in
Appendix~\ref{app:proof}: 

\begin{theorem}  \label{theo:af} Given a causal DAG $\cg$ and a set of
  variables $\mb X \subseteq \mb V$, suppose
  $\mb X=\{X_0,X_1 \ldots X_m \}$ are ordered such that $X_i$ is a
  non-descendant of $X_{i+1}$ in $\cg$. The effect of a set of
  interventions $do(\mb X= \mb x )$ is given by the following {\em
    extended adjustment formula}:
%
{
	\begin{align}
\pr(y|do(\mb X= \mb x )) &=& \nonumber \\
    &&  \hspace*{-2cm}\sum_{ \mb z \in Dom(\mb Z)} \pr( y | \mb x, \mb z )  \bigg( \prod_{i=0}^{m} \pr\big(\mb{pa}(X_i)\bigg|  \bigcup_{j=0}^{i-1} \mb{pa}(X_j ), \bigcup_{j=0}^{i-1}x_j  \big) \bigg) \label{eq:af}
	\end{align}
}
%
	\noindent where $\mb Z= \bigcup_{X \in \mb X} \mb{Pa}(X)$ and
	$j\geq 0$.
\end{theorem}
%
In particular, if $\mb X$ has no parents, then intervention coincides
with conditioning, $\pr(y|do(\mb X = \mb x)) = \pr(y|\mb X = \mb x)$.

%\babak{The following example is way too long. I suggest moving it to the Appendix.}

\begin{example} \em \label{ex:cmexm} Continuing Example~\ref{ex:berkeley},
	Fig.~\ref{fig:cgex}(a) shows a small fragment of the causal DAG of
	the admission process in a college.  Admissions decisions are made
	independently by each department and are based on a rich collection
	of information about the candidates, such as test scores, grades,
resumes, statement of purpose, etc.  These characteristics affect not
	only the admission decisions, but also which department the
	candidate chooses to apply to.  We
	show only a tiny fragment of the causal graph, where $O=$ admission
	outcome, $D=$ department, $G=$ candidate's gender, and $H=$
	hobbies, which can be influenced by gender.
	\footnote{In the Amazon hiring
		example~\cite{amazonhire2018}, hobbies correlated with gender, \eg,\ {\em Captain of the women's chess team}.}
	%Sandy:  Note that a male in preceding example can be the captain of the women's chess team.
	The admissions office anonymizes gender, but it does consider extracurricular activities
	such as hobbies, so we include an edge $H \rightarrow O$.  Since different
	genders apply to departments at different rates, there is an edge $G \rightarrow D$.
	Some departments may tend to attract applicants with certain hobbies (e.g.,
	the math department may attract applicants who play chess),
	so we also include an edge $H \rightarrow D$.  The joint distribution is given by
	%This causal DAG constrains the joint probability distribution. In the absence
	%of these causal constraints, the joint distribution could be factored as
	%$$
	%\pr(g,h,d,o)=\pr(g)\pr(h|g)\pr(d|g,h)\pr(o|g,h,d)
	%$$
	%But if the distribution is faithful to the causal DAG in Fig.~\ref{fig:cgex},
	% then the joint distribution is
	%
{	\begin{align}
	\pr(g,h,d,o)=\pr(g)\pr(h|g)\pr(d|g,h)\pr(o|h,d) \label{exjd1}
	\end{align}}
	%  Note the difference in the last factor: the outcome $o$ is conditionally  dependent on department $d$ and hobbies $h$, but is not conditionally dependent  on gender $g$.
%%%      Consider the following counterfactual: {\em update the
%%%        applicant's department to Computer Science Department (cs)}.
%%%      Then the outcome is given by
%%%%
%%%      {\small \begin{align} \pr(o|do(D=\text{cs})) = & \sum_{g,h}
%%%          \pr(g)\pr(h|g) \pr(o|D=\text{cs},h) \label{exjd2}
%%%	\end{align}}
	%The expression for intervention is obtained from the observed distribution probability
	%(line 3) by removing the term $\pr(D=\text{cs}|g,h)$ and summarization.  This term was removed, because
	%the intervention is a modification of the causal graph: we
	%removed the edge $G\rightarrow D$, as illustrated in Fig.~\ref{fig:cgex}(b).
      Consider the counterfactual: {\em update the
        applicant's department to $cs$}.  We compare
      the marginal probability of $O$, the conditional probability,
      and the intervention:
%
      {
	\begin{align}
%	\pr(o) = & \sum_{g,h,d} \pr(g)\pr(h|g) \pr(d|g,h) \pr(o|d,h)\nonumber \\
	\pr(o|D=\text{cs}) = & \sum_{g,h} \pr(g) \pr(h|g) \pr(D=\text{cs}|g,h) \pr(o|D=\text{cs},h)\nonumber \\
	\pr(o|do(D=\text{cs})) = & \sum_{g,h} \pr(g)\pr(h|g)  \pr(o|D=\text{cs},h) \label{exjd2}
	\end{align}
}
	%
The expression for intervention (\ref{exjd2}), based on
\cite[Theorem 3.2.2]{pearl2009causality} is obtained from the
conditional probability by removing the term $\pr(D=\text{cs}|g,h)$,
or equivalently deleting the edge $G\rightarrow D$ from the
graph in Fig.~\ref{fig:cgex}(b).  Alternatively, we can express the
intervention using Eq.(\ref{eq:af}) (notice that
$\mb{Pa}(D) = \set{G,H}$):
	%
{	\begin{align}
	\pr(o|do(D=\text{cs})) = & \sum_{g,h} \pr(o|g,h,D=\text{cs})\pr(h|g)  \pr(g) \label{eq:babak:do}
	\end{align}}
	%
	%ignoring for space -Luke
The reader may check that Eq.(\ref{exjd2}) and (\ref{eq:babak:do}) are equivalent.
	%are equivalent.

\end{example}

%The probability that the modified model $\cm_x$ assigns $y$ to $Y$ is given by $P(y|do(X=x))$. The {\em causal effect} of $X$ on $Y$ can be computed by comparing aspects of the distribution  $P(y|do(x))$ for each $x \in Dom(X)$ ($X$ has no causal effect on $Y$ if for any $x, x' \in Dom(X)$, $P(y|do(x))$=$P(y|do(x'))$).


%\babak{The following almost exactly repeated in the next section.}
\vspace*{-0.2cm}

%\reve{(D3)  The authors seem to misunderstand the counterfactual fairness paper [22]. The authors' discussion on counterfactual fairness, first paragraph on page 5, is a bit off. In fact, the authors' understanding of [22], in their notation Pr(Y | X, do(S)) is exactly what [22] tried to avoid, see the paragraph below equation (1) in [22]. (To make it clearer: the authors' understanding of counterfactual is in fact the individual proxy of [21, Definition 4], i.e., we cut the parents of S, and then compute the conditional probability. This is the do operator but not the counterfactual operator. To compute counterfactuals, we need the structural equations, or causal graphs.)}


% \luke{(To address revf D3 above) In other words, counterfactual 	fairness implies the ability to change the value of $S$ and any causally dependent	variables while holding causally independent variables fixed, all without changing	the distribution of $\tilde{Y}$}.

\subsection{Causal Fairness}
\label{sec:cf}
%

%
  \paragraph*{\bf Counterfactual Fairness}
  Kusner et
  al.~\cite{kusner2017counterfactual,DBLP:journals/corr/KusnerLRS17}
  (see also the discussion in~\cite{loftus2018causal}) defined a
  classifier as {\em counterfactually fair} if the protected attribute
  of an individual is not a cause of the outcome of the classifier for
  that individual, i.e., had the protected attributes of the
  individual been different, and other things being equal, the outcome
  of the predictor would have remained the same. However, the
  definition of counterfactual fairness in
  \cite{kusner2017counterfactual} captures individual-level fairness
  only under certain assumptions (see Appendix~\ref{app:addback}).
  \ignore{In terms of causal DAGs, a classifier is counterfactually
    fair if there is no directed path from $S$ to $\tilde{Y}$.}
  Indeed, it is known in statistics that individual-level
  counterfactuals can not be estimated from data \cite{rubin1970thesis,rubin1986statistics,rubin2008comment}.
   %i.e., it is
  %impossible to estimate them from observational data or even
  %controlled experiments (see \cite{rubin1970thesis}).
%

%

  \paragraph*{\bf Proxy Fairness} To avoid individual-level
  counterfactuals, a common is to study
  population-level counterfactuals or interventional distributions
  that capture the effect of interventions at population level rather
  than individual level
  \cite{pearl2009causal,rubin1970thesis,rubin1986statistics}.
  % Interventional distributions can be identified from data under
  % mild assumptions articulated in Sec~\ref{sec:peri}.
  % Using interventional distributions,
  Kilbertus et. al. \cite{kilbertus2017avoiding} defined proxy
  fairness as follows:
%
  {
%
    \begin{align}
      P(\tilde{Y}=1| do(\mb P=\mb p ))=P(\tilde{Y}=1| do(\mb  P=\mb p')) \label{eq:pfair}
    \end{align}
%
  }
%
  \noindent for any $\mb p, \mb p' \in Dom(\mb P)$, where $\mb P$
  consists of proxies to a sensitive variable $S$ (and might include
  $S$).  Intuitively, a classifier satisfies proxy fairness in
  Eq~\ref{eq:pfair}, if the distribution of $\tilde{Y}$ under two
  interventional regimes in which $\mb P$ set to $\mb p$ and $\mb p'$
  is the same. Thus, proxy fairness is not an individual-level notion.
  Next example shows proxy fairness fails to capture group-level
  discrimination in general.  
  %Note that in thev absence of confounding factors between $\mb P$ and $\tilde{Y}$, it  holds that  $P(\tilde{Y}| do(\mb P)=\mb p)= P(\tilde{Y}| \mb P=\mb p)$, hence proxy fairness becomes Demographic Parity.
%


%
  \begin{example} \label{ex:obsvsprox} \em To illustrate the difference
    between counterfactual and proxy fairness, consider the college
    admission example.  Both departments make decisions based on
    students' gender and qualifications, $O=f(G,D,Q)$, for a binary
    $G$ and $Q$. The causal DAG is
    $G \rightarrow O, D \rightarrow O, Q \rightarrow O$. Let $D=U_D$
    and $Q=U_Q$, where $U_D$ and $U_Q$ are exogenous factors that are
    independent and that are uniformly distributed, e.g.,
    $P(U_Q=1)=P(U_Q=0)=\frac{1}{2}$. Further suppose
    $f(G, \text{'A'},Q)= G \land Q$ and
    $f(G, \text{'B'},Q)= (1-G) \land Q$, i.e., dep.~A admits only
    qualified males and dep.~B admits only qualified females.  This
    admission process is proxy-fair\footnote{Here $D$ is not a proxy
      to $G$, because $D \indep G$ by assumption.}, because
    $P(O=1| do(G=1))=P(O=1| do(G=0))=\frac{1}{2}$.  On the other hand,
    it is clearly individually-unfair, in fact it is group-level
    unfair (for all applicants to the same department).  To capture
    individual fairness, counterfactual
    fairness~\cite{kusner2017counterfactual,DBLP:journals/corr/KusnerLRS17}
    is a non-standard definition that does both conditioning {\em and}
    intervention on the sensitive attribute.
    \ignore{($P(-|G=g,\texttt{do}(G=g))$.}  Conditioning ``extracts
    information from the individual to learn the background
    variables''~\cite[pp.11, footnote 1]{loftus2018causal}.
  \end{example}
%

%

\paragraph*{\bf Path-specific fairness} These definitions are based on
graph properties of the causal graph, \eg, prohibiting specific paths from the
sensitive attribute to the outcome~\cite{nabi2018fair,loftus2018causal}; however,
identifying path-specific causality from data requires very strong assumptions and is often impractical~\cite{avin2005identifiability}.






==> Capuchin(Pre-print) (1)/repair.tex <==

\vspace*{-0.2cm}
\section{Repairing Training Data to Ensure Fairness}
\label{sec:repdata}

We have shown in Corollary~\ref{col:fair_learn} that, if the training
data $D$ satisfies a certain saturated conditional independence (CI),
then a classification algorithm trained on $D, \pr$ is justifiably
fair.  We show here how to modify (repair) the training data to
enforce the CI and thus ensure that any reasonable classifier trained
on it will be justifiably fair.

%\luke{(To help address f:D2 below) We stress that this is a property of the trained classifier, and as such the predicted outcomes will have the fairness property even when applied to potential biased test datasets.}

% This section formally defines the problem of repairing a database
% w.r.t. a set of CIs (Sec~\ref{sec:prov}), which is internally used by
% \sys\ for building justifiably fair classifiers. We propose a suite of
% techniques for solving this repair problem using lineage expression
% (Sec~\ref{sec:prov}) and matrix factorization (Sec~\ref{sec:mf}).


%\reva{To address (D1) can we establish a relation between minimal cardinality repair and L1 norm of the distributions of the original and repaired data?}



	\vspace*{-0.3cm}
\subsection{Minimal Repair for MVD and CI}
\label{sec:prob_stat}

We first consider repairing an MVD.  Fix an MVD $\mb Z \mvd \mb X$ and
a database $D$ that does not satisfy it.  The minimal database repair
problem is this: find another database $D'$ that satisfies the MVD
such that the distance between $D$ and $D'$ is minimized.  In this section,
 we restrict the distance function to the symmetric difference, i.e, $|\Delta(D, D')|$.

%%% We show in Sec.~\ref{sec:mf} that this problem is NP-complete in
%%% general.

%%% Given a database $D$ with attributes $\mb V$ that is inconsistent
%%% wrt. a set of CI statements $\Gamma$, our goal is to find another
%%% dataset $\rep$ that is close to $\rep$ and consistent with $\Gamma$,
%%% i.e., $D \models \varphi$ for all $\varphi \in \Gamma$.  Recall that
%%% $D \models \varphi$ if $\varphi$ holds under distribution induced by a
%%% database $D$, i.e.,
%%% $\pr(\mb v) \defeq \frac{1}{n}\sum_{t \in D}1_{t=\mb v}$
%%% (cf. Sec.~\ref{sec:peri}).  To formally define this problem we first
%%% need a way to compare databases in terms of their distance to $D$.
%%%
%%% \begin{definition}
%%%   Given two database instances $D_1$ and $D_2$ with attributes
%%%   $\mb V$, we say that $D_1$ is at least as close to $D$ as $D_2$,
%%%   denoted $D_1 \preceq_D D_2$ if $d(D,{D_1}) \leq d(D,{D_2})$ for a
%%%   distance function $d$.
%%% \end{definition}
%%%
%%%
%%% \begin{definition} \label{def:rep} Given a database $D$ from $\mb V$
%%%   that is inconsistent with a set of CIs $\Sigma$, a {\em repair} of
%%%   $D$ w.r.t., the distance function $d$ is an instance $\rep$ if (a)
%%%   $\rep$ is consistent with $\Sigma$; (b) $\rep$ is $\preceq_D$
%%%   minimal in the class of all databases that are consistent with
%%%   $\Sigma$.
%%% \end{definition}
%%%
%%%
%%% We refer to a repair $\rep$ of $D$ w.r.t. the cardinality of symmetric
%%% difference, i.e., $|\Delta(D,\rep)|$ as {\em cardinality-based
%%%   repair}.  It is known that computing carnality-based repairs
%%% w.r.t. a single FD is NP-hard in general
%%% \cite{lopatenko2007complexity}. In section, \ref{sec:mf}, we show that
%%% repair w.r.t. a single CI is also NP-hard in general.
%%%

\begin{figure} 
  \centering
  \begin{minipage}[b]{0.32\hsize}\centering
    \[
      \begin{tabular}{c|ccc|c}
	\cline{2-4}
        D: &	X & Y & Z & $\pr$ \\
	\cline{2-4}
        $t_1$&	$a$ & $a$ & $c$ & $3/8$ \\
        $t_2$&	$a$ & $b$ & $c$ & $2/8$ \\
        $t_3$&	$b$ & $a$ & $c$ & $2/8$ \\
        $t_4$&	$b$ & $b$ & $d$ & $1/8$ \\
	\cline{2-4}
      \end{tabular}
    \]
  \end{minipage}
  \begin{minipage}[b]{0.32\hsize}\centering
    \[
      \begin{tabular}{c|ccc|}
	\cline{2-4}
        $D_1:$ &	X & Y & Z \\
	\cline{2-4}
        $t_1$&	$a$ & $a$ & $c$ \\
        $t_2$&$a$ & $b$& $c$\\
        $t_3$&$b$ & $a$ & $c$\\
        $t_4$&$b$ & $b$ & $c$ \\
        $t_5$& $b$ & $b$ & $d$\\
	\cline{2-4}
      \end{tabular}
    \]
  \end{minipage}
  \begin{minipage}[b]{0.32\hsize}\centering
    \[
      \begin{tabular}{c|ccc|}
	\cline{2-4}
        $D_2:$	&X & Y & Z \\
	\cline{2-4}
        $t_1$&	$a$ & $a$ & $c$\\
        $t_2$& $a$ & $b$ & $c$ \\
        $t_4$& $b$ & $b$ & $d$ \\
	\cline{2-4}
      \end{tabular}
    \]
\end{minipage}
    \caption{      \textmd{ A simple database repair: $D$ does not satisfy the MVD $Z \mvd X$. In $D_1$, we inserted
the tuple $(b,b,c)$ to satisfy the MVD, and in $D_2$ we deleted the tuple $(b,a,c)$ to satisfy the MVD.}}
    \label{fig:simple:repair}
  \end{figure}
\begin{example} \label{ex:rep1} \em
Consider the database $D$ in Fig.~\ref{fig:simple:repair} (ignoring the
probabilities for the moment), and the MVD $Z \mvd X$.  $D$ does not
satisfy the MVD.  The figure shows two minimal repairs, $D_1, D_2$,
one obtained by inserting a tuple, and the other by deleting a tuple.
\end{example}

%%% \noindent It is clear that $D$ is inconsistent with $\varphi$ because:
%%% $\pr(X=0|Y=1,Z=1)=1$ but $\pr(X=0|Z=1)=\frac{2}{3}$. However, $D_1$
%%% and $D_2$ are cardinality-based repairs of $D$, where $D_5$ is
%%% obtained by inserting $t_5$ and $D_2$ is obtained by deleting $t_3$.



%%% In the rest of the paper, unless otherwise stated we focus on repair
%%% w.r.t. a single saturated CI, which is sufficient for building
%%% justifiably fair classifiers (cf. Sec~\ref{sec:jfc}).

% \subsection{Minimal Repair for a  CI}

However, our problem is to repair for a saturated CI, not an MVD,
since that is what is required in Corollary~\ref{col:fair_learn}.  The repair
problem for a database constraint is well-studied in the literature,
but here we need to repair to satisfy a CI, which is not a database
constraint.  We first  formally define the repair problem for a CI
then show how to reduce it to the repair for an MVD.  More precisely,
our input is a database $D$ and a probability distribution $\Pr$, and
the goal is to define a ``repair'' $D',\pr'$ that satisfies the given
CI.

% If $\pr$ where the empirical distribution on $D$, then the a
% saturated CI $(\mb X; \mb Y|\mb Z)$ and it associated MVD
% $\mb Z \mvd \mb Z$ are equivalent, however, in practice training
% data usually has duplicates, which means that the distribution $\pr$
% for Corollary~\ref{col:fair_learn} is not uniform.  Duplicates occur
% naturally when the original data had a key attribute which is
% dropped in the training data, thus creating duplicates. Here we
% define the CI repair problem for an arbitrary distribution $\pr$,
% and describe our proposed technique to convert it to an MVD repair
% problem.

We assume that all probabilities are rational numbers.  Let the {\em
  bag associated} to $D, \pr$ to be the smallest bag $B$ such that
$\pr$ is the empirical distribution on $B$.  In other words, $B$ is
obtained by replicating each tuple $t \in D$ a number of times
proportional to $\pr(t)$. \footnote{Equivalently, if the tuples have
  probabilities $p_1/q, p_2/q, \ldots$ (same denominator), then each
  tuple $t_i$ occurs exactly $p_i$ times in $B$.}  If $\pr$
is uniform, then $B=D$.
   
\begin{definition} 
  The minimal repair of $D, \pr$ for a saturated CI
  $(\mb X; \mb Y|\mb Z)$ is a pair $D',\pr'$ such that $\pr'$
  satisfies the CI and $|\Delta(B,B')|$ is minimized, where $B$ and
  $B'$ are the bags associated to $D,\pr$ and $D',\pr'$, respectively.
\end{definition}

Recall that $\mb V$ denotes the set of attributes of $D$.  Let $\pr$
be any probability distribution on the variables $\set{K} \cup \mb V$,
where $K$ is a fresh variable not in $\mb V$.
   
\begin{lemma} \label{lemma:k:v} If $\pr$ satisfies
  $(K\mb X; \mb Y | \mb Z)$, then it also satisfies
  $(\mb X; \mb Y | \mb Z)$.
\end{lemma}

The lemma follows immediately from the Decomposition axiom in Graphoid (see Appendix~\ref{app:addback}).

% \dan{Better: the lemma is precisely the axiom BLAH (which one?).}

%
%%% So far we assumed databases are in set-semantics. However, many real
%%% datasets used for training machine learning models has duplicates,
%%% hence in bag-semantics.  Next, we extend the lineage expression
%%% approach to databases in bad-semantics.
%

We now describe our method for computing a minimal repair of $D, \pr$
for some saturated CI.  First, we compute the bag $B$ associated to
$D, \pr$.  Next, we add the new attribute $K$ to the tuples in $B$ and
assign distinct values to $t.K$ to all duplicate tuples $t$, thus
converting $B$ into a set $D_B$ with attributes $K \cup \mb V$.
Importantly, we use as few distinct values for $K$ as possible,
i.e., we enumerate the instances of each unique tuple.  More precisely, we
define:
%
\begin{align}
  D_B =  \set{ (i,t)| t \in B, i = 1,\ldots,|t_B|} \label{eq:bad-set}
\end{align}
%
were $|t_B|$ denotes the number of occurrences (or multiplicity) of a
tuple $t$ in the bag $B$.
Then, we repair $D_B$ w.r.t. to the MVD
$\mb Z \mvd K\mb X$, obtaining a repaired database $D_B'$.  Finally,
we construct a new training set $D' = \Pi_{\mb V}(D_B')$, with the
probability distribution obtained by marginalizing the empirical
distribution on $D_B'$ to the variables $\mb V$.  We prove the
following:

% \dan{I don't know how to prove it, but I'm pretty sure it's true.
% I'm willing to gamble and keep this in the paper even if we don't
% find the proof before the deadline}:

%%%
%%% We are given a bag $B$ with attributes $\mb V$
%%%  that is inconsistent with a CI statement $\varphi$. Let us denote  the number of occurrence or  multiplicity of a tuple $t$ in a bag $B$, by $|t|_B$. We transform $B$ to the a corresponding database a $D_B$ with attributes  $\set{K} \cup \mb V$  in set-semantics as follows:
%%%


%%% That is, for each tuples $t \in B$ with multiplicity $|t|_B$, we
%%% insert a set of tuples $(i,t)$ for $i=0,|t|_B$ in $D_B$. It is clear
%%% that $D_B$ is a set.  We show the following.

\begin{theorem} \label{th:bag_set}  Let $D$ be a database and $\pr$ a
  probability distribution on its tuples, and let $B$ be the
  associated bag (with attributes $\set{K} \cup \mb V$).  Fix a
  saturated CI $(\mb X; \mb Y|\mb Z)$, and let $B'$ be a minimal
  repair for the MVD $\mb Z \mvd K\mb X$.  Then, $D', \pr'$ is a
  minimal repair of $D, \pr$ for the CI, where $D'$ is $B'$ with
  duplicates removed, and $\pr'$ is the empirical distribution on
  $B'$.
\end{theorem}

%%% \begin{proof}[Proof of Proposition \ref{lema:bag_set}]{ \babak{To be
%%%       moved to Appendix}It follows from the Decomposition axiom in
%%%     Graphoid that
%%%     $D_B ' \models (\mb X\cup \set{K} \indep \mb Y| \mb Z)$ implies
%%%     $D_B ' \models (\mb X \indep \mb Y| \mb Z)$. Minimality of $D_B '$
%%%     is immediate.}
%%% \end{proof}


We illustrate with an example.

\begin{figure}

\begin{minipage}[t]{0.22\hsize}\centering
	\[
	\begin{tabular}{c|ccc|}
	\cline{2-4}
	B: &	X & Y & Z \\
	\cline{2-4}
	&	$a$ & $a$ & $c$ \\
	&	$a$ & $a$ & $c$ \\
	&	$a$ & $a$ & $c$ \\
	&	$a$ & $b$ & $c$\\
	&	$a$ & $b$ & $c$\\
	&	$b$ & $a$ & $c$\\
	&	$b$ & $a$ & $c$\\
%	&	$b$ & $b$ & $c$\\
	&	$b$& $b$ & $d$ \\
	\cline{2-4}
	\end{tabular}
	\]
\end{minipage}
\begin{minipage}[t]{0.23\hsize}
	\[
	\begin{tabular}{c|cccc|}
	\cline{2-5}
	$D_B:$ & K &X & Y & Z \\
	\cline{2-5}
&1&		$a$ & $a$ & $c$ \\
&2&	$a$ & $a$ & $c$ \\
&3&	$a$ & $a$ & $c$ \\
&1&	$a$ & $b$ & $c$\\
&2&	$a$ & $b$ & $c$\\
&1&	$b$ & $a$ & $c$\\
&2&	$b$ & $a$ & $c$\\
% &1&     $b$ & $b$ & $c$\\
&1&	$b$& $b$ & $d$ \\
	\cline{2-5}
	\end{tabular}
	\]
\end{minipage} 
\begin{minipage}[t]{0.23\hsize}\centering 
	\[
\begin{tabular}{c|cccc|}
\cline{2-5}
$D'_B:$ & K &X & Y & Z \\
\cline{2-5}
&1&	$a$ & $a$ & $c$ \\
&2&	$a$ & $a$ & $c$ \\
&1&	$a$ & $b$ & $c$\\
&2&	$a$ & $b$ & $c$\\
&1&	$b$ & $a$ & $c$\\
&1&     $b$ & $b$ & $c$\\
&1&	$b$& $b$ & $d$ \\
\cline{2-5}
\end{tabular}
\]
\end{minipage}
\begin{minipage}[t]{0.23\hsize}\centering 
\[
\begin{tabular}{c|ccc|c}
\cline{2-4}
$D':$ &X & Y & Z & $\pr'$  \\
\cline{2-4}
&	$a$ & $a$ & $c$ & $2/7$ \\
&	$a$ & $b$ & $c$ & $2/7$ \\
&	$b$ & $a$ & $c$ & $1/7$ \\
&	$b$ & $b$ & $c$ & $1/7$ \\
&	$b$ & $b$ & $d$ & $1/7$ \\
\cline{2-4}
\end{tabular}
\]
\end{minipage}
  \caption{      \textmd{ Repairing a conditional independence (CI).}}
  \label{fig:repair:ci}
\end{figure}
   
\begin{example} \label{ex:rep2} \em In Example~\ref{ex:rep1} we showed two
  repairs $D_1, D_2$ of the database $D$ in
  Fig~\ref{fig:simple:repair} for the MVD $Z \mvd X$.  Consider now
  the probability distribution, $\pr$ shown in the figure.  Suppose
  we want to repair it for the CI $(X; Y | Z)$.  Clearly, both $D_1$
  and $D_2$, when endowed with the empirical distribution {\em do}
  satisfy this CI, but they are very poor repairs because they
  completely ignore the probabilities in the original training data,
  which are important signals for learning.  Our definition captures
  this by insisting that the repaired bag $B'$ be close to the bag $B$
  associated to $D,\pr$ (see $B$ in Fig.~\ref{fig:repair:ci}), but the
  sets $D_1$ and $D_2$ are rather far from $B$.  Instead, our method
  first converts $B$ into a set $D_B$ by adding a new attribute $K$
  (see Fig.~\ref{fig:repair:ci}) then, it repairs $D_B$ for the MVD
  $Z \mvd KX$, obtaining $D_B'$.  The final repair $D',\pr'$ consists
  of the empirical distribution on $D_B'$, but with the attribute $K$
  and duplicates removed.
%%% \vspace*{0.3cm}
%%% $B$ is inconsistent with $\varphi$, because $\pr(X=a|Y=a,Z=c)=\frac{3}{5}$ but $\pr(X=a|Z=c)=\frac{5}{9}$.
%%%  The reader can verify that $D'_B$ is consistent with both $(X\cup K \indep Y | Z)$ and $(X \indep Y | Z)$. Hence, a repair
%%% of $B$ can be obtained from $D'_B$ by a bag-projection.
\end{example}

We note that, in order for Theorem~\ref{th:bag_set} to hold, it is
critical that we use minimum distinct values for the
attribute $K$ in $D_B$; otherwise minimal repairs of $D_B$ are no
longer minimal repairs of the original data $D, \pr'$.  For example,
if we use distinct values for $K$, thus making $K$ a key, then only
subset of $D_B$ that satisfies the MVD $\mb Z \mvd K\mb X$ is the
empty set.



\vspace*{-0.2cm}
\subsection{\bf Reducing Minimal Repair to 3SAT}
\label{sec:prov}

Corollary~\ref{col:fair_learn} requires us to repair the training data
$D$ to satisfy a CI.  We have shown how to convert this problem into
the problem of repairing a derived data $D_B$ to satisfy an MVD.  In
this section we describe how to find a minimal repair for an MVD by
reduction to the weighted MaxSAT problem.

We denote the database by $D$, the MVD by $\varphi: \mb Z \mvd \mb X$,
and assume that $D$'s attributes are
$\mb V = \mb X \cup \mb Y \cup \mb Z$.  Recall that $D$ satisfies the
MVD iff $D = \Pi_{\mb X \mb Z}(D) \Join \Pi_{\mb Y \mb Z}(D)$.  Since
we want to allow repairs that include both insertions and deletions,
we start by finding an upper bound on the set of tuples that we may
want to insert in the database. For example, one can
restrict the set of tuples to those that have only constants that
already occurring in the database, i.e., an upper bound is $ADom^k$, where
$ADom$ is the active domain of $D$, and $k$ is the arity of $D$.
However, this set is too large in practice.  Instead, we prove that it
suffices to consider candidate tuples in a much smaller set, given by:
$\hb \defeq   \Pi_{\mb X \mb Z}(D) \Join \Pi_{\mb Z \mb Y}(D)$.
%
\ignore{ {  
\begin{align*}
\hb \defeq &  \Pi_{\mb X \mb Z}(D) \Join \Pi_{\mb Z \mb Y}(D)
\end{align*}
}}


\begin{prop} \label{prop:min_rep_lin}  Any minimal repair $\rep$ of $D$
  for an MVD satisfies $\rep \subseteq \hb$.
\end{prop}
%
Next, we associate the following Boolean Conjunctive query to the MVD $\varphi$:
{   
\begin{align}
\icq \leftarrow \ D( \mb X_1, \mb Y_1, \mb Z),  D( \mb X_2, \mb Y_2, \mb Z),  \neg
D( \mb X_1, \mb Y_2, \mb Z)  \label{eq:cq_ci}
\end{align} }
It follows immediately that $D \not \models \varphi$ iff
$D \models \icq$, and therefore the repair problem becomes: modify the
database $D$ to make $\icq$ false.  For that purpose, we use the
lineage of the query $\icq$.  By the previous proposition, we know
that we need to consider as candidates for insertions only those tuples in  $\hb$; hence we compute the lineage over the set of
possible tuples $\hb$.  We briefly review here the construction of the
lineage and refer the reader to~\cite{xu2018provenance} and the
references there for more detail.  We associate a distinct Boolean
variable $X_t$ to each tuple $t \in \hb$, and consider all mappings
$\theta : Var(\icq) \rightarrow ADom(D)$ such that each of the three
tuples--
$\hb(\theta(X_1),\theta(Y_1),\theta(Z)),
\hb(\theta(X_2),\theta(Y_2),\theta(Z))$, and
$\hb(\theta(X_1),$ $\theta(Y_2),\theta(Z))$-- are in $\hb$.  Then, the
lineage and its negation are:
%

{ 
\begin{align}
\Phi_\varphi = &  \bigvee_{\theta }
\left(X_{\hb(\theta(X_1),\theta(Y_1),\theta(Z))} \land   X_{\hb(\theta(X_2),\theta(Y_2),\theta(Z))} \land  \neg X_{\hb(\theta(X_1),\theta(Y_2),\theta(Z))} \right) \label{eq:le}\\
\neg \Phi_\varphi = &  \bigwedge_{\theta} \left(\neg X_{\hb(\theta(X_1),\theta(Y_1),\theta(Z))} \lor \neg  X_{\hb(\theta(X_2),\theta(Y_2),\theta(Z))} \lor X_{\hb(\theta(X_1),\theta(Y_2),\theta(Z))}\right) \label{eq:3cnf}
\end{align}
}

Recall that an {\em assignment} is a mapping from Boolean variables
$X_t$ to $\set{0,1}$.  Thus, our goal is to find an assignment
satisfying the 3CNF $\neg \Phi_\varphi$, which is as close as possible
to the initial assignment $X_t = 1$ for $t \in D$, $X_t = 0$ for
$t \in \hb - D$.

We briefly review the weighted MaxSAT problem here.  Its input is a
3CNF $\mb F$ whose clauses are partitioned into
$\mb F = (\mb F_h, \mb F_s, \mc C)$, where $\mb F_h$ are called the
hard clauses, and $\mb F_s$ are the soft clauses, and a function
$\mb C : \mb F_s \rightarrow R^+$  associates a non-negative cost
with each  soft clause.  A solution to the problem finds an
assignment that satisfies all  hard constraints, and maximizes the
weight of the satisfied soft constraints.

To ensure ``closeness'' to the initial assignment, we add to the
Boolean formula a clause $X_t$ for every $t \in D$, and a clause
$\neg X_t$ for every $t \in \hb - D$.  The final 3CNF formula is:

{  
\begin{align*}
  \Psi = & \underbrace{(\neg \Phi_\varphi)}_{\mbox{hard clauses}}
%
 \wedge
%
\underbrace{\bigwedge_{t \in D} X_t \wedge \bigwedge_{t \in \hb-D} (\neg X_t)}_{\mbox{soft clauses}}
\end{align*}}


The algorithm constructing $\Psi$ is shown in
Algorithm~\ref{algo:maxsat}.

% \begin{algorithm}
% 	\DontPrintSemicolon
% 	\KwIn{A database $D$ with vairables $\mb X \cup \mb Y  \cup \mb Z$ and a saturated CI $\varphi: (\mb X \indep \mb Y |\mb Z )$}
% 	\KwOut{ $\neg \Phi_\varphi$ the negation of the lineage of $\varphi$.}
% 	$D^c(\mb X_1,\mb Y_2, \mb Z) = D(\mb X_1,\mb Y_1,\mb Z) \land D(\mb X_2,\mb Y_2,\mb Z)$ \\
% 		\For{$t \in D^c$}{	Add clause $X_t$ to $\Phi_\varphi$ if 	$X_t \not \in D$ \\
% 		Add clause $ \neg \overline{X_t}$ to $\Phi_\varphi$ if 	$X_t \in D$}
% 	$C(\mb X_1,\mb Y_1,\mb X_2,\mb Y_2,  \mb Z) = D^c(\mb X_1,\mb Y_1,\mb Z) \land D^c (\mb X_2,\mb Y_2,\mb Z)$\\
% \For{$t \in C$}{
% 	$t_1 \gets t[\mb X_1,\mb Y_1,\mb Z]$; $t_2 \gets t[\mb X_2,\mb Y_2,\mb Z]$;	$t_3 \gets t[\mb X_1,\mb Y_2,\mb Z]$\\
% 	Add clause $\neg W_{t_1} \lor \neg W_{t_2} \lor W_{t_3}$ to $\Phi_\varphi$, where
% 	$W=X$ if $t_i \in D$, otherwise  $W=\overline{X}$ \\}
%
% 	\caption{Converts the problem of finding a database repair w.r.t. a CI statement
% 		into solving a general CNF formula.} \label{algo:maxsat}
% \end{algorithm}



\begin{algorithm} 
	\DontPrintSemicolon
	\KwIn{A database $D$ with vairables $\mb X \cup \mb Y  \cup \mb Z$ and a saturated CI $\varphi: (\mb X \indep \mb Y |\mb Z )$}
	\KwOut{ A 3CNF $\Psi$ consisting of hard and soft clauses.}
	Compute $\hb(\mb X_1,\mb Y_2, \mb Z) = D(\mb X_1,\mb Y_1,\mb Z) \land D(\mb X_2,\mb Y_2,\mb Z)$ \\
		\For{$t \in \hb$}{If $t \in D$, add the soft clause $X_t$ to $\Psi$ \\
		If $t \in \hb-D$ add the soft clause $(\neg X_t)$ to  $\Psi$}
	Compute $C(\mb X_1,\mb Y_1,\mb X_2,\mb Y_2,  \mb Z) = \hb(\mb X_1,\mb Y_1,\mb Z) \land \hb (\mb X_2,\mb Y_2,\mb Z)$\\
\For{$t \in C$}{
	$t_1 \gets t[\mb X_1,\mb Y_1,\mb Z]$; $t_2 \gets t[\mb X_2,\mb Y_2,\mb Z]$;	$t_3 \gets t[\mb X_1,\mb Y_2,\mb Z]$\\
	Add the hard clause $(\neg X_{t_1} \lor \neg X_{t_2} \lor X_{t_3})$ to $\Psi$\\}

	\caption{Converts the problem of finding a database repair w.r.t. a CI statement
		into solving a general CNF formula.} \label{algo:maxsat}
\end{algorithm}



% \paragraph{\bf Lineage of a CI} Fix a BCQ
% $\icq \leftarrow G_0,G_1,\neg G_3$ associated to a CI statement
% $\varphi$ (cf. Eq~\ref{eq:cq_ci}). For every tuple $t \in \hb$, we
% associate a distinct Boolean $X_t$ if $t \in D$; and $\overline{X}_t$
% if $t \not \in D$.  A valuation for $\icq$ is a mapping
% $\theta : Var(\icq) \rightarrow Dom(\mb V)$ such that the
% instantiation of every atom is a tuple in $\hb$, i.e.,
% $t_i = \theta(G_i) \in \hb$, for $i = \{1,3\}$.  We define the lineage
% of a CI $\varphi$ as the following DNF expression:
%
% \begin{align}
%   \Phi_\varphi:  \bigvee_{ \theta : \icq \rightarrow \hb } \theta(G_1)
%   \land  \theta(G_2) \land \neg \theta(G_3) \label{eq:le}
% \end{align}
%
%
% The lineage expression $\Phi_\varphi$ can be further simpled by
% removing contradictory conjuncts that include both $X_t$ and
% $\neg X_t$. Let $\sigma$ be a truth assignment that maps the Boolean
% variables of $\Phi_\varphi$ to 1 (true) or 0 (false).  It is clear
% that any truth assignment that satisfies the negation of
% $\Phi_\varphi$, i.e, $\sigma(\neg \Phi_\varphi)=1$ gives a sequence of
% updates to make $D$ consistent with $\varphi$ as follows: delete $t$
% from $D$ if $\sigma({X_t})=0$; and insert $t'$ to $D$ if
% $\sigma(\overline{X}_{t'})=1$. It is immediate that
% $\neg \Phi_\varphi$ is a CNF expression.
 
\begin{example} \em Continuing Ex.~\ref{ex:rep1}, we observe that
  $\hb=D_1$; hence, there are 5 possible tuples.  The lineage expression for $\varphi$  and it negation are:
  {  
	\begin{align}
	\Phi_\varphi  &=&  (X_{t_1} \land  X_{t_4}  \land  \neg X_{t_2}) \lor  ( X_{t_2}  \land  X_{t_3}  \land \neg X_{t_1})  \ \lor  \nonumber \\ &&
	( X_{t_3} \land  X_{t_2}  \land \neg X_{t_4}) \lor  ( X_{t_4} \land  X_{t_1}  \land \neg X_{t_3}) \nonumber
	\end{align} }
	Hence, {  
		\begin{align}
	\neg \Phi_\varphi  &=&  (\neg X_{t_1} \lor   \neg X_{t_4}  \lor   X_{t_2}) \land  ( \neg X_{t_2}  \lor \neg  X_{t_3}  \lor  X_{t_1})  \ \land  \nonumber \\ &&
	( \neg X_{t_3} \lor  \neg X_{t_2}  \lor   X_{t_4}) \land  ( \neg X_{t_4} \lor  \neg X_{t_1}  \lor  X_{t_3}) \nonumber
	\end{align}}
	The reader can check that the repairs $D_1$ and $ D_2$ in
        Ex.~\ref{ex:rep1} are corresponded to some satisfying
        assignment of $\neg \Phi_\varphi $, e.g., $D_2$ obtained from
        the truth assignment $\sigma(X_{t_1})=\sigma(X_{t_2})=1$,
        $\sigma(X_{t_3})=\sigma(X_{t_5})=0$; both satisfy all clauses
        in $\neg \Phi_\varphi$.  The formula $\Psi$ that we give as
        input to the weighted MaxSAT consists of $\neg \Phi_\varphi$
        plus these five clauses:
        $X_{t_1} \wedge X_{t_2} \wedge X_{t_3} \wedge X_{t_4} \wedge
        \neg X_{t_5}$, each with cost 1.  MaxSAT will attempt to
        satisfy as many as possible, thus finding a repair that is
        close to the initial database $D$.
\end{example}


Note that repairing a database w.r.t. a CI $(\mb X \indep \mb Y |\mb Z )$ can be reduced to repairing subsets $\sigma_{\mb Z=\mb z}(D)$ for $\mb z \in Dom(Z)$ w.r.t. the marginal independence $(\mb X \indep \mb Y)$.  Therefore, the problem is highly parallelizable.  \sys\ partition  subsets $\Pi_{\mb Z}(D)$ into chunks of even size (if possible) and repairs them in parallel (see Sec~\ref{sec:rep_metho_com}).

 % Note that partitioning data speeds up the MaxSAT even on a single machine. This is because MaxSAT solvers are much more efficient on smaller input sizes.

% Lineage expression of a CI enables us to compute a repair of an
% inconsistent database by creating an instance of a partial weighted
% MaxSAT problem for which several highly optimal tools exists.


% \paragraph{\bf MaxSAT Encoding}
%

%In Sec~\ref{sec:experi}, we empirically compare the efficacy of using MaxSAT for computing repar rather than naively removing tuples that leawe empirically show that using MaxSAT for repairing data lead to much more

% \begin{theorem} \label{thei:maxsat} Given a database instance $D$ that
%   is inconsistent w.r.t. a CI $\varphi$, consider the MaxSAT problem
%   $\mb F = (\mb F_h, \mb F_s, \mc C)$, where $\mb F_h$ consists of the
%   clauses in $\neg \Phi_\varphi$, the negation of the lineage
%   expression of $\varphi$, $\mb F_s$ contains $X_t$ for all $t \in D$
%   and $\neg X_{t'}$ for all $t' \in \hb-D$, and the wight function
%   $\mc C(X_{t'})=1$ assign same wights to all clauses. The database
%   $D'$ obtained from updating $D$ according to $\sigma$ an optimal
%   solution of $\mb F $ is a cardinality-based repair of $D$.
% \end{theorem}
%
%
% We also restrict to set semantic. Due to the following lemma repairs of a database in bag-semantic i.e, with duplicates, can be obtained from repairs of a corresponding database in set-semantic; proved in the Appendix~\ref{app:proof}.





%\begin{lemma} \label{lema:bag_set} Given a database $D$ with a set of attributes $\mb V$ in bag semantics and a CI  $ (\mb X \indep \mb Y| \mb Z)$ there exists a database $\rep$ with attributes $\mb V \cup \set{K}$  in set semantics such that $(D \models \mb X \indep \mb Y| \mb Z)$ iff $ (\rep \models \mb X \indep \mb Y \cup \set{K}| \mb Z)$ and $D$ can be obtained from $\rep$ by summarization over $K$.
%\end{lemma}

%We illustrate Lemma~\label{lema:bag_set} with an example.

%Prob.~\ref{pro:mvs_ci} implies that the repair problem in Def.~\ref{def:rep} is related to and generalizes the notion of database repair wrt. FDs. Specifically, the repair problem in Def.~\ref{def:rep} closely related to  minimal cardinality based repair wrt. FD, which is shown to be  NP-hard even for a single FD.

%\dan{I stopped here}

\begin{algorithm}  
	\DontPrintSemicolon
	\KwIn{ A bag $B$ with attributes $\mb V= \mb X \mb Y \mb Z $ a CI statment $(\mb X  \indep \mb Y| \mb Z)$.}
	\KwOut{$B'$ a repair of  $B$}
	\For{$\mb z \in Dom(\mb Z)$} {
		$ M^{B'}_{\mb X}, M^{B'}_{\mb Y} \gets  \mb{Factorize}(M^{B_{\mb z}}_{\mb X, \mb Y})$\\
		$ M^{B'{\mb z}}_{\mb X, \mb Y} \gets \frac{1}{|B_{\mb Z}|}{M^{B'}_{\mb X}}^\intercal M^{B'}_{\mb Y}$\\
	}

	$ \Return  \ \text{$B'$ associated with} \ \mb M^{B'}_{\mb X, \mb Y,\mb Z}=\{M^{B'{\mb z}}_{\mb X, \mb Y} \}$

	\caption{Repair using Matrix Factorization.} \label{algo:smi}
\end{algorithm}

\vspace*{-0.25cm}
\subsection{\bf Repair via Matrix Factorization}
	\label{sec:mf}
In this section, we use matrix factorization to repair a bag w.r.t. a CI statement. We are given a bag $B$ to which we associate the empirical distribution $\pr(\mb v) = \frac{1}{|B|}\sum_{t \in B}1_{t=\mb v}$, and a CI statement $\varphi: (\mb X \indep \mb Y| \mb Z)$ such that $B$ is inconsistent with $\varphi$, meaning  that $\varphi$ does not hold in $\pr$.  Our goal is to find a repair of $B$, i.e., a bag $B'$ that is close to $B$ such that $(\mb X \indep \mb Y|_{\pr'} \mb Z)$, where
$\pr'$ is the empirical distribution associated to $B'$.

First, we review the problem of non-negative rank-one matrix factorization. Given a matrix $\mb M \in \mathbb{R}^{n \times m}$, the problem of  {\em rank-one nonnegative matrix factorization (NMF)} is the  minimization problem:  $\argmin_{\mb U \in \mathbb{R}_+^{n \times 1}, \mb V  \in \mathbb{R}_+^{1 \times m}} \rVert \mb M-\mb U\mb V \rVert_F $, where  $\mathbb{R}_+ $ stands for  non-negative real numbers and   $\rVert . \rVert_F$ is the Euclidean norm  of a matrix.\footnote{Recall that a matrix is of rank-one if and only if it can be represented by the outer product of two vectors.}


We express the connection between our repair problem and the NMF problem using  contingency matrices. Given three disjoint subsets of attributes $\mb X, \mb Y, \mb Z \subseteq \mb V$,  let  $m=|Dom(\mb X)|$, $n=|Dom(\mb Y)|$,  $k=| Dom(\mb Z)|$ and  $B_{\mb z}=\sigma_{\mb Z=\mb z}(B)$.   A {\em multiway-contingency matrix} over  $\mb X$,  $\mb Y$ and $\mb Z$ consists of $k$  $n \times m$ matrices $\mb M^{B}_{\mb X, \mb Y,\mb Z}=\{ \mb M^{B_{\mb z}}_{\mb X, \mb Y} | \mb z \in Dom(\mb Z) \}$ where, $\mb M^{B_{\mb z}}_{\mb X, \mb Y}(ij)= \sum_{t \in B} 1_{t[\mb X \mb Y]=  ij}$.  Intuitively, $\mb M^{B_{\mb z}}_{\mb X, \mb Y}(ij)$ represents the  joint frequency of $\mb X$ and $\mb Y$ in a subset of bag with $\mb Z=\mb z$.

The following  obtained immediately from the connection between independence and rank of a contingency matrix.

%A one-way contingency matrix over $\mb X$  is a $1 \times m$ matrix $M^{D}_{\mb X}$ where, $\mb M^{D}_{\mb X, \mb Y}(i)= \sum_{t \in D} 1_{t[\mb X]=  i}$. A  two-way contingency matrix over $\mb X$ and $\mb Y$ is a $n \times m$ matrix $\mb M^{D}_{\mb X, \mb Y}$ where

%\luke{Can we just define multi to save space?, with one-way and two-way as special cases?}

\begin{prop} \label{theo:md}  Let $B$ be a bag and $\pr$ be the
empirical  distribution associated to $B$. It holds that $(\mb X \indep \mb Y|_\pr \mb Z)$ iff each contingency matrix $\mb M \in \mb M^{B}_{\mb X, \mb Y,\mb Z} $ is of rank-one.
\end{prop}

We illustrate with an example.
\begin{example}  \em  Let $\mb M_1=\begin{bmatrix}
	1      &1  \\
	1      &0  \\
\end{bmatrix}$, $\mb M_2=\begin{bmatrix}
0      &0  \\
0      &1  \\
\end{bmatrix}$,  $\mb M_3=\begin{bmatrix}
1      &1  \\
1    &1  \\
\end{bmatrix}$, $\mb M_4=\begin{bmatrix}
1      &1  \\
0      &0  \\
\end{bmatrix}$. The following contingency matrices are associated to  $D$, $D_1$ and $D_2$ in  Ex.~\ref{ex:rep1}:
$\mb M^{D}_{\mb X, \mb Y,\mb Z}=\{\ \mb M_1, \mb M_2 \}$,
$\mb M^{D_1}_{\mb X, \mb Y,\mb Z}=\{\ \mb M_3, \mb M_2 \}$ and
$\mb M^{D_2}_{\mb X, \mb Y,\mb Z}=\{\  \mb M_4, \mb M_2 \}$. The reader can verify that $\mb M_2, \mb M_3$ and $ \mb M_4$ are of rank-one but $ \mb M_1$ is not. It is clear that, $D$ is inconsistent with  $\varphi$ but $  D_1$ and $  D_2$ are consistent with $\varphi$.
\end{example}





The following implied  from  NP-hardness of
NMF \cite{vavasis2009complexity}.

%Luke relabled this, it was named theo:md and causing a conflict
%\babak{Discuss the following with Dan. The idea is to reduce MF for integer matrices to our repair problem. But details are not clear.}
\begin{prop}  \label{theo:md2} The problem of repairing a database w.r.t. a single CI is NP-hard in general.
\end{prop}

Based on Prop~\ref{theo:md}, we propose Algorithm \ref{algo:smi} for
repairing a bag w.r.t. a single CI
$ \varphi: (\mb X \indep \mb Y| \mb Z$).  The algorithm works as
follows: for each $\mb z \in Dom(\mb Z)$, it uses the
$\mb{Factorize}$ subroutine to factorize the $n \times m$ contingency
matrix $\mb M^{B_{\mb z}}_{\mb X, \mb Y}$ into a $1 \times n$ matrix
$\mb M^{B'}_{\mb X}$ and a $1 \times m$ matrix
$\mb M^{B'}_{\mb Y}$. Then, it uses the product of
${\mb M^{B'}_{\mb X}}^\intercal$ and $\mb M^{B'}_{\mb X}$ to
construct a new bag $B'$. It is clear that
${\mb M^{B'}_{\mb X}}^\intercal \mb M^{B'}_{\mb Y}$ is of rank-one
by construction; thus, the algorithm always returns a bag $B'$
that is consistent with $\varphi$. Note that any off-the-shelf NMF
algorithm (such as \cite{fevotte2011algorithms}) can be used in
Algorithm \ref{algo:smi}, to minimize the Euclidean distance between $\pr$ and $\pr'$, the empirical distributions associated to $B$ and $B'$, respectively. \ignore{(These approached can be adopted for computing approximate repairs.)}  In addition, we use the simple
factorization of $\mb M^{B_{\mb z}}_{\mb X, \mb Y}$ into
$\mb M^{B_{\mb z}}_{\mb X}$ and $\mb M^{B_{\mb z}}_{ \mb Y}$, i.e.,
the marginal frequencies of $\mb X$ and $\mb Y$ in $B_{\mb z}$.  We
refer to this simple factorization as {\em Independent Coupling
  (IC)}. It is easy to see that KL-divergence between $\pr$ and $\pr'$ is
bounded by conditional mutual information
$I(\mb X \indep \mb Y| \mb Z)$.
 % (See Appendix~\ref{app:prop} for details  \babak{add a proposition}).

 %It can be shown that the KL-divergence between  $F_{D}(\mb v)$ and $F_{\rep}(\mb v)$ is bounded by $I(X; Y|\mb Z)$.



==> Capuchin(Pre-print) (1)/transpar.tex <==




\vspace*{-0.2cm}
\section{Defining and Enforcing Algorithmic Fairness}
\label{sec:counter_fair}


\revb{In this section we introduce a new definition of fairness,
  which, unlike proxy fairness~\cite{kilbertus2017avoiding}, captures
  correctly group-level fairness, and, unlike counterfactual
  fairness~\cite{kusner2017counterfactual,DBLP:journals/corr/KusnerLRS17}
  is based on the standard notion of intervention and, hence, it is
  testable from the data.  In the next section we will describe how to
  repair an unfair training dataset to enforce fairness.
  % This section introduces a new causal notion of fairness that
  % similar to proxy fairness \cite{kilbertus2017avoiding} avoids
  % individual-level counterfactuals, hence it is at group-level.
  % However, it addresses some of the shortcomings of proxy fairness
  % discussed in Sec~\ref{sec:peri}. Then we describe our approach to
  % enforcing fairness.
}


%In this section we propose a new definition of fairness that is 
%significantly stronger than proxy fairness
%In this section, we characterize fairness based on interventional distributions,


\subsection{{Interventional Fairness}}
\label{sec:fairdef}

This section assumes that the causal graph is given. The
algorithm computes an output variable $O$ from input variables $\mb X$
(Sec.~\ref{sec:cvs}). We begin with a definition describing when an
outcome $O$ is causally independent of the protected attribute $S$ for
any possible configuration of a given set of variables $\mb K$.

\begin{definition}[$\mb K$-fair]   \label{def:cnf} Fix a set of
  attributes $\mb K \subseteq \mb V-\set{S,O}$.  We say that an
  algorithm $\mc A : Dom(\mb X) \rightarrow Dom(O)$ is $\mb K$-fair
  w.r.t. a protected attribute $S$ if, for any context $\mb K = \mb k$
  and every outcome $O=o$, the following holds:
	%
	{ 
	\begin{eqnarray}
	\pr(O=o| do(S=0),do(\mb K = \mb k))= \pr(O=o| do(S=1), do(\mb K = \mb k)) \label{eq:cfair}
	\end{eqnarray}
}
\end{definition}


%\babak{Last reviewer suggested not to use use the term indisputable fairness.}



% As an extreme case, we call the algorithm \reve{{\em interventionally
%     fair}} if it is $\mb K$-fair for every set $\mb K$. As opposed to
% proxy fairness that ensures $S$ (or its proxies) does not causally
% affects $O$ at population level, interventional fairness ensures $S$
% does not affect $O$ in any configuration of the system obtained by
% fixing other variables at some arbitrary values.  Intuitively, it
% ensures that the algorithm produces the same output for the protected
% and privileged groups no matter how we intervene on any other
% attributes. \revb{Therefore, even if the algorithm uses $S$ for
%   decision making at individual level, the unfairness cancel out in
%   all configurations of the system obtained by fixing other variables
%   by external interventions; motivating the term
%   ``interventional''. We argue that interventional fairness is the
%   strongest notion of fairness that is testable from data, hence it is
%   stronger than proxy fairness in Eq.~ \ref{eq:pfair}. We illustrate
%   with an example (see also Ex~\ref{ex:ap_str}).}


\revb{We call an algorithm \reve{{\em interventionally fair}} if it is
  $\mb K$-fair for every set $\mb K$.  Unlike proxy fairness, this
  notion captures correctly group-level fairness, because it ensures
  that $S$ does not affect $O$ in \emph{any configuration} of the
  system obtained by fixing other variables at some arbitrary values.
  Unlike counterfactual fairness, it does not attempt to capture
  fairness at the individual level, and therefore it uses the standard
  definition of intervention (the \texttt{do}-operator).  In fact, we
  argue that interventional fairness is the strongest notion of
  fairness that is testable from data, yet captures correctly
  group-level fairness. We illustrate with an example (see also
  Ex~\ref{ex:ap_str}).}



%  intervening on observed variables  do not reveal any signal in data that reveals the algorithm uses sensitive attributes at individual level for decision making, 

%\reva{To address (D3), add a discussion that justifiable fairness might still not capture fairness in general.}


\begin{example} \label{ex:intsprox} \em  In contrast to proxy
    fairness, interventional fairness correctly identifies the
    admission process in Ex.  \ref{ex:obsvsprox} as unfair at
    department-level. This is because the admission process fails to
    satisfy $\set{D}$-fairness since,
    $P(O=1| do(G=0), do(D=\text{'A'}))=0$ but
    $P(O=1| do(G=1), do(D=\text{'A'}))=\frac{1}{2}$. Therefore,
    interventional fairness is a more fine-grained notion than proxy
    fairness.
%
  \reve{We note however that, interventional fairness does not
    guarantee individual faintness in general. To see this suppose the
    admission decisions in both departments are based on student's
    gender and an unobserved exogenous factor $U_O$ that is uniformly
    distributed, i.e., $O=f(G,U_O)$, such that $f(G, 0)= G$ and
    $f(G,1)=1-G$. Hence, the causal DAG is $G \rightarrow O$.  Then
    the admission process is $\emptyset$-fair because,
    $P(O=1| do(G=1))=P(O=1| do(G=0))=\frac{1}{2}$. Therefore, it is
    interventionally fair (since $\mb V-\set{O,G} = \emptyset$).
    However, it is clearly unfair at individual level.  If the
    variable $U_0$ were endogenous (i.e. known to the algorithm), then
    the admission process is no longer interventionally fair, because
    it is not $\set{U_o}$-fair:
    $P(O=1| do(G=1), do(U_o=1))= P(O=1| G=1, U_o=1)=0$, while
    $P(O=1| do(G=1), do(U_o=1))=P(O=1| G=0, U_o=1)=1$. Under the same setting counterfactual fairnesses \cite{kusner2017counterfactual,DBLP:journals/corr/KusnerLRS17} fails to capture individual-level discrimination in this example (see Appendix~\ref{app:addback}).
% Note that,
%     counterfactual fairnesses in
%     \cite{kusner2017counterfactual,DBLP:journals/corr/KusnerLRS17}
%     also fails to identify individual-level unfairness in this example
%    See more discussion in %Appendix~\ref{app:addback}.}
%Note that if $U_O$ were observed,  interventional fairness  would have identified this case as unfair.
}
\end{example} 



% This is because  Eq~\ref{eq:cfair} ensures that the outcome of the algorithm is neutral to any changes in the sensitive attribute,  in all configurations of the system obtained by setting values to the other variables. In other words, not matter how the system is manipulated by external interventions, the (potential) effect of $S$ on the outcome of the algorithm is unobservable. We note however that an algorithm can be inteventionally fair but still unfair at individual level. This would happen if in all configurations of a system unfairness toward individuals cancel out at population level.

In practice, interventional fairness is too restrictive, as we show
below. To make it practical, we allow the user to classify variables
into {\em admissible} and {\em inadmissible}.  The former variables
through which it is permissible for the protected attribute to
influence the outcome.  In Example~\ref{ex:berkeley}, the user would
label department as admissible since it is considered a fair use in
admissions decisions, and would (implicitly) label all other variables
as inadmissible, for example, hobby.  Only users can identify this
classification, and therefore admissible variables are part of the
problem definition:

%\reve{D5: Examples. I liked the many illustrating examples given in the paper, but I think the paper would be much stronger if the authors also comment on what examples the proposed justifiable fairness would actually fail. Note that since justifiable fairness is an observational definition, according to [21] it must be insufficient to address certain discriminatory problems. The writing of the current draft gives the wrong impression that justifiable fairness is a better choice (in all cases). I would also suggest the authors refrain from using the term "indisputable fairness."}


\begin{definition}[Fairness application]  \label{def:app} A \fairapp
  over a domain $\mb V$ is a tuple $(\mc A, S, \mb A, \mb I)$, where
  $\mc A$ is an algorithm $Dom(\mb X) \rightarrow Dom(O)$;
  $\mb X \subseteq \mb V$ are its input variables; $S,O \in \mb V$ are
  the protected attribute and outcome, and
  $\mb A \cup \mb I = \mb V - \set{S,O}$ is a partition of the
  variables into admissible and inadmissible.
\end{definition}

We can now introduce our definition of fairness:
%%%, which always
%%%intervenes on all supersets of admissible variables (i.e., it sets
%%%fixed values for these variables):

\begin{definition}[Justifiable fairness]  \label{def:jf} A \fairapp 
  $(\mc A,$ $S, \mb A, \mb I)$ is {\em justifiability fair} if it is
  $\mb K$-fair w.r.t. all supersets $\mb K \supseteq \mb A$.
\end{definition}

%\revb{W1) Novelty of the proposed definition needs to be justified compared to proxy fairness in [21]}


Notice that
interventional fairness corresponds to the case where no variable is
admissible, i.e., $\mb A = \emptyset$.

%Intuitively, an algorithm is justifiably fair if, by setting any
%values to all admissible variables and any other variables, the
%algorithm's outcome is neutral to any changes in $S$.  Notice that
%indisputable fairness corresponds to the case where no variable is
%admissible, i.e., $\mb A = \emptyset$.

We give next a characterization of justifiable fairness in terms of
the structure of the causal DAG:
\vspace*{-0.1cm}
\begin{theorem} \label{th:jfcd}  If all directed paths from $S$ to $O$
  go through an admissible attribute in $\mb A$, then the algorithm is
  justifiably fair.  If the probability distribution is faithful to
  the causal DAG, then the converse also holds.
\end{theorem}

To  ensure interventional fairness,  a sufficient
condition is that there exists no path from $S$ to $O$ in the causal
graph (because $\mb A = \emptyset$).  \reve{(Hence, under faithfulness, interventional fairness implies fairness at individual-level, i.e., intervening on the sensitive attribute does not change the counterfactual outcome of individuals.}) Since this is too strong in most
scenarios, we adopt justifiable fairness instead.
%
%
%
\begin{figure*} \centering
	\begin{subfigure}{0.3\textwidth} 
		\hspace*{-0.8cm}
		\includegraphics[scale=0.15]{Fig2_a.pdf}
		\caption{College~\RNum{1}}
	\end{subfigure}
	\begin{subfigure}{0.3\textwidth} 
		%	\hspace*{-1.3cm}
		\includegraphics[scale=0.15]{Fig4_b.pdf}
		\caption{ College~\RNum{2}}
	\end{subfigure}



	{
		\begin{tabular}{c@{\qquad}ccc@{\qquad}ccc}
			\toprule
			\multirow{2}{*}{\raisebox{-\heavyrulewidth}{{\bf College~\RNum{1}}}} & \multicolumn{2}{c}{Dept.~A} & \multicolumn{2}{c}{Dept.~B} & \multicolumn{2}{c}{Total}  \\
			\cmidrule{2-7}
			& Admitted & Applied & Admitted &Applied & Admitted & Applied \\
			\midrule
			Male& 16 &  20 & 16 & 80 & 32 & 100 \\
			Female& 16 & 80 & 16 & 20 & 32 & 100 \\
			\bottomrule
		\end{tabular}
\hspace*{-0.2cm}			\begin{tabular}{c@{\qquad}ccc@{\qquad}ccc}
			\toprule
			\multirow{2}{*}{\raisebox{-\heavyrulewidth}{\bf College~~\RNum{2}}} & \multicolumn{2}{c}{Dept.~A} & \multicolumn{2}{c}{Dept.~B} & \multicolumn{2}{c}{Total}  \\
			\cmidrule{2-7}
			& Admitted & Applied & Admitted &Applied & Admitted & Applied \\
			\midrule
						Male& 10 & 10 & 40 & 90 & 50 & 100 \\
			Female& 40 &  50 & 10 & 50 & 50 & 100 \\

			\bottomrule
		\end{tabular}
	}
	%Sandy: note changes made below to figure caption text.
	\caption{      \textmd{ Admission process representation in two colleges where  the associational notions of fairness fail (see Ex.\ref{ex:ap_str}).}}
	\label{adm_rate}
\end{figure*}
%
We illustrate with an example.
%
%
 %\revb{D2) The introduction does a good job highlighting why simplistic fairness measure such as DP fails to capture fairness and highlight many other families of definitions. But at the same time, the paper highlights the benefits of the k-neutrality definition compared only to the conditional statistical parity (and its related causality-based, counterfactual fairness). Other more related definitions like path-specific and individual fairness were ignored even in the motivating examples. More elaboration here will be great}

\begin{example} \label{ex:ap_str} \em Fig~\ref{adm_rate} shows how fair or
  unfair situations may be hidden by coincidences but exposed through
  causal analysis.  In both examples, the protected attribute is
  gender $G$, and the admissible attribute is department $D$. Suppose
  both departments in College~\RNum{1} are admitting only on the basis
  of  their applicants' hobbies.  Clearly, the admission process is
  discriminatory in this college because department~A admits 80\% of
  its male applicants and 20\% of the female applicants, while
  department~B admits 20\% of male and 80\% of female applicants.  On
  the other hand, the admission rate for the entire college is the
  same 32\% for both male and female applicants, falsely suggesting
  that the college is fair.  Suppose $H$ is a proxy to $G$ such that $H=G$ ($G$ and $H$ are the same), then proxy
  fairness classifies this example as
  fair: indeed, since Gender has no parents in the causal graph,
  intervention is the same as conditioning, hence
  $\pr(O=1|do(G=\text{i}))=\pr(O=1| G = \text{i})$ for $i=0,1$.  Of the previous methods, only conditional
  statistical parity correctly indicates discrimination.  We
  illustrate how our definition correctly classifies this examples as
  unfair.  Indeed, assuming the user labels the department $D$ as
  admissible, $\set{D}$-fairness fails because, by Eq.(\ref{eq:af}),
  $\pr(O=1|do(G=1),do(D=\text{'A'}))=\sum_h
  \pr(O=1|G=1,D=\text{'A'},h)\pr(h|G=1) =
  \pr(O=1|G=1,D=\text{'A'})=0.8$,
%
%   {\small
%     \begin{align*}
%       \sum_h \pr(O=1|G=1,D=\text{'A'},h)\pr(h|G=1) = & \pr(O=1|G=1,D=\text{'A'})=0.8
%     \end{align*}
%   }
%
% %
%     \begin{align*}
%       \pr(O=1|do(G=1),do(D=\text{'A'}))=&\sum_h \pr(O=1|G=1,D=\text{'A'},h)\pr(h|1) \\
%        = & \pr(O=1|G=1,D=\text{'A'})=0.8 \\
%       \pr(O=1|do(G=0),do(D=\text{'A'}))=&\sum_h \pr(O=1|G=0,D=\text{'A'},h)\pr(h|0) \\
%        = & \pr(O=1|G=0,D=\text{'A'})=0.2
%     \end{align*}
%
%
  and, similarly $\pr(O=1|do(G=0),do(D=\text{'A'}))=0.2$.
%
  Therefore, the admission process is not justifiably fair.

  Now, consider the second table for College~\RNum{2}, where both
  departments~A and B admit only on the basis of student
  qualifications $Q$.  A superficial examination of the data suggests
  that the admission is unfair: department A admits 80\% of all
  females, and 100\% of all male applicants; department B admits 20\%
  and 44.4\% respectively.  Upon deeper examination of the causal DAG,
  we can see that the admission process is justifiably fair because
  the only path from Gender to the Outcome goes through department,
  which is an admissible attribute.  To understand how the data could
  have resulted from this causal graph, suppose 50\% of each gender
  have high qualifications and are admitted, while others are
  rejected, and that 50\% of females apply to each department but
  more qualified females apply to department A than to B (80\%
  v.s. 20\%). Further, suppose fewer males apply to department A, but
  all of them are qualified.  The algorithm satisfies demographic
  parity and proxy fairness but fails to satisfy conditional
  statistical parity since $\pr(A=1|G=1,D=\text{A})=0.8$ but
  $\pr(A=1|G=0,D=\text{A})=0.2)$.  Thus, conditioning on $D$ falsely
  indicates discrimination in College~\RNum{2}. One can check that the
  algorithm is justifiably fair, and thus our definition also
  correctly classifies this example; for example, $\set{D}$-fairness
  follows from Eq.(\ref{eq:af}):
  $\pr(O=1|do(\text{G}=\text{i}),do(D=d))= \sum_{q}\pr(O=1|G=i,d,q))
  \nonumber \pr(q|G=i)= \frac{1}{2}$.
% 	$$
% 	\pr(O=1|do(\text{G}=\text{i}),do(D=d))=
% 	\sum_{q}\pr(O=1|G=i,d,q)) \nonumber \pr(q|G=i)= \frac{1}{2}
% 	$$  for $i=0,1$ and $d=\{\text{A},\text{B}\}$. It is easy to verify that $\set{D,Q}$-neutrality also holds.
%	Hence, the admission process in the second collage is justifiably fair.
  To summarize, unlike previous definitions of fairness, justifiable
  fairness correctly identifies College~\RNum{1} as discriminatory and
  College~\RNum{2} as fair.


\end{example}

\ignore{
	\begin{figure}
		\begin{subfigure}{0.2\textwidth} \centering
			\hspace*{-0.8cm}
			\includegraphics[scale=0.1]{fig/Fig5_a.pdf}
			\caption{ }
		\end{subfigure}
		\begin{subfigure}{0.2\textwidth} \centering
			%	\hspace*{-1.3cm}
			\includegraphics[scale=0.1]{fig/Fig5_b.pdf}
			\caption{ }
		\end{subfigure}

		\ignore{
			\vspace*{2mm}	\begin{subfigure}{0.2\textwidth} \centering
				\hspace*{-0.8cm}
				\includegraphics[scale=0.4]{fig/safe.png}
				\caption{ }
			\end{subfigure}
			\begin{subfigure}{0.2\textwidth} \centering
				\hspace*{0.5cm}
				\includegraphics[scale=0.4]{fig/admi.png}
				\caption{ }

			\end{subfigure}
		}
		\caption{Represent a PCM in which the admission process is contextually fair w.r.t. department.}
		\label{fig:cgex2}
	\end{figure}
}


\ignore{
	\begin{figure}

		\begin{subfigure}{0.2\textwidth} \centering
			\includegraphics[scale=0.15]{fig/gDAG.png}
		\end{subfigure}
		\begin{subfigure}{0.2\textwidth} \centering

			\begin{align}
			O &: &  \text{Outcome} \nonumber \\
			\mb N &: &  \text{Inadmissibles} \nonumber \\
			\mb D &: &  \text{Admissibles} \nonumber \\
			S &: &  \text{Sensitive} \nonumber \\
			\mb D' &: &  \text{Other Admissibles} \nonumber
			\end{align}
		\end{subfigure}
		\caption{A generic causal DAG that illustrates an algorithm that is not Justifiably fair.}
		\label{fig:dic}
	\end{figure}
}

% In the next section, we establish a sufficient condition for justifiable fairness. Then, we propose methods for building justifiably fair classification algorithms that do not rely on the existence of causal DAGs.



\subsection{Testing Fairness on the Training Data}
\label{sec:jfc}

In this section we introduce a sufficient condition for testing
justifiable fairness, which uses only the training data $D, \pr$
(Sec.~\ref{sec:peri}) and does not require access to the causal graph
$\cg$.  We  assume only that $\cg$ and $\pr$ are Markov compatible
(Sec.~\ref{sec:causal:dag}). The training data has an additional
response variable $Y$.  As before, we assume a \fairapp $(\mc A,$
$S, \mb A, \mb I)$ is  given and  that the algorithm is a
good prediction of the response variable, \ie\,
%
%
% We are given a set of attributes $\mb V$ from a domain with an
% underlying causal DAG $\cg$ that is unknown, an outcome attribute
% $Y \in \mb V$, a protected attribute $S \in \mb V$, and a set of
% admissible attributes $\mb{A} \subseteq \mb{V} -\set{S,Y}$.  Our goal
% is to ensure that a classification algorithm $\mc A$ trained on a
% subset of attributes $\mb X \subseteq \mb V$ is justifiably fair.  A
% naive solution to the problem that is canonical in practice is to
% simply hide all protected attributes during training an algorithm.
% For example, to prevent an algorithm from learning a relationship
% between gender and admissions, it might be tempting to simply not
% expose gender during training.  But since inadmissible variables can
% encode gender, this approach is not effective.
% In this section first we establish a sufficient condition for an
% algorithm to be justifiably fair. Then we propose two methods for
% building justifiably fair predictive classification algorithms.
% Throughout this paper, we make the typical assumption that $\mc{A}$
% approximates the true conditional distribution, i.e., we assume
%
$\pr(Y=1| \mb X=\mb x) \approx \pr(O=1| \mb X=\mb x)$; we call the
algorithm a \emph{reasonable} classifier to indicate that it satisfies
this condition. \reve{ Note that this is a typical assumption in pre-processing approachs, see e.g., \cite{NIPS2017_6988} and needed to decouple the
	the issues of model accuracy and fairness. If the distributions of $\pr(Y=1| \mb X=\mb x)$ and $\pr(O=1| \mb X=\mb x)$ could be arbitrarily far apart, no fairness claims can be made about a classifier that, for example, imposes
	a pre-determined distribution on the outcome predictions rather than learning
	an approximation of $\pr(Y=1| \mb X=\mb x)$ from the training data.}
%  We defer to future work a full characterization of
% approximation error and mismatch between the distribution of sample
% and training data and its effect on fairness.

% this implied that the following result holds in approximation.

We first establish a technical condition for fairness based on the
Markov boundary, and then we simplify it.  Recall that, give a probability
distribution $\Pr$, the {\em Markov boundary} of a variable
$Y \in \mb V$, denoted $\mmb(Y)$, is a minimal subset of
$\mb V-\set{Y}$ that satisfies the saturated conditional independence
$(Y \indep_\pr \mb V-(\mmb(Y) \cup \set{Y}) | \mmb(Y))$. Intuitively,
$\mmb(Y)$ shields $Y$ from the influence of other variables.  It is
usually assumed that the Markov boundary of a variable is unique (see
Appendix~\ref{app:addback}).  We prove:
% and it is known that $\mmb(Y)$ can be learned from data using a
% number of iterations on $D$ that is linear in the
% variables~\cite{margaritis2003learning}.

% First, we give a sufficient condition for justifiable fairness:

\begin{theorem} \label{theo:suff_jf}  A sufficient condition for a
  \fairapp $(\mc A, S, \mb A, \mb I)$ to be justifiably fair is
  $\mmb(O) \subseteq \mb A$.
\end{theorem}

If $\pr$ is faithful to the causal graph, then the theorem follows
immediately from Theorem~\ref{th:jfcd}; but we prove it without
assuming faithfulness in Appendix~\ref{app:proof}.  The condition in
Theorem~\ref{theo:suff_jf} can be checked without knowing the causal
DAG, but requires the computation of the Markov boundary;
%%%
%%%It says that, if admissible variables shield
%%%the outcome of algorithm from the influence of sensitive and
%%%inadmissible variables, the algorithm is justifiably fair.
% The fact
% that CIs can be checked effectively against data, is a key observation
% that enables us to build justifiably fair classifiers without
% adherence to causal DAGs.
moreover, it is expressed in terms of the outcome $O$ of the
algorithm.  We derive from here a sufficient condition without
reference to the Markov boundary, which refers only to the response
variable $Y$ present in the training data.



% However, our goal is to ensure that the sufficient articulated in Theorem~\ref{theo:suff_jf} holds for the outcome of a predictive classification algorithm.
% We give next a sufficient conditions for building justifiably fair classifiers. %The following obtained from Theorem~\ref{theo:suff_jf} and the assumption of reasonable classifier.

%However, to use this theorem, we must reason about the outcome of an algorithm. \babak{classification algorithm ?} In our pre-processing setting, we have access only to training data.   We want to repair the training data so that any reasonable classifier trained on it is justifiably fair. Therefore, we need a sufficient condition for justifiable fairness that can be checked using the training data, which the following Corollary provides:




\begin{corollary} \label{col:fair_learn} Fix a training data $D, \pr$,
  where $Y \in \mb V$ is the training label, and $\mb A, \mb I$ are
  admissible and inadmissible attributes.  Then any reasonable
  classifier trained on a set of variables $\mb X \subseteq \mb V$ is
  justifiably fair w.r.t. a protected attribute $S$, if any of the following hold:
	\begin{itemize}
		\item[(a)] $\pr$ satisfies the CI $(Y \indep \mb X \cap \mb I  | \mb X \cap \mb{A} )$, or
		\item[(b)] $\mb X \supseteq \mb A$ and $\pr$ satisfies the saturated CI $(Y \indep \mb \mb I |\mb{A})$.
	\end{itemize}
\end{corollary}



The proof is the Appendix.
%\luke{(To address F:D4 above) We require that the classifier be reasonable, as otherwise the distributions of $\pr{Y|X}$ and $\pr{O|X}$ could be arbitrarily far apart. No fairness claims can be made about a classifier that, for example, imposes a pre-determined distribution on the outcome predictions rather than learning an approximation of $\pr{Y|X}$ from the training data.}
While condition (a) is the weaker
assumption, condition (b) has the advantage that the CI is saturated.
Our method for building a fair classifier is to repair the training
data in order to enforce (b).



%\begin{corollary} \label{col:fair_learn_mb}  Given a dataset  $D$ over $\mb V$ with a protected attribute $S$ and training labels $Y$, and given a set of admissible variables $\mb A$, if $D$ satisfies the saturated CI $(Y \indep \mb V-(\mb{A} \cup \set{Y}) |\mb{A})$, where  then any classifier trained on $\mb X \supseteq \mb A$ is justifiably fair.
%\end{corollary}


\subsection{Building Fair Classifiers}
\label{sec:build}

This leads us to the following methods for building justifiably fair classifiers.




\paragraph*{\bf Dropping Inadmissible Attributes} A naive way to
satisfy Corollary~\ref{col:fair_learn}(a) is to set $\mb X = \mb A$,
in other words  to
train the classifier only
on  admissible attributes
% $\mb A$, i.e., $\mb X=\mb A$ (other variables that are independent
% of $Y$ by conditioning on $\mb A$ can be also added to $\mb X$).
This method guarantees fairness, but, as we will show in
Sec.~\ref{sec:experi}, dropping even one inadmissible variable can
negatively affect the accuracy of the classifier.  Moreover, this
approach cannot be used in data release situations, where all
variables must be included. Releasing data that reflect  discrimination can
 unintentionally reinforce and amplify discrimination in other
 contexts that data is used.
%Our approach allows all attributes to be released, but it repairs the unwanted bias.
%If the requirement in Corollary~\ref{col:fair_learn}  is satisfied, then the classifier is not only justifiably fair  but also satisfies Conditional Statistical Parity $S \indep O | \mb V'$ for any  $ \mb A \cap \mb X \subseteq \mb V' \subseteq \mb V-\set{O,S}$. This in turn implies $(S \indep O | \mb V', Y)$, meaning the classifier has the same FP and FN rates for protected and privileged groups in subpopulations that are homogeneous on $\mb V'$.
%It is clear tthat training a classifier on  only admissible variable ensures the classifier is justifiably fair.
%However, our goal is to ensure fairness by repairing data.
%
%We would refer this property as {\em Conditional Equalized Odds}, meaning that condition on the admissible variables the protected and privileged groups have the  TP and FP rates. Notice that for $\mb D=\emptyset$, i.e., all variables deemed to be inadmissible, then Theorem~Corollary~\ref{col:fair_learn}   gives a sufficient condition for satisfying Statistical Parity and Equalized Odds.
%\babak{I suggest put the paragraph on dropping attributes back. But now make it very short. I also like to sate one can select other variables using DAG if its available.}
% \paragraph*{\bf Dropping Inadmissible Attributes}  A canonical  method for ensuring both requirements in Corollary~\ref{col:fair_learn} is to train the classifier on $\mb X= \mb A$, i.e., to drop sensitive attribute and inadmissible variables from the training variables. Note that if the underling causal DAGs is available, one can further read a set of variables  $\mb W$  off the causal DAG such that $Y$ and $\mb W$ are d-separated by  $\mb  A$, hence $Y \indep \mb W |\mb{A}$), and train the classifier on $\mb X=\mb A \cup \mb W$.

%While dropping variables is effective for preventing discrimination, in Sec.~\ref{sec:experi}, we empirically show that dropping even one inadmissible variable can negatively affect the precision of classifier.  In addition, this approach can not be integrated with data release mechanism. Releasing data that reflect historical bias and discrimination or collected using a discriminatory mechanism can intendedly reinforce and amplify the bias in other contexts that data is used.

\paragraph*{\bf Repairing Training Data}
Instead, our approach is to repair the training data to enforce the
condition in Corollary~\ref{col:fair_learn}(b).
% essentially shows if Markov boundary
% of $Y$ consists of admissible variables, then training a classifier on
% any supersets $\mb X \supseteq \mb A$ that can possibly include the
% protected and inadmissible attributes leads to a classifier that is
% justifiably fair. Note that $\mmb(Y) = \mb A$ implies that the
% mechanism or algorithm that generated the training labels were
% justifiably fair. However, the training labels typically reflect
% discrimination in the real world or the data collection
% process. Therefore, the Markov Boundary of $Y$ may include sensitive
% and inadmissible variables.
We consider the saturated CI
$(Y \indep \mb I |\mb{A})$ as an {\em integrity constraint} that
should always hold in training data $D, \pr$.  \sys\ performs a
sequence of database updates (viz., insertions and deletions of
tuples) to obtain another training database $D'$ to satisfy
$(Y \indep \mb I |\mb{A})$.
% such that $\mmb(Y) = \mb A$ that satisfies the saturated CI
% $D' \models (Y \indep \mb V-(\mb{A} \cup \set{Y}) |\mb{A})$.
We describe this repair problem in Sec.~\ref{sec:repdata}.
% Hence, we reduce fairness to a database repair problem w.r.t. a
% saturated CI statement (see Section \ref{sec:peri}).
To the causal DAG, this approach can be seen as
modifying the underlying causal model to enforce the fairness
constraint.  However, instead of intervening on the causal DAG, which
we do not know and over which we have no control, we intervene on
the training data to ensure fairness. %We show emperically in sec~\ref{}
\reva{Note that minimal repairs are crucial for preserving the utility of data.  Specifically, we need to ensure that the joint distribution of training and repaired data are close. Since there is no general metric to measure the distance between  two distributions that works well for all datasets and applications, in Sec~\ref{sec:repdata} we propose several minimal repair methods. We empirically show that these methods behave differently for different datasets and ML algorithms.} \revb{We also note that the negative effect of repair on utility depends on several factors such as the size of data, sparsity of data,  repair method, ML algorithm, strongness of dependency that the repair method enforces; hence accuracy should be trade with fairness at training time. }




%In other words, the repaired training data can be seen as a sample from a hypothetical world that is  justifiably fair.  Hence, instead of intervening on the causal model, over which we have no control, to make it justifiably fair, we intervene on data. Note that the described approaches can be naturally extended to multiple sensitive attributes $\mb S$ by assuming that $\mb A$ consists of a set of variables that are admissible for all $ S \in \mb S$.

%Sandy:  verify meaning of following sentence that I edited.
%To preserve the utility of data, we need to ensure that the repaired dataset $D'$ is close enough to the original training data $D$ to motivate the problem of computing minimal database repairs that are inconsistent w.r.t. CI statements. We study this problem in Sec.~\ref{sec:repdata}.

